Adjoint Method in PDE-based Image Compression

We consider a shape optimization based method for finding the best interpolation data in the compression of images with noise. The aim is to reconstruct missing regions by means of minimizing a data fitting term in an $L^p$-norm between original images and their reconstructed counterparts using linear diffusion PDE-based inpainting. Reformulating the problem as a constrained optimization over sets (shapes), we derive the topological asymptotic expansion of the considered shape functionals with respect to the insertion of small ball (a single pixel) using the adjoint method. Based on the achieved distributed topological shape derivatives, we propose a numerical approach to determine the optimal set and present numerical experiments showing, the efficiency of our method. Numerical computations are presented that confirm the usefulness of our theoretical findings for PDE-based image compression.

==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/abstract.tex <==
\begin{abstract}

We consider a shape optimization  based method for finding the best interpolation data in the compression of images with noise. The aim is to reconstruct missing regions by means of minimizing a data fitting term in an $L^p$-norm, for $1\leq p<+\infty$, between original images and their reconstructed counterparts using linear diffusion PDE-based inpainting. Reformulating the problem as a constrained optimization over sets (shapes), we derive the topological asymptotic expansion of the considered shape functionals with respect to the insertion of small ball (a single pixel) using the adjoint method. Based on the achieved distributed topological shape derivatives, we propose a numerical approach to determine the optimal set and present numerical experiments showing the efficiency of our method. Numerical computations are presented that confirm the usefulness of our theoretical findings for PDE-based image compression.
\end{abstract}

\keywords{image compression \and shape optimization \and adjoint method \and image interpolation \and inpainting \and PDEs \and image denoising}


==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/conclusion.tex <==
\section*{Conclusion and Perspectives}

In this article, we formulated a (PDE-)compression problem based on the linear diffusion inpainting as a shape optimization one, and we estimated the topological expansion for the optimality condition by the adjoint method. More precisely, and following the approaches of \cite{Garreau2001, Amstutz2006}, we computed the asymptotic development with respect to insertion of a circular hole for variations of the $L^p$-error with general exponents $p \geq 1$, which leads to an analytic criterion to select relevant pixels of the mask using a hard-thresholding rule.
%
This criterion is determined by solving the linear diffusion equation and its adjoint equation which make the method easy to implement with a reasonable cost as both equations are linear.
%
Finally, we presented numerical results in the two following settings: when the data is corrupted by salt and pepper noise ($p=1$) and when the data is affected by Gaussian noise ($p=2$). In these experiments, we relaxed the hard-thresholding from the topological gradient by introducing a soft-thresholding, enforced with the \textit{Floyd-Steinberg} digital halftoning \cite{Ulichney1987}. This new approach delivers better results than hard-thresholding by giving a better distribution of the selected pixels.
%
Then, we compared our methods with those presented in \cite{Belhachmi2009}, which is also a PDE-based compression problem, but rely on homogeneous diffusion inpainting and use the $H^1$ semi-norm as the cost function.
%
Our mask selection methods outperform the other approaches when compressing images affected by Gaussian or impulse noise. Specifically, our methods effectively denoise the data by excluding corrupted pixels from the mask, resulting in a cleaner reconstruction. In contrast, the homogeneous diffusion inpainting methods include all noisy pixels, as the Laplacian of the noisy image is high around the corrupted pixels.

For future research, we aim to explore additional inpainting operators and alternative cost functionals to address various types of noise or combinations of different noise patterns. In the numerical section, the selection of $\alpha$ proves to be critical: if it is too low, there is no denoising, preserving the corrupted pixels; if it is too high, we end up losing the edges. However, determining the appropriate value of $\alpha$ remains unclear, which opens up potential research direction. Another goal would be to extend the method to colored images. Finally, further numerical studies, along with the use of advanced scientific computing tools -- such as parallelization and more precise algorithms -- will undoubtedly enhance this approach.

==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/draft.tex <==
% \section{draft}

% \[ E(z) := \frac{1}{2\pi} K_0\left(\frac{z}{\sqrt{\alpha}}\right). \]

% Lorsque $z$ est grand,

% \[ K_n(z) = \sqrt{\frac{\pi}{2}}z^{-1/2}e^{-z} + O\big(z^{-3/2}e^{-z}\big). \]

% Taylor quand $|y|\to +\infty$,

% \[ E\big(|y-x|\big) = E\big(|y|\big) + o(1) = E\big(|y|\big) - \nabla_y E\big(|y|\big)\cdot x + o(1). \]

% et

% \[ \nabla_y E\big(|y|\big) = \frac{1}{2\pi} \nabla_y K_0\left(\frac{|y|}{\sqrt{\alpha}}\right) = -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y \]

% d'où 

% \[ E\big(|y-x|\big) = E(|y|) + \nabla E(|y|) \cdot x + o(\|x\|^2) \]
% \[ = \frac{1}{2\pi} K_0\left(\frac{|y|}{\sqrt{\alpha}}\right) + \frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y\cdot x + O\left(K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y\cdot x\right). \]

% \[ \tilde{V}(y) := E(|y|) =\frac{1}{2\pi} K_0\left(\frac{|y|}{\sqrt{\alpha}}\right) \]
% \[ \tilde{W}(y) := O\left( K_0\left(\frac{|y|}{\sqrt{\alpha}}\right) \right) \]
% \[ \nabla \tilde{V}(y) := -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y \]

% \[ \nabla E\big(|y-x|\big) = \nabla\tilde{V}(y) + \nabla \tilde{W}(y) \]
% \[ \Leftrightarrow -\frac{1}{2\pi} K_1\left(\frac{|y-x|}{\sqrt{\alpha}}\right) |y-x|^{-1} y = -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y + \nabla \tilde{W}(y) \]
% \[ \Leftrightarrow -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y + O\left(K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y\right) = -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y + \nabla \tilde{W}(y) \]
% \[ \Leftrightarrow  \nabla \tilde{W}(y) = O\left(K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y\right) \]



% % \[ V(y) := \sqrt{\frac{\sqrt{\alpha}}{8\pi}}|y|^{-1/2}e^{-|y|/\sqrt{\alpha}} \int p\ d\sigma \]
% % \[ W(y) := O\big(|y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\big) \]
% % \[ \nabla V(y) := \sqrt{\frac{\sqrt{\alpha}}{8\pi}}|y|^{-3/2}e^{-|y|/\sqrt{\alpha}} y \int p\ d\sigma \]
% % \[ \nabla W(y) := O\big(|y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\big) y \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow V(y) := \sqrt{\frac{1}{8\pi\sqrt{\alpha}}}|y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\int_{\partial B_1} p(x)\ d\sigma(x) \]
% \[ \Longrightarrow W(y) := O\big(|y|^{-3/2}e^{-|y|/\sqrt{\alpha}}\big) \]

% ---------------------------------------------------------------------------------

% SageMath : 

% \[ -\frac{e^{\left(-\frac{u\left(z\right)}{\sqrt{\alpha}}\right)} \frac{\partial}{\partial z}u\left(z\right)}{\sqrt{\alpha} \sqrt{u\left(z\right)}} - \frac{e^{\left(-\frac{u\left(z\right)}{\sqrt{\alpha}}\right)} \frac{\partial}{\partial z}u\left(z\right)}{2 \, u\left(z\right)^{\frac{3}{2}}} \]

% et 

% \[ u(z) = |z|, \]
% \[ \partial_z u(z) = \nabla u(z) = |z|^{-1} z, \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow \nabla V(y) = - \sqrt{\frac{1}{8\pi\sqrt{\alpha}}} e^{\left(-\frac{|y|}{\sqrt{\alpha}}\right)} |y|^{-1} \left( \frac{1}{\sqrt{\alpha} \sqrt{|y|}} + \frac{1}{2 \, |y|^{\frac{3}{2}}} \right) y \int_{\partial B_1} p(x)\ d\sigma(x) \]

% ---------------------------------------------------------------------------------

% \[ \nabla_y v_\omega(y) = -\frac{1}{2\pi}\int_{\partial B_1} |y-x|^{-1} K_1(|y-x|)\, p(x)\ d\sigma(x)\ y \]
% \[ = -\sqrt{\frac{1}{8\pi\sqrt{\alpha}}}|y|^{-1}\int_{\partial B_1}  |y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\, p(x)\ d\sigma(x)\ y + O\big(|y|^{-5/2}e^{-|y|/\sqrt{\alpha}}\big)y \]
% \[ = -\sqrt{\frac{1}{8\pi\sqrt{\alpha}}}\int_{\partial B_1}  |y|^{-3/2}e^{-|y|/\sqrt{\alpha}}\, p(x)\ d\sigma(x)\ y + O\big(|y|^{-5/2}e^{-|y|/\sqrt{\alpha}}\big)y. \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow \nabla W(y) = O\big(|y|^{-7/2}e^{-|y|/\sqrt{\alpha}}\big)y \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow |V(y)| \leq C_1\, |y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\, \|\varphi\|, \]
% \[ \Longrightarrow |W(y)| \leq C_2\, |y|^{-3/2}e^{-|y|/\sqrt{\alpha}}\, \|\varphi\|, \]
% \[ \Longrightarrow |\nabla V(y)| \leq C_3\,|y|^{-1/2}\left( 1 + |y|^{-1} \right) e^{-|y|/\sqrt{\alpha}} \, \|\varphi\| \leq C_3\,|y|^{-1/2}e^{-|y|/\sqrt{\alpha}} \, \|\varphi\|, \]
% \[ \Longrightarrow |\nabla W(y)| \leq C_4\, |y|^{-5/2}e^{-|y|/\sqrt{\alpha}}\, \|\varphi\|. \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow |V(y)| \leq C_1\, |y|^{-1/2}\, \|\varphi\|_{1/2,\partial B_1}, \]
% \[ \Longrightarrow |W(y)| \leq C_2\, |y|^{-3/2}\, \|\varphi\|_{1/2,\partial B_1}, \]
% \[ \Longrightarrow |\nabla V(y)| \leq C_3\,|y|^{-1/2} \, \|\varphi\|_{1/2,\partial B_1}, \]
% \[ \Longrightarrow |\nabla W(y)| \leq C_4\, |y|^{-5/2}\, \|\varphi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|V\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |V|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_3\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |W|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_4\, \, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|V\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_5\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |V|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_6\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_7\, \varepsilon^{1/2} \,\|\psi\|_{1/2,\partial B_1}, \]
% \[ |W|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_8\, \varepsilon^{3/2}\, \|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|V\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\,\|\psi\|_{1/2,\partial B_1}, \]
% \[ \|V\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_3\, \varepsilon^{-1/2} \,\|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_4\, \varepsilon^{1/2} \,\|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |v_\omega|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_3\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_4\,\varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |v_\omega|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_5\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_6\,\varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \begin{proposition} Soit $\psi\in H^{1/2}(\partial B_1)$.

%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta v_\varepsilon + v_\varepsilon = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         v_\varepsilon = \psi(\,\cdot\,/\varepsilon), & \text{sur}\ \partial B_\varepsilon, \\
%         v_\varepsilon = 0, & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\varepsilon\|_{0,B_R\setminus B_\varepsilon} \leq C_1\,\varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}, \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_\varepsilon} \leq C_2\,\varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}, \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C_3\,\varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}. \]
% \end{proposition}

% \begin{proposition}
%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta v_\varepsilon + v_\varepsilon = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         v_\varepsilon = \psi, & \text{sur}\ \partial B_\varepsilon, \\
%         v_\varepsilon = \varphi, & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\varepsilon\|_{0,B_R\setminus B_\varepsilon} \leq C_1\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}\big), \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_\varepsilon} \leq C_2\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}\big), \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C_3\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}\big). \]
% \end{proposition}

% ---------------------------------------------------------------------------------

% \[ \int_{\partial B_R} (T_\varepsilon-T_0) v_0\ d\sigma = \int_{\partial B_R} \partial_n (v_\varepsilon^{0,v_0} - v_0^{0,v_0})\ d\sigma \]

%     On pose pour $x\in \R^2\setminus B_\varepsilon$,
    
%     \[ w_\varepsilon^{0,v_0}(x) := v_\varepsilon^{0,v_0}(x) - v_0^{0,v_0}(x) + v_\omega(x/\varepsilon). \]
    
%     Ainsi, 
    
%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta w_\varepsilon^{0,v_0} + w_\varepsilon^{0,v_0} = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         w_\varepsilon^{0,v_0} = v_0(x_0) - v_0^{0,v_0}, & \text{sur}\ \partial B_\varepsilon, \\
%         w_\varepsilon^{0,v_0} = v_\omega(\cdot/\varepsilon), & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\omega(\cdot/\varepsilon)\|_{1/2,\partial B_R} \leq \|v_\omega(\cdot/\varepsilon)\|_{1,B_{R/2}\setminus B_R} \]
%     \[ \leq \|v_\omega(\cdot/\varepsilon)\|_{0,B_{R/2}\setminus B_R} + |v_\omega(\cdot/\varepsilon)|_{1,B_{R/2}\setminus B_R} \]
%     \[ \leq \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|v_\omega|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \]
%     \[ \leq \|V\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \|W\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|V|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|W|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \]
%     \[ \leq \big(C_5\,R^{1/2}\varepsilon^{-1/2} + C_6\,R^{-1/2}\varepsilon^{1/2} + C_7\,R^{-1/2}\varepsilon^{3/2} + C_8\,R^{1/2}\varepsilon^{1/2}\big)\|\psi\|_{1/2,\partial B_1} \]
%     \[ \leq C\,\varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}. \]
    
%     Aussi, (Annexe)

%     \[ \| v_0(x_0) - v_0^{0,v_0}(\varepsilon \cdot) \|_{1/2,\partial B_1} \leq \| v_0(x_0) - v_0^{0,v_0}(\varepsilon \cdot) \|_{1, B_1\setminus B_{1/2}} \]
%     \[ \leq \| v_0(x_0) - v_0^{0,v_0}(\varepsilon \cdot) \|_{1, B_1} \]
    
%     Ainsi,
    
%     \[ |w_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C\big( \varepsilon^{?}\|v_\omega(x/\varepsilon)\|_{1/2,\partial B_R} + \varepsilon^{?}\|v_0(x_0) - v_0^{0,v_0}(\cdot/\varepsilon)\|_{1/2,\partial B_1} \big) \]
    
%     Enfin, (44)
    
%     \[ \|\nabla (v_\varepsilon^{0,\psi} - v_0^{0,\psi} + V^{0,\psi} ) \cdot n\|_{-1/2,\partial B_R} \leq C |v_\varepsilon^{0,\psi} - v_0^{0,\psi} + V^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ \leq C |v_\varepsilon^{0,\psi} - v_0^{0,\psi} + V^{0,\psi} + W^{0,\psi} - W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ = C |v_\varepsilon^{0,\psi} - v_0^{0,\psi} + v_\omega - W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ = C |w_\varepsilon - W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ \leq C \Big(|w_\varepsilon|_{1,B_R\setminus B_{R/2}} + |W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \Big) \]
    
% \newpage \section{Draft 2}

% \[ \Longrightarrow |V(y)| \leq C_1\, |y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\, \|\varphi\|, \]
% \[ \Longrightarrow |W(y)| \leq C_2\, |y|^{-3/2}\, \|\varphi\|, \]
% \[ \Longrightarrow |\nabla V(y)| \leq C_3\,|y|^{-1/2}e^{-|y|/\sqrt{\alpha}} \, \|\varphi\|, \]
% \[ \Longrightarrow |\nabla W(y)| \leq C_4\, |y|^{-5/2}\, \|\varphi\|. \]

% ---------------------------------------------------------------------------------

% \[ \|V\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |V|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_3\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |W|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_4\, \, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|V\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_5\, e^{-R/(\varepsilon\sqrt{\alpha})}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |V|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_6\, e^{-R/(\varepsilon\sqrt{\alpha})}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_7\, \varepsilon^{1/2} \,\|\psi\|_{1/2,\partial B_1}, \]
% \[ |W|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_8\, \varepsilon^{3/2}\, \|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|V\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\,\|\psi\|_{1/2,\partial B_1}, \]
% \[ \|V\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_3\, e^{-R/(\varepsilon\sqrt{\alpha})} \,\|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_4\, \varepsilon^{1/2} \,\|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |v_\omega|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_3\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_4\,\varepsilon^{1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |v_\omega|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_5\, \varepsilon^{3/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_6\,\varepsilon^{1/2}\, \|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \begin{proposition} Soit $\psi\in H^{1/2}(\partial B_1)$.

%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta v_\varepsilon + v_\varepsilon = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         v_\varepsilon = \psi(\,\cdot\,/\varepsilon), & \text{sur}\ \partial B_\varepsilon, \\
%         v_\varepsilon = 0, & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\varepsilon\|_{0,B_R\setminus B_\varepsilon} \leq C_1\,\varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}, \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_\varepsilon} \leq C_2\,\varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}, \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C_3\,\varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}. \]
% \end{proposition}

% \begin{proposition} Soient $\psi\in H^{1/2}(\partial B_1)$ et $\varphi\in H^{1/2}(\partial B_R)$.
%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta v_\varepsilon + v_\varepsilon = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         v_\varepsilon = \psi(\,\cdot\,/\varepsilon), & \text{sur}\ \partial B_\varepsilon, \\
%         v_\varepsilon = \varphi, & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\varepsilon\|_{0,B_R\setminus B_\varepsilon} \leq C_1\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}\big), \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_\varepsilon} \leq C_2\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}\big), \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C_3\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}\big). \]
% \end{proposition}


\section{Draft}



==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/introduction.tex <==
\section*{Introduction and Related Works}

PDE-based methods have attracted growing interest by researchers and engineers in image analysis field 
%are gaining more attention 
during the last decades \cite{Perona1990, Catte1992, Weickert1996, Masnou1998, Weickert1999, Bertalmio2000, Scherzer2008, Lenzen2011, Larnier2012, Adam2017}.
Actually, such methods have reached their maturity both from the point of view of modeling and scientific computing allowing them to be used in modern image technologies and their various applications. Image compression is one of the domain where they appear among the state-of-the-art methods \cite{Chan2001, Galic2008, Schmaltz2009, Bae2010, Peter2015, Andris2016, Mohideen2020}. In fact, the aim for such problems is to store few pixels of a given image (coding phase) and to recover/restore  
the missing part in an accurate way (decoding). The PDE-based methods use a diffusion differential operator for the inpainting of missed parts 
from an available data (boundary or small parts of the initial image) therefore their efficiency for decoding is guaranteed/encoded in the operator without any pre- or post-treatment. The question then is how to ensure with these methods a good choice, if it exists, of the ``best'' pixels to store for high quality reconstruction of the entire image?
An answer to this question is given in \cite{Belhachmi2009, Belhachmi2022Jun} for the harmonic or the heat equation, where its reformulation as a constrained (shape) optimisation problem permitted to exhibit an optimal set of pixels to do the job. In addition, analytic selection criteria using topological asymptotics were derived. Due to the simple structure of the shape functionals considered in these previous works, the topological expansion is easily derived (more or less with formal computations) and gives an analytic criterion to characterize the optimal set in compression. 
The limitation in obtaining the topological expansion this way is twofold : the criterion gives pointwise information on the importance of the location (pixel) to store which results in hard thresholding selection strategy not robust with respect to the noise. Second, the technique is limited to simple functionals, namely an $L^2$ data-fitting term and a linear diffusion operator.

The main contribution of this article is the use of the adjoint method \cite{Amstutz2006}-\cite{Garreau2001} to derive an analytic criterion for PDE-based compression. In fact, we consider the compression problem in the same framework than \cite{Belhachmi2009}, but we introduce a new approach to the characterization of the set of pixels to select using the adjoint method \cite{Guillaume2002, Garreau2001, Amstutz2006, Belhachmi2018}. This approach to obtain the topological expansion is more general than the one previously studied for the same problem in \cite{Belhachmi2009}, in the sense that it may be used for other diffusion operators and nonlinear data-fitting term, moreover it allows a better stability with respect to noise. In particular, when the accuracy of the reconstruction (fidelity term) is measured with an $L^p$-norm, $1\leq p < +\infty$, the adjoint method is still linear and no significant complexity or cost are added. Thus, the main results in the article include the rigorous derivation of the topological expansion based on the adjoint problem in the spirit of \cite{Amstutz2006,Garreau2001}. 
%We notice that the adjoint technique in this compression problem is innovative and not obvious at all. 
We notice that the Dirichlet boundary condition in the inclusion prevents from a direct transposition of the method based on a local perturbation of the material properties by inserting small holes. Therefore, we adapt the sensibility analysis to the problem under consideration and we perform the asymptotic expansion of the proposed shape functional using non-standard perturbation techniques combined with truncation techniques. The asymptotic allows us to deduce a gradient
algorithm for the reconstruction that we implement and compare to previous works \cite{Belhachmi2009, Belhachmi2022Jun}.

The article is organized as follows : in Section \ref{sec:problem-formulation}, we introduce the compression problem that takes the form of a constrained optimization problem of finding the best set of pixels to store, denoted $K$. Section \ref{sec:topological-derivatives} is devoted to describe the adjoint method to compute the topological derivative of the cost functional considered. In Section \ref{sec:summary-numerical}, we perform the computations to obtain the topological expansion and the ``shape'' derivatives which involve the direct and adjoint states. Finally, in Section \ref{sec:numerical-results}, we describe the resulting algorithm and we give some numerical results to confirm the usefulness of the theory.

\section{Problem Formulation}
\label{sec:problem-formulation}

Let $D\subset\R^2$ and $f: D\to\R$, a given image in some region $K\subset\subset D$. We consider the mixed elliptic boundary problem for a  given $u_0$ in $L^2(D)$, \\

\begin{problem} Find $u$ in $H^1(D)$ such that
	\begin{equation}
		\left\{\begin{array}{rl}
			u - \alpha \Delta u = u_0, & \text{in}\ D\setminus K, \\
			u = f, & \text{in}\ K, \\
			\frac{\partial u}{\partial \mathbf{n}} = 0, & \text{on}\ \partial D. \\
		\end{array}\right .\label{eq:problem_1}
	\end{equation}
	\label{pb:problem_1}
\end{problem}
where the available data $f$ is a Dirichlet ``boundary'' condition and with homogeneous Neumann boundary condition on $\partial D$. This PDE corresponds to the first term in the time discretization of the homogeneous heat equation, where we assume that the initial condition is $u_0$. For compatibility condition with the ``boundary'' data on $K$, we take as $u_0$ the image $f\in H^1(D)$, with $\Delta f\in L^2(D)$ and such that $\frac{\partial f}{\partial n}=0$ on $\partial D$.
In the compression step (coding phase), the datum $f$ is available in the entire domain $D$, so we can set the initial condition $u_0$ to the function $f$. The result of this coding step consists of a set $K$ of the pixels to store and the values of $f$ on $K$. In the decompression step (decoding phase), the data is only available in the subset $K$ of the domain, so we set $u_0=0$ (at least in $D\setminus K$). When the reconstruction is performed by solving the heat equation, it means that we start with an initial datum which do not satisfy the compatibility conditions, but 
this does not influence the dynamic as far as the convergence to an equilibrium, that is a steady state, holds (regularizing effect).
Setting $v=u-f$, we can write equivalently \\

\begin{problem} Find $v$ in $H^1(D)$ such that
	\begin{equation}
		\left\{\begin{array}{rl}
			- \alpha \Delta v + v = \alpha \Delta f, & \text{in}\ D\setminus K, \\
			v = 0, & \text{in}\ K, \\
			\frac{\partial v}{\partial \mathbf{n}} = 0, & \text{on}\ \partial D. \\
		\end{array}\right .\label{eq:problem_1:v}
	\end{equation}
	\label{pb:problem_1:v}
\end{problem}
Denoting by $v_K=u_K-f$ the solution of Problem \ref{pb:problem_1:v}, the question is to identify the region $K$ which gives the “best” approximation $u_K$, in a suitable sense, that is to say which minimizes some $L^p$-norm. The constrained optimization problem for the compression reads \cite{Belhachmi2009}, for $1\leq p < +\infty$,
\begin{equation}\label{eq1}
	\min_{K\subseteq D,\ m(K)\leq c}\Big\{  \frac{1}{p}\int_D |u_K-f|^p\ dx\ \Big|\ u_K\ \text{solution of Problem}\ \ref{pb:problem_1} \Big\},
\end{equation}
where $m$ is a ``size measure". The optimization problem \eqref{eq1} is studied in \cite{Belhachmi2009} and the existence of an optimal set is established for $p=2$ and $m$ is the capacity of sets \cite{Ziemer1969} and the result extends to $1\leq p < +\infty$ as noticed in \cite{Belhachmi2022Jun}. The optimal set $K$ is obtained via a relaxation procedure but its regularity is not considered yet, nevertheless the relaxation technique allows us to derive first order optimality conditions via topological derivatives, which was done in the case of the Laplacian as inpainting operator. In this article, we aim to compute the topological gradient \cite{Cea1973, Amstutz2006} of the shape functional using the adjoint method which possesses two main advantages on the previous approaches: it is more general and systematic with respect to the inpainting operator and the exponent $1\leq p < +\infty$, on one side and secondly, it leads to a better characterization of the relevant pixels as it gives a distribution of such pixels taking into account local information from their neighborhood. Loosely speaking, to obtain the topological derivative, let $x_0\in D$ and $K_\varepsilon=K\cup \overline{B(x_0,\varepsilon)}$ ($B(x_0,\epsilon)$ denotes the ball centered at $x_0$ with radius $\varepsilon$), then we look for an expansion of the form
\[ J(u_{K_\varepsilon}) - J(u_K) = \rho(\varepsilon)\,G(x_0) + o\big( \rho(\varepsilon) \big). \]
where $\rho$ is a positive function going to zero with $\varepsilon$ and $G$ is the so-called topological
gradient \cite{Amstutz2006, Belhachmi2018, Garreau2001}. Therefore, to minimize the cost functional $J$, one has to create small holes
at the locations $x\in D$ where $G(x)$ is the most negative. For the compression problem this amounts to select the locations where the pixels are the most important to keep.

\section{Adjoint Method and Variations of the Cost Functional}
\label{sec:topological-derivatives}

The adjoint method has been extensively studied and successfully applied to many second order elliptic problems and Helmholtz equation (see \cite{Amstutz2006,Garreau2001} and references therein). We will recall the main principle (theorem) of the method and apply it to our specific setting. 
We introduce the following abstract result which describes the adjoint method for the computation of the first variation of a given cost functional (see for instance \cite{Amstutz2006}). Let $V$ be a Hilbert space. For $\varepsilon\in [0,\zeta]$, $\zeta> 0$, we consider a symmetric bilinear form $a_\varepsilon: V\times V\to \R$ and a linear form $l_\varepsilon: V\to \R$ such that the following assumptions are fulfilled 
\begin{itemize}
    \item $|a_\varepsilon(v,w)| \leq M_1\|v\|\|w\|$, $\forall (v,w)\in V\times V$ (\textbf{continuity of the bilinear form}),
    \item $a_\varepsilon(v,v) \geq \xi\|v\|^2$, $\forall v\in V$ (\textbf{uniform coercivity}),
    \item $|l_\varepsilon(w)| \leq M_2\|w\|$, $\forall w\in V$ (\textbf{continuity of the linear form}),
\end{itemize}
with $\alpha,M_1,M_2>0$ independent of $\varepsilon$. Moreover, we suppose that there exists a continuous bilinear form $\delta a: V\times V\to \R$, a continuous linear form $\delta l: V\to \R$ and a function $\rho: \R_+\to \R_+$ such that, for all $\varepsilon\geq 0$,
\begin{itemize}
    \item $\|a_\varepsilon-a_0-\rho(\varepsilon)\,\delta a\|_{\mathcal{L}_2(V)} = o\big(\rho(\varepsilon)\big)$,
    \item $\|l_\varepsilon-l_0-\rho(\varepsilon)\, \delta l\|_{\mathcal{L}(V)} = o\big(\rho(\varepsilon)\big)$,
    \item $\lim_{\varepsilon\to 0} \rho(\varepsilon) = 0$.
\end{itemize}
We emphasize that $\delta a$ and $\delta l$ do not depend on $\varepsilon$. Finally, for all $\varepsilon\in [0,\zeta]$, consider a functional $J_\varepsilon:V\to \R$, Fr\'echet-differentiable at the point $v_0$. Assume further that there exists a number $\delta J(v_0)$ such that
%be a We suppose that $J_0$ is differentiable on $V$ and that there is a function $\delta J: V\to \R$ such that, 
\[ J_\varepsilon(w) - J_0(v) = DJ_0(v)(w-v) + \rho(\varepsilon)\,\delta J(v) + o\big(\|w-v\|+\rho(\varepsilon)\big),\ \forall (v,w)\in V\times V. \]
Then we have \cite{Amstutz2006} \\
%Again, $\delta J$ do not depend $\varepsilon$. Then we have the adjoint method, \\

\begin{theorem}\label{thm1} Let $v_\varepsilon \in V$ be the solution of the following problem : find $v\in V$ such that,
    \[ a_\varepsilon(v,\varphi) = l_\varepsilon(\varphi),\ \forall \varphi\in V. \]
    Let $w_0$ be the solution of the so-called adjoint problem : find $w\in V$ such that
    \[ a_0(w,\varphi) = - DJ_0(v_0)\varphi, \ \forall\varphi\in V. \]
    Then,
    \[ J_\varepsilon(v_\varepsilon) - J_0(v_0) = \rho(\varepsilon)\big(\delta a(v_0,w_0) - \delta l(w_0) + \delta J(v_0)\big) + o\big(\rho(\varepsilon)\big). \]
    \label{thm:adjoint-method}
\end{theorem}
%Since the $L^p$ norm do not satisfies properties that we will discuss below, we take as cost function,
%\[ \tilde{J}_\varepsilon(v) := \int_{D\setminus B_\varepsilon} g(x,v(x))\ dx,\ \forall v\in V_\varepsilon, \]
%and $g$ such that :
%\begin{itemize}
%    \item[(H1)] for all $x\in$ D, $s\mapsto g(x,s)$ is $\mathcal{C}^1(R)$ and we denote its derivative by $g_s$,
%    \item[(H2)] for all $x\in$ D, $s\mapsto g_s(x,s)$ is $M$-Lipschitz continuous,
%    \item[(H3)] $x\mapsto g_s(x,0)$ is in $L^2(D)$ and $x\mapsto g(x,0)$ is in $L^p(D)$, $p>1$.
%\end{itemize}
%
%We have then \cite{Guillaume2002}, \\
%
%\begin{proposition}
%    For all $(x,s,t)\in D\times\R\times\R$, we have
    % \begin{itemize}
    %     \item ?$|g(x,s)| \leq |g(x,0)| + |g_s(x,0)\,s| + \frac{M}{2}s^2$,
    %     \item ?$|g_s(x,s)| \leq |g_s(x,0)| + M\, |s|$,
    %     \item $g(x,t) - g(x,s) \leq g_s(x,s)(t-s) + \theta(x,s,t)(t-s)^2$, with $|\theta(x,s,t)|\leq \frac{M}{2}$.
    % \end{itemize}
 %   \[ g(x,t) - g(x,s) \leq g_s(x,s)(t-s) + \theta(x,s,t)(t-s)^2, \] with $|\theta(x,s,t)|\leq \frac{M}{2}$.
%    \label{prop:g}
%\end{proposition}
%
%The paper is organized as follow : in Section \ref{sec:model} we formulate the compression problem as a shape optimization one, and reformulate it to handle the adjoint method. In Section \ref{sec:adjoint} we give the adjoint problem. In Section \ref{sec:variations} we compute the asymptotic development of the functional's variations. Finally, in Section \ref{sec:summary-numerical}, we give a recap of the results and present some numerical experiments to confirm the usefulness of the theory. Some of the proofs and intermediate results are given in Appendix \ref{appendix:norms}, \ref{appendix:properties-proofs}, \ref{appendix:estimates} and \ref{appendix:exterior-pb}.

==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/maths.tex <==
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}

\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\esssup}{ess\ sup}
\DeclareMathOperator{\essinf}{ess\ inf}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\supp}{Supp}
\DeclareMathOperator{\capop}{cap}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\cl}{cl}

\def\restriction#1#2{\mathchoice
              {\setbox1\hbox{${\displaystyle #1}_{\scriptstyle #2}$}
              \restrictionaux{#1}{#2}}
              {\setbox1\hbox{${\textstyle #1}_{\scriptstyle #2}$}
              \restrictionaux{#1}{#2}}
              {\setbox1\hbox{${\scriptstyle #1}_{\scriptscriptstyle #2}$}
              \restrictionaux{#1}{#2}}
              {\setbox1\hbox{${\scriptscriptstyle #1}_{\scriptscriptstyle #2}$}
              \restrictionaux{#1}{#2}}}
\def\restrictionaux#1#2{{#1\,\smash{\vrule height .8\ht1 depth .85\dp1}}_{\,#2}}


\mdfdefinestyle{thm}{
	nobreak=true,
	hidealllines=true,
	leftline=true,
	innerleftmargin=10pt,
	innerrightmargin=10pt,
	innertopmargin=0pt,
}

\newtheorem{definition}{Definition}[section]\surroundwithmdframed[style=thm]{definition}
\newtheorem{proposition}{Proposition}[section]\surroundwithmdframed[style=thm]{proposition}
\newtheorem{theorem}{Theorem}[section]\surroundwithmdframed[style=thm]{theorem}
\newtheorem{lemma}{Lemma}[section]\surroundwithmdframed[style=thm]{lemma}
\newtheorem{property}{Property}[section]\surroundwithmdframed[style=thm]{property}
\newtheorem{problem}{Problem}[section]\surroundwithmdframed[style=thm]{problem}
\newtheorem*{problem*}{Problem}\surroundwithmdframed[style=thm]{problem*}

\theoremstyle{remark}
\newtheorem*{notations}{\textbf{Notations}}
\newtheorem*{note}{\textbf{Remark}}

==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/section01.tex <==
%\section{The Analytic Model}
%\label{sec:model}

%Going back to our initial problem, we start from $K=\emptyset$ and we seek for a set $K_\varepsilon := K\cup 

To be more specific, for $x_0\in D$ and $r>0$, we denote by $B_r$ the open ball centred at $x_0$ and of radius $r$.
%for a given $K$ : \\
% \begin{problem} Find $u_D$ in $H^1(D)$ such that
% 	\begin{equation}
% 		\left \{ \begin{array}{cc}
%             -\alpha\Delta u_D + u_D = f, & \text{in}\ D, \\
%             \partial_n u_D = 0, & \text{on}\ \partial D.
%         \end{array}
%         \right .\label{eq:problem:u-D}
% 	\end{equation}
% 	\label{pb:problem:u-D}
% \end{problem}
% We set $v_D := u_D - f$ and we have \\
We set 
$$V_\varepsilon :=  \{ v\in H^1(D\setminus B_\varepsilon)\ |\ v=0\ \text{on}\ \partial B_\varepsilon \}.$$
Then we consider the boundary value problem: \\
\begin{problem} Find $\widetilde{v}_\varepsilon$ in $V_\varepsilon$ such that
	\begin{equation}
    	\left \{ \begin{array}{cl}
            -\alpha\Delta \widetilde{v}_\varepsilon + \widetilde{v}_\varepsilon = h, & \text{in}\ D\setminus B_\varepsilon, \\
            \widetilde{v}_\varepsilon = 0, & \text{in}\ B_\varepsilon, \\
            \partial_n \widetilde{v}_\varepsilon = 0, & \text{on}\ \partial D.
        \end{array}
        \right .\label{eq:problem:u-D}
	\end{equation}
	\label{pb:problem:u-D}
\end{problem}
with $h:= \alpha\Delta f$, but $h$ can be any $L^2(D)$ function. We denote $\widetilde{v}_0$ the solution of the problem \\
\begin{problem} Find $\widetilde{v}_0$ in $H^1(D)$ such that
	\begin{equation}
		\left \{ \begin{array}{cl}
            -\alpha\Delta \widetilde{v}_0 + \widetilde{v}_0 = h, & \text{in}\ D, \\
            \partial_n \widetilde{v}_0 = 0, & \text{on}\ \partial D.
        \end{array}
        \right .\label{eq:problem:v-D}
	\end{equation}
	\label{pb:problem:v-D}
\end{problem}
The weak formulation of problems above reads, find $\widetilde{v}_\varepsilon$ in $V_\varepsilon$ such that, for all $\varphi$ in $V_\varepsilon\cap H^1(D)$, we have
\[ \tilde{a}_\varepsilon(\widetilde{v}_\varepsilon, \varphi) = \tilde{l}_\varepsilon(\varphi), \]
with,
\begin{align*}
    & \tilde{a}_\varepsilon(\widetilde{v}_\varepsilon, \varphi) := \alpha\int_{D\setminus B_\varepsilon} \nabla \widetilde{v}_\varepsilon\cdot\nabla\varphi\ dx + \int_{D\setminus B_\varepsilon} \widetilde{v}_\varepsilon\,\varphi\ dx, \\
    %
    & \tilde{l}_\varepsilon(\varphi) := \int_{D\setminus B_\varepsilon} h\,\varphi\ dx.
\end{align*}
%Also, we set $V_\varepsilon :=  \{ v\in H^1(D\setminus B_\varepsilon)\ |\ v=0\ \text{on}\ \partial B_\varepsilon \}$ and we denote by $v_{D_\varepsilon}$ the solution of the following problem : \\

%\begin{problem} Find $v_{D_\varepsilon}$ in $V_\varepsilon$ such that
%	\begin{equation}
%    	\left \{ \begin{array}{cc}
%            -\alpha\Delta v_{D_\varepsilon} + v_{D_\varepsilon} = \alpha\Delta f, & \text{in}\ D\setminus B_\varepsilon, \\
%            v_{D_\varepsilon} = 0, & \text{in}\ B_\varepsilon, \\
%            \partial_n v_{D_\varepsilon} = 0, & \text{on}\ \partial D.
%        \end{array}
%        \right .\label{eq:problem:u-D}
%	\end{equation}
%	\label{pb:problem:u-D}
%\end{problem}
%Since the $L^p$ norm do not satisfies properties that we will discuss below, we take as cost function,
%\[ \widetilde{J_\varepsilon}(v) := \int_{D\setminus B_\varepsilon} g(x,v(x))\ dx,\ \forall v\in V_\varepsilon, \]
%and $g$ such that :
%\begin{itemize}
 %   \item[(H1)] for all $x\in$ D, $s\mapsto g(x,s)$ is $\mathcal{C}^1(R)$ and we denote its derivative by $g_s$,
%    \item[(H2)] for all $x\in$ D, $s\mapsto g_s(x,s)$ is $M$-Lipschitz continuous,
%    \item[(H3)] $x\mapsto g_s(x,0)$ is in $L^2(D)$ and $x\mapsto g(x,0)$ is in $L^p(D)$, $p>1$.
%\end{itemize}
%
%We have then \cite{Guillaume2002}, \\
%
%\begin{proposition}
 %   For all $(x,s,t)\in D\times\R\times\R$, we have
    % \begin{itemize}
    %     \item ?$|g(x,s)| \leq |g(x,0)| + |g_s(x,0)\,s| + \frac{M}{2}s^2$,
    %     \item ?$|g_s(x,s)| \leq |g_s(x,0)| + M\, |s|$,
    %     \item $g(x,t) - g(x,s) \leq g_s(x,s)(t-s) + \theta(x,s,t)(t-s)^2$, with $|\theta(x,s,t)|\leq \frac{M}{2}$.
    % \end{itemize}
%    \[ g(x,t) - g(x,s) \leq g_s(x,s)(t-s) + \theta(x,s,t)(t-s)^2, \] with $|\theta(x,s,t)|\leq \frac{M}{2}$.
%    \label{prop:g}
%\end{proposition}
The dependency of the space $V_\varepsilon$ on $\varepsilon$ prevents us from using Theorem \ref{thm1} directly, therefore, we introduce a  truncation technique \cite{Guillaume2002}, which consists of 
% On pose pour $v,\varphi\in V_0 := H^1(D)$,
% \begin{align*}
%     & \tilde{J}_0(v) := \frac{1}{p}\int_D |v|^p\ dx, \\
%     %
%     & \tilde{a_0}(v,\varphi) := \alpha\int_D\nabla v\cdot\nabla \varphi\ dx + \int_D v\,\varphi\ dx, \\
%     %
%     & \tilde{l_0}(\varphi) := \int_D (\alpha\Delta f)\,\varphi\ dx.
% \end{align*}
% et pour $v,\varphi\in V_\varepsilon := \{ v\in H^1(D\setminus B_\varepsilon)\ |\ v=0\ \text{sur}\ \partial B_\varepsilon \}$, $\varepsilon>0$,
% \begin{align*}
%     & \widetilde{J_\varepsilon}(v) := \frac{1}{p}\int_{D\setminus B_\varepsilon} |v|^p\ dx, \\
%     %
%     & \tilde{a_\varepsilon}(v,\varphi) := \alpha\int_{D\setminus B_\varepsilon}\nabla v\cdot\nabla \varphi\ dx + \int_{D\setminus B_\varepsilon} v\,\varphi\ dx, \\
%     %
%     & \tilde{l_\varepsilon}(\varphi) := \int_{D\setminus B_\varepsilon} (\alpha\Delta f)\,\varphi\ dx.
% \end{align*}
% Problème, notre espace de travail $V_\varepsilon$ dépend de $\varepsilon$ : pas bon.
inserting a ball $B_R$, for a fixed $R>\varepsilon$ and splitting Problem \ref{pb:problem:u-D} into two sub-problems that we glue at their common boundary (see Figure \ref{fig:domain-split}). More precisely, we consider the sub-problems: an \textit{internal} problem
\[ \left \{ \begin{array}{cl}
    -\alpha\Delta v_{\varepsilon,R} + v_{\varepsilon,R} = h, & \text{in}\ B_R\setminus B_\varepsilon, \\
    v_{\varepsilon,R} = 0, & \text{on}\ \partial B_\varepsilon, \\
    v_{\varepsilon,R} = v_\varepsilon, & \text{on}\ \partial B_R,
\end{array} \right .\]
% and if $\varepsilon=0$,
% \[ \left \{ \begin{array}{cc}
%     -\alpha\Delta v_0^{\alpha\Delta f,v_0} + v_0^{\alpha\Delta f,v_0} = \alpha\Delta f, & \text{in}\ B_R, \\
%     v_0^{\alpha\Delta f,v_0} = v_0, & \text{on}\ \partial B_R.
% \end{array}
% \right .\]
and an \textit{external} problem
\[ \left \{ \begin{array}{cl}
    -\alpha\Delta v_\varepsilon + v_\varepsilon = h, & \text{in}\ D\setminus B_R, \\
    \partial_n v_\varepsilon = \partial_n v_{\varepsilon,R}, & \text{on}\ \partial B_R, \\
    \partial_n v_\varepsilon = 0, & \text{on}\ \partial D.
\end{array}
\right .\]

\begin{figure}[H]
    \centering
    \subfloat[Before splitting.]{
        \begin{tikzpicture}[scale=0.35]
            % \draw [help lines] (-17, 20) grid (8, -5);
            
            \draw[fill=black!10] % , show curve controls
                (-6.75, 15) .. controls + (-1,-0.5) and + (1,1.5) ..
                (-12.5, 10.75) .. controls + (-1,-1.5) and + (-0.5,1.5) ..
                (-13.25, 0) .. controls + (0.5,-1.5) and + (-3,-1) ..
                (-5, 4.75) .. controls + (3,1) and + (1,-2) ..
                (5, 7.25) .. controls + (-1,2) and + (2,-1) ..
                (-2.75, 14.75) .. controls + (-2,1) and + (1,0.5) ..
                (-6.75, 15) -- cycle;
                
            \node (6) at (-11,3.5) {$D\setminus B_\varepsilon$};
                
        	\node[circle, draw=black, fill=white, inner sep=0pt,minimum size=25pt] (1) at (-5,10) {$B_\varepsilon$};
        	
        	\draw[->] (-13,14) -- (-10,10);
        	
        	\node (3) at (-13.5,14.5) {$\widetilde{v}_\varepsilon$};
        \end{tikzpicture}
    }
	\qquad
	\subfloat[After splitting.]{
        \begin{tikzpicture}[scale=0.35]
            % \draw [help lines] (-17, 20) grid (8, -5);
            
            \draw[fill=black!10] % , show curve controls
                (-6.75, 15) .. controls + (-1,-0.5) and + (1,1.5) ..
                (-12.5, 10.75) .. controls + (-1,-1.5) and + (-0.5,1.5) ..
                (-13.25, 0) .. controls + (0.5,-1.5) and + (-3,-1) ..
                (-5, 4.75) .. controls + (3,1) and + (1,-2) ..
                (5, 7.25) .. controls + (-1,2) and + (2,-1) ..
                (-2.75, 14.75) .. controls + (-2,1) and + (1,0.5) ..
                (-6.75, 15) -- cycle;
            
            \node (6) at (-11,3.5) {$D\setminus B_R$};
                
            \node[circle, dashed, draw=black, fill=black!25, inner sep=0pt,minimum size=70pt] (1) at (-5,10) {};
        	\node (6) at (-5,7.8) {$B_R\setminus B_\varepsilon$};
        	\node[circle, draw=black, fill=white, inner sep=0pt,minimum size=25pt] (2) at (-5,10) {$B_\varepsilon$};
        	
        	\draw[->] (-13,14) -- (-10,10);
        	\node (3) at (-13.5,14.5) {$v_\varepsilon$};
        	\draw[->] (1,14) -- (-2.8,11);
        	\node (3) at (1.5,14.5) {$v_{\varepsilon,R}$};
        \end{tikzpicture}
    }
    \caption{Illustration of the splitting.}
	\label{fig:domain-split}
\end{figure}

% \begin{figure}[H]
% 	\centering
% 	\subfloat[.]{
% 		\includegraphics[width=3.6cm]{images/K_R.png}
% 	}
% 	\quad
% 	\subfloat[.]{
% 		\includegraphics[width=3.6cm]{images/v_R.png}
% 	}
% 	\quad
% 	\subfloat[.]{
% 		\includegraphics[width=3.6cm]{images/v_epsilon.png}
% 	}
% 	\caption{Illustration of the splitting of the problem.}
% 	\label{fig:domain-split}
% \end{figure}

As the two sub-problems transform the initial one into a transmission problem. Then, \\
%% pas besoin de cette appendice
%the following property, proved in Appendix \ref{appendix:properties-proofs}, \\

\begin{proposition} We have,
    \[ \widetilde{v}_\varepsilon = \begin{cases} 
        v_\varepsilon, & \text{in}\ D\setminus B_R, \\
        v_{\varepsilon,R}, & \text{in}\ B_R\setminus B_\varepsilon.
    \end{cases} \]
    \label{prop:gluing-solutions}
\end{proposition}
\begin{proof}
    We set \begin{equation} v := \begin{cases} 
        v_\varepsilon, &  \text{in}\ D\setminus B_R, \\
        v_{\varepsilon,R}, & \text{in}\ B_R\setminus B_\varepsilon.
    \end{cases} \label{eq:gluing-solutions}\end{equation}
    Let $\varphi$ be in $V_\varepsilon$, then,
    \begin{align*}
        \tilde{a}_\varepsilon(v, \varphi) & = \alpha\int_{D\setminus B_R} \nabla v\cdot\nabla\varphi\ dx + \int_{D\setminus B_R} v\,\varphi\ dx + \alpha\int_{B_R\setminus B_\varepsilon} \nabla v\cdot\nabla\varphi\ dx + \int_{B_R\setminus B_\varepsilon} v\,\varphi\ dx \\
        %
        % & = \alpha\int_{D\setminus B_R} \nabla v_\varepsilon\cdot\nabla\varphi\ dx + \int_{D\setminus B_R} v_\varepsilon\,\varphi\ dx + \alpha\int_{B_R\setminus B_\varepsilon} \nabla v_{\varepsilon,R}\cdot\nabla\varphi\ dx + \int_{B_R\setminus B_\varepsilon} v_{\varepsilon,R}\,\varphi\ dx \\
        %
    \end{align*}
    Replacing $v$ by its expression \eqref{eq:gluing-solutions} and integrating by parts yields,
    \begin{align*}
        % & = -\alpha\int_{D\setminus B_R} \Delta v_\varepsilon\,\varphi\ dx + \alpha \underbrace{\int_{\partial D} \partial_{n_\text{ext}} v_\varepsilon\,\varphi\ d\sigma}_{=0} + \alpha\int_{\partial B_R} \partial_{n_\text{int}} v_\varepsilon\,\varphi\ d\sigma + \int_{D\setminus B_R} v_\varepsilon\,\varphi\ dx \\ & \hspace{2cm} - \alpha\int_{B_R\setminus B_\varepsilon} \Delta v_{\varepsilon,R}\,\varphi\ dx + \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_{\varepsilon,R}\,\varphi\ d\sigma + \alpha\underbrace{\int_{\partial B_\varepsilon} \partial_{n_\text{int}} v_{\varepsilon,R}\,\varphi\ d\sigma}_{=0\ \text{since}\ \varphi\in V_\varepsilon} \\ & \hspace{2cm} + \int_{B_R\setminus B_\varepsilon} v_{\varepsilon,R}\,\varphi\ dx \\
        %
        \tilde{a}_\varepsilon(v, \varphi) & = \int_{D\setminus B_R} (-\alpha\Delta v_\varepsilon + v_\varepsilon)\,\varphi\ dx + \int_{B_R\setminus B_\varepsilon} (-\alpha\Delta v_{\varepsilon,R} + v_{\varepsilon,R})\,\varphi\ dx \\ & \hspace{2cm} + \alpha\int_{\partial B_R} \partial_{n_\text{int}} v_\varepsilon\,\varphi\ d\sigma + \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_{\varepsilon,R}\,\varphi\ d\sigma \\
        %
        % & = \int_{D\setminus B_\varepsilon} h\,\varphi\ dx + \alpha\int_{\partial B_R} \partial_{n_\text{int}} v_\varepsilon\,\varphi\ d\sigma + \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_{\varepsilon,R}\,\varphi\ d\sigma \\
        %
        % & = \int_{D\setminus B_\varepsilon} h\,\varphi\ dx - \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_{\varepsilon,R}\,\varphi\ d\sigma + \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_{\varepsilon,R}\,\varphi\ d\sigma \\
        %
        & = \int_{D\setminus B_\varepsilon} h\,\varphi\ dx = \tilde{l}_\varepsilon(\varphi).
    \end{align*}
    By the uniqueness of the solution of Problem \ref{pb:problem:u-D}, we have $v=\widetilde{v}_\varepsilon$.
\end{proof}
% \begin{proof}
%     On pose \[ v := \begin{cases} 
%         v_\varepsilon & ,\ \text{dans}\ D\setminus B_R, \\
%         v_\varepsilon^{\alpha\Delta f,v_\varepsilon} & ,\ \text{dans}\ B_R\setminus B_\varepsilon.
%     \end{cases} \]
%     Soit $\varphi\in V_\varepsilon$, alors,
%     \begin{align*}
%         \tilde{a}_\varepsilon(v, \varphi) & := \alpha\int_{D\setminus B_\varepsilon} \nabla v\cdot\nabla\varphi\ dx + \int_{D\setminus B_\varepsilon} v\,\varphi\ dx \\
%         %
%         & = \alpha\int_{D\setminus B_R} \nabla v\cdot\nabla\varphi\ dx + \int_{D\setminus B_R} v\,\varphi\ dx + \alpha\int_{B_R\setminus B_\varepsilon} \nabla v\cdot\nabla\varphi\ dx + \int_{B_R\setminus B_\varepsilon} v\,\varphi\ dx \\
%         %
%         & = \alpha\int_{D\setminus B_R} \nabla v_\varepsilon\cdot\nabla\varphi\ dx + \int_{D\setminus B_R} v_\varepsilon\,\varphi\ dx + \alpha\int_{B_R\setminus B_\varepsilon} \nabla v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\cdot\nabla\varphi\ dx + \int_{B_R\setminus B_\varepsilon} v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\,\varphi\ dx \\
%         %
%         & = -\alpha\int_{D\setminus B_R} \Delta v_\varepsilon\,\varphi\ dx + \alpha \underbrace{\int_{\partial D} \partial_{n_\text{ext}} v_\varepsilon\,\varphi\ d\sigma}_{=0} + \alpha\int_{\partial B_R} \partial_{n_\text{int}} v_\varepsilon\,\varphi\ d\sigma + \int_{D\setminus B_R} v_\varepsilon\,\varphi\ dx \\ & \hspace{2cm} - \alpha\int_{B_R\setminus B_\varepsilon} \Delta v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\,\varphi\ dx + \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\,\varphi\ d\sigma + \alpha\underbrace{\int_{\partial B_\varepsilon} \partial_{n_\text{int}} v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\,\varphi\ d\sigma}_{=0\ \text{car}\ \varphi\in V_\varepsilon} \\ & \hspace{2cm} + \int_{B_R\setminus B_\varepsilon} v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\,\varphi\ dx \\
%         %
%         & = \int_{D\setminus B_R} (-\alpha\Delta v_\varepsilon + v_\varepsilon)\,\varphi\ dx + \int_{B_R\setminus B_\varepsilon} (-\alpha\Delta v_\varepsilon^{\alpha\Delta f,v_\varepsilon} + v_\varepsilon^{\alpha\Delta f,v_\varepsilon})\,\varphi\ dx \\ & \hspace{2cm} + \alpha\int_{\partial B_R} \partial_{n_\text{int}} v_\varepsilon\,\varphi\ d\sigma + \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\,\varphi\ d\sigma \\
%         %
%         & = \int_{D\setminus B_\varepsilon} \alpha\Delta f\,\varphi\ dx + \alpha\int_{\partial B_R} \partial_{n_\text{int}} v_\varepsilon\,\varphi\ d\sigma + \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\,\varphi\ d\sigma \\
%          %
%         & = \int_{D\setminus B_\varepsilon} \alpha\Delta f\,\varphi\ dx - \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\,\varphi\ d\sigma + \alpha\int_{\partial B_R} \partial_{n_\text{ext}} v_\varepsilon^{\alpha\Delta f,v_\varepsilon}\,\varphi\ d\sigma \\
%         %
%         & = \int_{D\setminus B_\varepsilon} \alpha\Delta f\,\varphi\ dx = \tilde{l}_0(\varphi).
%     \end{align*}
%     Par unicité de la solution $v=v_{D_\varepsilon}$.
% \end{proof}

For the \textit{internal} problem, we introduce the notation $v_\varepsilon^{h,\phi}$ instead of $v_{\epsilon, R}$, the solution of the more general problem \\

\begin{problem} Find $v_\varepsilon^{h,\phi}$ in $\{ v\in H^1(B_R\setminus B_\varepsilon)\ |\ v=0\ \text{on}\ \partial B_\varepsilon \}$ such that
	\begin{equation}
    	\left \{ \begin{array}{cl}
            -\alpha\Delta v_\varepsilon^{h,\phi} + v_\varepsilon^{h,\phi} = h, & \text{in}\ B_R\setminus B_\varepsilon, \\
            v_\varepsilon^{h,\phi} = 0, & \text{on}\ \partial B_\varepsilon, \\
            v_\varepsilon^{h,\phi} = \phi, & \text{on}\ \partial B_R.
        \end{array}
        \right .\label{eq:problem:v-epsilon-inside}
	\end{equation}
	\label{pb:problem:v-epsilon-inside}
\end{problem}
% et si $\varepsilon=0$,
% \[ \left \{ \begin{array}{cc}
%     -\alpha\Delta v_0^{g,\phi} + v_0^{g,\phi} = g, & \text{dans}\ B_R, \\
%     v_0^{g,\phi} = \phi, & \text{sur}\ \partial B_R.
% \end{array}
% \right .\]
Therefore, $v_{\varepsilon,R} = v_\varepsilon^{h,\phi}$, when $\phi=v_\varepsilon$. We also notice that,
\[ v_\varepsilon^{h,\phi} = v_\varepsilon^{h,0} + v_\varepsilon^{0,\phi}. \]
We remind the Dirichlet-to-Neumann operator $T_\varepsilon : H^{1/2}(\partial B_R) \to H^{-1/2}(\partial B_R)$ by 
\[ T_\varepsilon(\phi) := \nabla v_\varepsilon^{0,\phi}\cdot n. \]
and we set \[ h_\varepsilon := -\nabla v_\varepsilon^{h,0}\cdot n\in H^{-1/2}(\partial B_R). \]
Hence, setting $V_R=H^1(D\setminus B_R)$, we can rewrite the \textit{external} problem using this operator as following (we still denote by $v_\varepsilon$ the solution): \\

\begin{problem} Find $v_\varepsilon$ in $V_R$ such that
	\begin{equation}
    	\left \{ \begin{array}{cl}
            -\alpha\Delta v_\varepsilon + v_\varepsilon = h, & \text{in}\ D\setminus B_R, \\
            -\partial_n v_\varepsilon + T_\varepsilon v_\varepsilon = h_\varepsilon, & \text{on}\ \partial B_R, \\
            \partial_n v_\varepsilon = 0, & \text{on}\ \partial D.
        \end{array}
        \right .\label{eq:problem:v-epsilon-outside}
	\end{equation}
	\label{pb:problem:v-epsilon-outside}
\end{problem}


% \begin{align*}
%     & \alpha\int_{D\setminus B_R}\nabla v_\varepsilon\cdot\nabla \varphi\ dx + \alpha\int_{\partial B_R} \partial_n v_\varepsilon \varphi\ d\sigma + \int_{D\setminus B_R}v_\varepsilon\varphi\ dx = \int_{D\setminus B_R}\alpha\Delta f\varphi\ dx \\
%     %
%     \Leftrightarrow\hspace{0.5cm} & \alpha\int_{D\setminus B_R}\nabla v_\varepsilon\cdot\nabla \varphi\ dx + \alpha\int_{\partial B_R} (T_\varepsilon v_\varepsilon - g_\varepsilon)\varphi\ d\sigma + \int_{D\setminus B_R}v_\varepsilon\varphi\ dx = \int_{D\setminus B_R}\alpha\Delta f\varphi\ dx \\
%     %
%     \Leftrightarrow\hspace{0.5cm} & \alpha\int_{D\setminus B_R}\nabla v_\varepsilon\cdot\nabla \varphi\ dx + \alpha\int_{\partial B_R} T_\varepsilon v_\varepsilon\varphi\ d\sigma + \int_{D\setminus B_R}v_\varepsilon\varphi\ dx = \int_{D\setminus B_R}\alpha\Delta f\varphi\ dx + \alpha\int_{\partial B_R} g_\varepsilon \varphi\ d\sigma.
% \end{align*}
For $\varepsilon\in [0,\zeta]$, $R>\zeta$, and $v,\varphi$ in $V_R := H^1(D\setminus B_R)$, we define
\begin{align*}
    & a_\varepsilon(v,\varphi) := \alpha\int_{D\setminus B_R}\nabla v\cdot\nabla \varphi\ dx + \alpha\int_{\partial B_R} T_\varepsilon v\,\varphi\ d\sigma + \int_{D\setminus B_R}v\,\varphi\ dx, \\
    %
    &  l_\varepsilon(\varphi) := \int_{D\setminus B_R} h\,\varphi\ dx + \alpha\int_{\partial B_R} h_\varepsilon\, \varphi\ d\sigma.
\end{align*}
So that the associated variational formulation reads: find $v\in V_R$, such that  
\[ a_\varepsilon(v,\varphi) = l_\varepsilon(\varphi),\qquad\forall \varphi\in V_R. \]
It is easily checked that $a_\varepsilon$ is symmetric and $l_\varepsilon$ is continuous.
%\\
%% PAS BESOIN D'APPENDICE
%We have the following properties, also proved in Appendix \ref{appendix:properties-proofs}, \\
%
%\begin{proposition} We have,
%    \begin{itemize}
 %       \item $a_\varepsilon$ is symmetric,
%        \item $l_\varepsilon$ is continuous.
 %   \end{itemize}
 %   \label{prop:symmetric-continuous}
%\end{proposition}
%
%To define the cost functionals on $V_R$, for $v\in V_R$, we define $v_\varepsilon \in V_\varepsilon$ (the extension of $v$ in $D$) such that,
%\begin{itemize}
%    \item[\textbullet] $v_\varepsilon|_{D\setminus B_R} = v$,
%    \item[\textbullet] $v_\varepsilon|_{B_R\setminus B_\varepsilon} = v_\varepsilon^{g, v}$.
%\end{itemize}
%we set $J_\varepsilon : V_R \to \R_+$ : 
%\[ J_\varepsilon (v) := J_\varepsilon(v_\varepsilon). \]

We take as cost function, for $1\leq p<+\infty$,
\[ \widetilde{J}_\varepsilon(\widetilde{v}) := \int_{D\setminus B_\varepsilon} |h-\widetilde{v}|^p\ dx,\ \forall \widetilde{v}\in V_\varepsilon, \]
\begin{comment}
\color{red}
In the sequel we write the cost functional in a slightly more general form, in particular to cope with the lack of differentiability for $p=1$.
We take as cost function,
\[ \widetilde{J}_\varepsilon(\widetilde{v}) := \int_{D\setminus B_\varepsilon} g(x,\widetilde{v}(x))\ dx,\ \forall \widetilde{v}\in V_\varepsilon, \]
where $g$ is such that :
\begin{itemize}
    \item[(H1)] for all $x\in$ D, $s\mapsto g(x,s)$ is $\mathcal{C}^1(\R)$ and we denote its derivative by $g_s$,
    \item[(H2)] for all $x\in$ D, $s\mapsto g_s(x,s)$ is $M$-Lipschitz continuous,
   \item[(H3)] $x\mapsto g_s(x,0)$ is in $L^2(D)$ and $x\mapsto g(x,0)$ is in $L^p(D)$, $p>1$.
\end{itemize}
%
Under these assumptions, it is readily checked that \\
%
\begin{proposition}
    For all $(x,s,t)\in D\times\R\times\R$, we have
     \begin{itemize}
         \item $|g(x,s)| \leq |g(x,0)| + |g_s(x,0)\,s| + \frac{M}{2}s^2$,
         \item $|g_s(x,s)| \leq |g_s(x,0)| + M\, |s|$,
         \item $g(x,t) - g(x,s) \leq g_s(x,s)(t-s) + \theta(x,s,t)(t-s)^2$, with $|\theta(x,s,t)|\leq \frac{M}{2}$.
     \end{itemize}
    \label{prop:g}
\end{proposition}
\end{comment}

We define now the cost functional on $V_R$ as follows: for $v\in V_R$, we set $\widetilde{v}_\varepsilon \in V_\varepsilon$ the extension of $v$ in $D\setminus B_\varepsilon$ such that,
\begin{itemize}
    \item[\textbullet] $\widetilde{v}_\varepsilon|_{D\setminus B_R} = v$,
    \item[\textbullet] $\widetilde{v}_\varepsilon|_{B_R\setminus B_\varepsilon} = v_\varepsilon^{h,\phi}$, for $\phi=v$ on $\partial B_R$.
\end{itemize}
We notice that $\widetilde{v}_\varepsilon$ do not satisfy Problem \ref{pb:problem:u-D} except if $v$ is the solution of Problem \ref{pb:problem:v-epsilon-outside}. Then, we may define the restriction of $\widetilde{J}_\varepsilon$ to $V_R$ by: 
\[ J_\varepsilon (v) := \widetilde{J}_\varepsilon(\widetilde{v}_\varepsilon),\ \forall v\in V_R. \]

==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/section02.tex <==
\subsection{The Adjoint Problem and Related Estimates}
\label{sec:adjoint}

We state now the adjoint problem associated to Problem \ref{pb:problem:v-epsilon-outside} when $\varepsilon=0$: we denote by $w_0$ the weak solution in $V_R$ of \[ a_0(w_0,\varphi) = -DJ_0(v_0)\,\varphi,\ \forall\varphi\in V_R, \]
where $v_0$ is the solution of Problem \ref{pb:problem:v-epsilon-outside}. The adjoint state $w_0$ is then the solution of \\
\begin{problem} Find $w_0$ in $V_R$ such that
	\begin{equation}
    	\left \{ \begin{array}{cl}
            -\alpha\Delta w_0 + w_0 = -v_0|v_0|^{p-2}, & \text{in}\ D\setminus B_R, \\
            -\partial_n w_0 + T_0 w_0 = h_0, & \text{on}\ \partial B_R, \\
            \partial_n w_0 = 0, & \text{on}\ \partial D.
        \end{array}
        \right .\label{eq:problem:w-epsilon-outside}
	\end{equation}
	\label{pb:problem:w-epsilon-outside}
\end{problem}
%In the next section, we compute the variations required in the adjoint method.
Note that, formally, when $p=1$, the right-hand side of \eqref{eq:problem:w-epsilon-outside} becomes $-\text{sign}(v_0)$.

We aim to find $\delta a$, $\delta l$ and $\delta J$ from the adjoint method, Theorem \ref{thm:adjoint-method}. Let $h\in L^2(D)$ and $\phi\in H^{1/2}(\partial B_R)$. \begin{comment}
\color{red} We consider the solution $v_\omega^{h,\phi}$ of the following \textit{exterior} problem,
\[ \left \{ \begin{array}{cl}
    -\alpha\Delta v_\omega^{h,\phi} + v_\omega^{h,\phi} = 0, & \text{in}\ \R^2\setminus B_1, \\
    v_\omega^{h,\phi} = v_0^{h,\phi}(x_0), & \text{on}\ \partial B_1, \\
    v_\omega^{h,\phi} = 0, & \text{at}\ \infty.
\end{array} \right .\]
Since $v_\omega^{h,\phi}$ is a radial function, we can explicitly compute it : for $x\in \R^2\setminus B_1$,
\[ v_\omega^{h,\phi}(x) = \frac{1}{K_0(\alpha^{-1/2})} \,v_0^{h,\phi}(x_0)\,K_0(\alpha^{-1/2}|x-x_0|), \]
where $K_0$ is the modified Bessel function of the second kind \cite{Oldham2009}. We extend this solution to $\R^2\setminus\{ x_0 \}$ (we still denote by $v_\omega^{h,\phi}$ this extension in the sequel) by setting for $x\in \R^2\setminus\{ x_0 \}$,
\[ v_\omega^{h,\phi}(x) := \frac{1}{K_0(\alpha^{-1/2})} \,v_0^{h,\phi}(x_0)\,K_0(\alpha^{-1/2}|x-x_0|). \] \color{black}
\end{comment}

==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/section03.tex <==
%\section{Variations}
%\label{sec:variations}

\subsection{Variations of the Bilinear Form} 

We start by giving an explicit formulation for both $v_0^{0,\phi}$ and $v_\varepsilon^{0,\phi}$, which is analogous to \cite{Samet2003}, with the following proposition: \\

\begin{proposition} For $\phi$ in $H^{1/2}(\partial B_R)$, we have,
    \[ v_0^{0,\phi} (r, \theta) = \sum_{n\in\mathbb{Z}} \frac{I_n(\alpha^{-1/2}r)}{I_n(\alpha^{-1/2}R)}\,\phi_n\,e^{in\theta}, \]
    and,
    \[ v_\varepsilon^{0,\phi}(r, \theta) = \sum_{n\in\mathbb{Z}} \frac{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}r) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}r)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)}\,\phi_n\,e^{in\theta}, \]
    where $(r,\theta)$ are the polar coordinates in $\R^2$, $(\phi_n)_n$ are the Fourier coefficients of $\phi$, $I_n$ and $K_n$ are the modified Bessel functions of the first and second kind respectively \cite{Abramowitz1972, Oldham2009}.
\end{proposition}
\begin{proof}
    Using polar coordinates in $\R^2$, we have,
    \[ v_\varepsilon^{h,0}(r, \theta) = \sum_{n\in\Z} c_n(r) \,e^{in\theta} \qquad \text{and} \qquad h(r, \theta) = \sum_{n\in\Z} h_n(r) \,e^{in\theta}, \]
    where $c_n$ satisfies, for all $n$ in $\Z$, and $0<r\leq R$,
    \begin{equation*}
        -\alpha\,r^2\,c_n''(r) - \alpha\,r\,c_n'(r) + (r^2+\alpha n^2) c_n(r) = 0.
    \end{equation*}
    We solve the equation, and we get,
    $$ c_{0,n}(r) = A_{0,n} I_n(\alpha^{-1/2}\,r), $$
    and
    $$ c_{\varepsilon,n}(r) = A_{\varepsilon,n} I_n(\alpha^{-1/2}\,r) + B_{\varepsilon,n} K_n(\alpha^{-1/2}\,r). $$
    By using the boundaries conditions, we have the result.
\end{proof}
\begin{note}
    According to \cite{Abramowitz1972,Oldham2009}, we have for all $n$ in $\Z$, $I_{-n} = I_n$ and $K_{-n} = K_n$.
\end{note}

Next, we state the variation of the solution with respect to hole's radius: \\

\begin{proposition} For $\phi$ in $H^{1/2}(\partial B_R)$, we set,
    \[ \delta v^{0,\phi}(r) := -\phi_0\frac{I_0(\alpha^{-1/2}R)K_0(\alpha^{-1/2}r) - K_0(\alpha^{-1/2}R)I_0(\alpha^{-1/2}r)}{I_0(\alpha^{-1/2} R)^2}. \]
    Then, for $\varepsilon$ sufficiently small, we have the following asymptotic estimation,
    \[ v_\varepsilon^{0,\phi}(r, \theta) - v_0^{0,\phi}(r, \theta) - \frac{-1}{\ln{\varepsilon}}\delta v^{0,\phi}(r) = o\left(\frac{-1}{\ln{\varepsilon}}\right). \]
\end{proposition}
\begin{proof} We have,
    \[ v_\varepsilon^{0,\phi}(r, \theta) - v_0^{0,\phi}(r, \theta) = \left( \frac{I_0(\alpha^{-1/2}\varepsilon)K_0(\alpha^{-1/2}r) - K_0(\alpha^{-1/2}\varepsilon)I_0(\alpha^{-1/2}r)}{I_0(\alpha^{-1/2}\varepsilon)K_0(\alpha^{-1/2}R) - K_0(\alpha^{-1/2}\varepsilon)I_0(\alpha^{-1/2}R)} - \frac{I_0(\alpha^{-1/2}r)}{I_0(\alpha^{-1/2}R)} \right)\,\phi_0 + R_\varepsilon(r,\theta), \]
    where, \[ R_\varepsilon(r,\theta) := \sum_{n\in\mathbb{Z}^*} \left( \frac{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}r) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}r)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)} - \frac{I_n(\alpha^{-1/2}r)}{I_n(\alpha^{-1/2}R)} \right)\,\phi_n\,e^{in\theta}. \]
    Then,
    \[ v_\varepsilon^{0,\phi}(r, \theta) - v_0^{0,\phi}(r, \theta) = -\delta v^{0,\phi}(r)\,\frac{I_0(\alpha^{-1/2} R) I_0(\alpha^{-1/2}\varepsilon)}{I_0(\alpha^{-1/2}\varepsilon)K_0(\alpha^{-1/2}R) - K_0(\alpha^{-1/2}\varepsilon)I_0(\alpha^{-1/2}R)} + R_\varepsilon(r,\theta). \]
    We use that, \cite{Abramowitz1972},
    \[ K_0(x) = -(\gamma-\ln{2} + \ln{x}) I_0(x) + x r_1(x), \]
    and get,
    \[ v_\varepsilon^{0,\phi}(r, \theta) - v_0^{0,\phi}(r, \theta) = -\delta v^{0,\phi}(r)\,\left( M + I_0(\alpha^{-1/2}R)\ln{\varepsilon} + \varepsilon r_2(\varepsilon)\right)^{-1} + R_\varepsilon(r,\theta), \]
    where, \[ M := \frac{K_0(\alpha^{-1/2}R) + I_0(\alpha^{-1/2}R)\big(\gamma-\ln{2} + \ln{(\alpha^{-1/2})} \big)}{I_0(\alpha^{-1/2} R)}, \]
    is a constant independent of $\varepsilon$. Finally,
    \[ v_\varepsilon^{0,\phi}(r, \theta) - v_0^{0,\phi}(r, \theta) = -\delta v^{0,\phi}(r)\,\frac{-1}{\ln{\varepsilon}}\left( 1 + \frac{M}{\ln{\varepsilon}} + \varepsilon r_3(\varepsilon)\right)^{-1} + R_\varepsilon(r,\theta). \]
    
    It remains to show that $R_\varepsilon(r,\theta) = o\left(\frac{-1}{\ln{\varepsilon}}\right)$. We have,
    $$ R_\varepsilon(r,\theta) := \frac{-1}{\ln{\varepsilon}}\Theta_\varepsilon(r,\theta), $$
    where,
    $$ \Theta_\varepsilon(r,\theta) := \sum_{n\in\mathbb{Z}^*} \ln{\varepsilon} \frac{ K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}r) - I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}r)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}\varepsilon)}\frac{I_n(\alpha^{-1/2}\varepsilon)}{I_n(\alpha^{-1/2}R)}\,\phi_n\,e^{in\theta}. $$
    Moreover,
    $$ \big|\Theta_\varepsilon(r,\theta)\big| \leq \sum_{n\in\mathbb{Z}^*} \big|\ln{\varepsilon}\big| \Bigg|\frac{ I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}r) - K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}r)}{ I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}\varepsilon) - I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R)}\Bigg|\Bigg|\frac{I_n(\alpha^{-1/2}\varepsilon)}{I_n(\alpha^{-1/2}R)}\Bigg|\,\big|\phi_n\big|. $$
    Since $I_n$ is an increasing function and $K_n$ is a decreasing function, we have, for $r\in[\varepsilon,R]$,
    $$ \big|I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}r) - K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}r)\big| \leq \big|I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}\varepsilon) - K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}\varepsilon)\big|. $$
    Thus,
    $$ \big|\Theta_\varepsilon(r,\theta)\big| \leq \sum_{n\in\mathbb{Z}^*} \big|\ln{\varepsilon}\big| \Bigg|\frac{I_n(\alpha^{-1/2}\varepsilon)}{I_n(\alpha^{-1/2}R)}\Bigg|\,\big|\phi_n\big|. $$
    Finally, using that $$ I_n(\alpha^{-1/2} \varepsilon) = \frac{1}{n!}\left(\frac{\alpha^{-1/2}}{2}\right)^n \varepsilon^n + \varepsilon^n\,r(\varepsilon), $$
    we have that $\Theta_\varepsilon$ tends to $0$ when $\varepsilon$ goes to $0$.
\end{proof}
By noticing that \cite{Abramowitz1972},
\begin{equation} \label{eq:wronskian}
    I_0(x)K_0'(x) - K_0(x)I_0'(x) = -I_0(x)K_1(x) - K_0(x)I_1(x) = - W\big(K_0(x),I_0(x)\big) = - \frac{1}{x},
\end{equation}
with $W$ the Wronskian and by using the previous result, we have the following: \\

\begin{proposition} For $\phi$ in $H^{1/2}(\partial B_R)$, we define,
    \[ \delta T(\phi) := \phi_0\frac{1}{R\, I_0(\alpha^{-1/2} R)^2}. \]
    Then, for $\varepsilon$ sufficiently small, we have the following asymptotic estimation,
    \[ \left\|T_\varepsilon - T_0 - \frac{-1}{\ln{\varepsilon}}\delta T\right\|_{\mathcal{L}\big(H^{1/2}(\partial B_R), H^{-1/2}(\partial B_R)\big)} = o\left(\frac{-1}{\ln{\varepsilon}}\right). \]
\end{proposition}

Finally, we can derive from the previous proposition the variations of the bilinear form: \\

\begin{proposition} For $\phi$ in $H^{1/2}(\partial B_R)$, we define,
    \[ \delta a(v,w) := \alpha\frac{v^\text{mean}}{I_0(\alpha^{-1/2} R)}\frac{w^\text{mean}}{I_0(\alpha^{-1/2} R)}, \]
    where $v^\text{mean}$ and $w^\text{mean}$ denote the mean value of $v$ and $w$ on $\partial B_R$. Then, for $\varepsilon$ sufficiently small, we have the following asymptotic estimation,
    \[ \left|a_\varepsilon(v,w) - a_0(v,w) - \frac{-2\pi}{\ln{\varepsilon}}\delta a(v,w)\right| = o\left(\frac{-1}{\ln{\varepsilon}}\right)\,\|v\|_{V_R} \|w\|_{V_R},\ \forall v,w \in V_R. \]
\end{proposition}

\begin{comment}

\color{black}
\newpage\color{red}
\subsection{Variations of the Bilinear Form} 

We start by giving the following lemma, \\

\begin{lemma} For $\varepsilon$ small enough, we have,
    \[ \|T_\varepsilon - T_0 - \varepsilon^{1/2}\delta T\|_{\mathcal{L}\big(H^{1/2}(\partial B_R), H^{-1/2}(\partial B_R)\big)} = O\big(\varepsilon^{1/2}\big). \]
    \label{prop:variations-T}
\end{lemma}
\begin{proof}
    We set for $x\in \R^2\setminus B_\varepsilon$,
    \[ \Psi_\varepsilon^{0,\phi}(x) := v_\varepsilon^{0,\phi}(x) - v_0^{0,\phi}(x) + \varepsilon^{1/2}\, v_\omega^{0,\phi}(x). \]
    By linearity, $\Psi_\varepsilon^{0,\phi}$ is the solution of
    \[ \left \{ \begin{array}{cl}
        -\alpha\Delta \Psi_\varepsilon^{0,\phi} + \Psi_\varepsilon^{0,\phi} = 0, & \text{in}\ B_R\setminus B_\varepsilon, \\
        %
        \Psi_\varepsilon^{0,\phi} = \varepsilon^{1/2}\, v_\omega^{0,\phi} - v_0^{0,\phi}, & \text{on}\ \partial B_\varepsilon, \\
        %
        \Psi_\varepsilon^{0,\phi} = \varepsilon^{1/2}\, v_\omega^{0,\phi}, & \text{on}\ \partial B_R.
    \end{array} \right .\]
    We notice that $(\varepsilon^{1/2}\, v_\omega^{0,\phi} - v_0^{0,\phi})$ is in $H^{1/2}(\partial B_\varepsilon)$ and that $\varepsilon^{1/2}\, v_\omega^{0,\phi}$ is in $H^{1/2}(\partial B_R)$. In fact,
    \begin{align*}
        \|\varepsilon^{1/2}\, v_\omega^{0,\phi}\|_{1/2,\partial B_R} & = C\, \varepsilon^{1/2} \, \big|v_0^{0,\phi}(x_0)\big| \, \big\|K_0\big(\alpha^{-1/2}|\cdot-x_0|\big)\big\|_{1/2,\partial B_R} = C'\, \varepsilon^{1/2} \, |v_0^{0,\phi}(x_0)|. \\
    \end{align*}
    % \begin{align*}
    %     \|\varepsilon\,v_\omega^{0,\phi}(\cdot/\varepsilon)\|_{1/2,\partial B_R} & \leq \varepsilon\,\|v_\omega^{0,\phi}(\cdot/\varepsilon)\|_{1,B_R\setminus B_{R/2}} \\
    %     %
    %     & \leq C\,\varepsilon\,\left( \|v_\omega^{0,\phi}(\cdot/\varepsilon)\|_{0,B_R\setminus B_{R/2}} + |v_\omega^{0,\phi}(\cdot/\varepsilon)|_{1,B_R\setminus B_{R/2}} \right).
    % \end{align*}
    
    % D'après la Proposition A.2. et la Proposition B.6., on a 
    
    % \begin{align*}
    %     \|\varepsilon\, v_\omega^{0,\phi}(\cdot/\varepsilon)\|_{1/2,\partial B_R} & \leq C\left(\varepsilon^2 \|v_\omega^{0,\phi}\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|v_\omega^{0,\phi}|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \right) \\
    %     %
    %     & \leq C\left(C_4\,\varepsilon^{5/2}\, \|v_0^{0,\phi}(x_0)\|_{1/2,\partial B_1} + C_5\, \varepsilon^{3/2}\, \|v_0^{0,\phi}(x_0)\|_{1/2,\partial B_1} \right) \\
    %     %
    %     & \leq C'\, \varepsilon^{3/2}\, \|v_0^{0,\phi}(x_0)\|_{1/2,\partial B_1} \\
    %     %
    %     & \leq C''\, \varepsilon^{3/2}\,|v_0^{0,\phi}(x_0)|.
    % \end{align*}
    From the maximum principle for $v_0^{0,\phi}$, we have $|v_0^{0,\phi}(x_0)|\leq \|\phi\|_{1/2,\partial B_R}$, and then,
    \begin{equation} \label{eq:variations-T}
        \|\varepsilon^{1/2}\, v_\omega^{0,\phi}\|_{1/2,\partial B_R} \leq C''\, \varepsilon^{1/2} \, \|\phi\|_{1/2,\partial B_R}.
    \end{equation} 
    % \[ \|\varepsilon\, v_\omega^{0,\phi}(\cdot/\varepsilon)\|_{1/2,\partial B_R} \leq C\, \varepsilon^{3/2}\,\|\varphi\|_{1/2,\partial B_R}. \]
    Thus,
    \begin{align*}
        \|\varepsilon^{1/2}\, v_\omega^{0,\phi}(\varepsilon\,\cdot) - v_0^{0,\phi}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} & \leq \|\varepsilon^{1/2}\, v_\omega^{0,\phi}(\varepsilon\,\cdot) - v_0^{0,\phi}(x_0)\|_{1/2,\partial B_1} + \|v_0^{0,\phi}(x_0) - v_0^{0,\phi}(\varepsilon\,\cdot)\|_{1/2,\partial B_1}.
    \end{align*}
    And the first term in the right hand side,
    \begin{align*}
        \|\varepsilon^{1/2}\, v_\omega^{0,\phi}(\varepsilon\,\cdot) - v_0^{0,\phi}(x_0)\|_{1/2,\partial B_1} & \leq \|\varepsilon^{1/2}\, v_\omega^{0,\phi}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} + \|v_0^{0,\phi}(x_0)\|_{1/2,\partial B_1} \\
        %
        %& \leq \varepsilon^{1/2}\|v_\omega^{0,\phi}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} + C|v_0^{0,\phi}(x_0)| \\
        %
        %& \leq \varepsilon^{1/2}\|v_\omega^{0,\phi}(\varepsilon\,\cdot)\|_{1,B_1\setminus B_{1/2}} + C\|\phi\|_{1/2,\partial B_R} \\
        %
        %& \leq \varepsilon^{1/2}\|v_\omega^{0,\phi}(\varepsilon\,\cdot)\|_{1,B_1} + C\|\phi\|_{1/2,\partial B_R} \\
        %
    \end{align*}
    Using the trace theorem and \eqref{eq:variations-T},
    \begin{align*}
        \|\varepsilon^{1/2}\, v_\omega^{0,\phi}(\varepsilon\,\cdot) - v_0^{0,\phi}(x_0)\|_{1/2,\partial B_1} & \leq \varepsilon^{1/2}\left( \|v_\omega^{0,\phi}(\varepsilon\,\cdot)\|_{0,B_1} + |v_\omega^{0,\phi}(\varepsilon\,\cdot)|_{1,B_1} \right) + C\|\phi\|_{1/2,\partial B_R} \\
        %
    \end{align*}
    By re-scaling, we rewrite,
    \begin{align*}
        \|\varepsilon^{1/2}\, v_\omega^{0,\phi}(\varepsilon\,\cdot) - v_0^{0,\phi}(x_0)\|_{1/2,\partial B_1} & \leq \varepsilon^{1/2}\left( \varepsilon^{-1/2}\|v_\omega^{0,\phi}\|_{0,B_\varepsilon} + \varepsilon^{1/2}|v_\omega^{0,\phi}|_{1,B_\varepsilon} \right) + C\|\phi\|_{1/2,\partial B_R} \\
        %
        & \leq  \|v_\omega^{0,\phi}\|_{0,B_1} + \varepsilon|v_\omega^{0,\phi}|_{1,B_1} + C\|\phi\|_{1/2,\partial B_R} \\
        %
        & \leq C\|\phi\|_{1/2,\partial B_R} + C\varepsilon\|\phi\|_{1/2,\partial B_R} + C\|\phi\|_{1/2,\partial B_R} \\
        %
        & \leq C\,\|\phi\|_{1/2,\partial B_R}.
    \end{align*}
    Similarly,
    \begin{align*}
        \|v_0^{0,\phi}(x_0) - v_0^{0,\phi}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} & = \varepsilon\left\|\varepsilon^{-1} \left(v_0^{0,\phi}(x_0) - v_0^{0,\phi}(\varepsilon\,\cdot)\right)\right\|_{1/2,\partial B_1} \\
        %
        %& \leq C\,\varepsilon\,\|v_0^{0,\phi}\|_{\mathcal{C}^1(B_{R/2})} \\
        %
        & \leq C\,\varepsilon\,\|\phi\|_{1/2,\partial B_R}.
    \end{align*}

    % \begin{align*}
    %     \|v_0^{0,\phi}(x_0) - v_0^{0,\phi}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} & = \varepsilon\left\|\varepsilon^{-1} \left(v_0^{0,\phi}(x_0) - v_0^{0,\phi}(\varepsilon\,\cdot)\right)\right\|_{1/2,\partial B_1} \\
    %     %
    %     & \leq C\,\varepsilon\,\|v_0^{0,\phi}\|_{\mathcal{C}^1(B_{R/2})} \\
    %     %
    %     & \leq C\,\varepsilon\,\|\varphi\|_{1/2,\partial B_R} ?.
    % \end{align*}
    Applying Proposition \ref{prop:v-epsilon-estimates} from the appendix, we have,
    \begin{align*}
        \|\Psi_\varepsilon^{0,\phi}\|_{1,B_R\setminus B_{R/2}} & \leq C\,\big(\|\varepsilon^{1/2}\, v_\omega^{0,\phi}\|_{1/2,\partial B_R} + e^{-R/(2\varepsilon\sqrt{\alpha})}\|\varepsilon^{1/2}\, v_\omega^{0,\phi}(\varepsilon\,\cdot) - v_0^{0,\phi}(\varepsilon\,\cdot)\|_{1/2,\partial B_1}\big) \\
        %
        & \leq C'\,\varepsilon^{1/2}\,\|\phi\|_{1/2,\partial B_R}.
    \end{align*}
    Finally, Proposition \ref{prop:norm-minus-1-2} gives,
    \begin{align*}
        \|(T_\varepsilon - T_0 - \varepsilon^{1/2}\,\delta T) \phi\|_{-1/2,\partial B_R} & = \|\nabla\big(v_\varepsilon^{0,\phi} - v_0^{0,\phi} + \varepsilon^{1/2}\, v_\omega^{0,\phi}\big)\cdot n\|_{-1/2,\partial B_R} \\
        %
        & = \|\nabla \Psi_\varepsilon^{0,\phi} \cdot n\|_{-1/2,\partial B_R} \\
        %
        & \leq C\,\|\Psi_\varepsilon^{0,\phi}\|_{1,B_R\setminus B_{R/2}} \\
        %
        & \leq C'\,\varepsilon^{1/2}\,\|\phi\|_{1/2,\partial B_R}.
    \end{align*}
\end{proof}

The asymptotic expansion of the variations for the bilinear form follows immediately from the Lemma \ref{prop:variations-T}  : \\

\begin{proposition}
    % Soit $\varphi\in H^{1/2}(\partial B_R)$. Soit $v_\omega^{0,\phi}$ la solution du problème extérieur 
    
    % \[ \left \{ \begin{array}{cc}
    %     -\alpha\Delta v_\omega^{0,\phi} + v_\omega^{0,\phi} = 0, & \text{dans}\ \R^2\setminus B(x_0,1), \\
    %     v_\omega^{0,\phi} = v_0^{0,\phi}(x_0), & \text{sur}\ \partial B(x_0,1), \\
    %     v_\omega^{0,\phi} = 0, & \text{à}\ \infty.
    % \end{array} \right .\]
    
    Let $\delta T : H^{1/2}(\partial B_R) \to H^{-1/2}(\partial B_R)$ such that for all $\phi$ in $H^{1/2}(\partial B_R)$,
    \[ \delta T\phi = -\nabla v_\omega^{0,\phi} \cdot n. \]
    Let $v,w$ be in $V_R$, we set,
    \[ \delta a(v,w) := \alpha\int_{\partial B_R} \delta T v\, w\ d\sigma. \]
    Then, for $\varepsilon$ small enough, we have,
    \[ \|a_\varepsilon - a_0 - \varepsilon^{1/2}\,\delta a\|_{\mathcal{L}_2(V_R)} = O(\varepsilon^{1/2}). \]
\end{proposition}
%\begin{proof} Let $v,w\in V_R$, we have,
%    \begin{align*}
%        a_\varepsilon(v, w) - a_0(v, w) % & = \alpha\int_{D\setminus B_R} \nabla v\cdot\nabla w\ dx + \int_{D\setminus %B_R} v\, w\ dx + \alpha\int_{\partial B_R} T_\varepsilon v\, w\ d\sigma - \alpha\int_{D\setminus B_R} \nabla v\cdot \nabla %w\ dx \\
        %& \hspace{2cm} - \int_{D\setminus B_R} v\, w\ dx - \alpha\int_{\partial B_R} T_0 v\, w\ d\sigma \\
        %
 %       & = \alpha\int_{\partial B_R} (T_\varepsilon-T_0) v\, w\ d\sigma. \\
 %   \end{align*}
 %   From Lemma \ref{prop:variations-T}, we get the result.
%\end{proof}

% \begin{proposition}
%     \[ a_\varepsilon(v_0, w_\varepsilon) - a_0(v_0, w_\varepsilon) = ?. \]
% \end{proposition}
% \begin{proof}
%     \[ a_\varepsilon(v_0, w_\varepsilon) - a_0(v_0, w_\varepsilon) = \alpha\int_{D\setminus B_R} \nabla v_0\cdot\nabla w_\varepsilon\ dx + \int_{D\setminus B_R} v_0\, w_\varepsilon\ dx + \int_{\partial B_R} T_\varepsilon v_0\, w_\varepsilon\ d\sigma \] \[ - \alpha\int_{D\setminus B_R} \nabla v_0\cdot w_\varepsilon\ dx - \int_{D\setminus B_R} v_0\, w_\varepsilon\ dx - \int_{\partial B_R} T_0 v_0\, w_\varepsilon\ d\sigma \]
%     \[ = \int_{\partial B_R} (T_\varepsilon-T_0) v_0\, w_\varepsilon\ d\sigma \]
%     \[ = \int_{\partial B_R} (T_\varepsilon-T_0) v_0\, w_0\ d\sigma + \int_{\partial B_R} (T_\varepsilon-T_0) v_0\, (w_\varepsilon-w_0)\ d\sigma \]
    
%     D'où avec Taylor 
    
%     \[ a_\varepsilon(v_0, w_\varepsilon) - a_0(v_0, w_\varepsilon) = w_0(x_0)\int_{\partial B_R} (T_\varepsilon-T_0) v_0\ d\sigma + O(\varepsilon)\int_{\partial B_R} (T_\varepsilon-T_0) v_0\ d\sigma + \int_{\partial B_R} (T_\varepsilon-T_0) v_0\, (w_\varepsilon-w_0)\ d\sigma \]
    
%     \underline{(J'affirme que le terme principal est $w_0(x_0)\int_{\partial B_R} (T_\varepsilon-T_0) v_0\ d\sigma$)}
    
%     De plus 
    
%     \[ \int_{\partial B_R} (T_\varepsilon-T_0) v_0\ d\sigma = \int_{\partial B_R} \partial_n (v_\varepsilon^{0,v_0} - v_0^{0,v_0})\ d\sigma \]

%     On pose pour $x\in \R^2\setminus B_\varepsilon$,
    
%     \[ w_\varepsilon^{0,v_0}(x) := v_\varepsilon^{0,v_0}(x) - v_0^{0,v_0}(x) + v_\omega(x/\varepsilon), \]
    
%     où $v_\omega$ est la solution du problème extérieur suivant
    
    
    
%     Ainsi, 
    
%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta w_\varepsilon^{0,v_0} + w_\varepsilon^{0,v_0} = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         w_\varepsilon^{0,v_0} = v_0(x_0) - v_0^{0,v_0}, & \text{sur}\ \partial B_\varepsilon, \\
%         w_\varepsilon^{0,v_0} = v_\omega(\cdot/\varepsilon), & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\omega(\cdot/\varepsilon)\|_{1/2,\partial B_R} \leq \|v_\omega(\cdot/\varepsilon)\|_{1,B_{R/2}\setminus B_R} \]
%     \[ \leq \|v_\omega(\cdot/\varepsilon)\|_{0,B_{R/2}\setminus B_R} + |v_\omega(\cdot/\varepsilon)|_{1,B_{R/2}\setminus B_R} \]
%     \[ \leq \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|v_\omega|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \]
%     \[ \leq \|V\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \|W\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|V|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|W|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \]
%     \[ \leq \big(C_5\,R^{1/2}\varepsilon^{-1/2} + C_6\,R^{-1/2}\varepsilon^{1/2} + C_7\,R^{-1/2}\varepsilon^{3/2} + C_8\,R^{1/2}\varepsilon^{1/2}\big)\|\psi\|_{1/2,\partial B_1} \]
%     \[ \leq C\,\varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}. \]
    
%     Aussi, (Annexe)

%     \[ \| v_0(x_0) - v_0^{0,v_0}(\varepsilon \cdot) \|_{1/2,\partial B_1} \leq \| v_0(x_0) - v_0^{0,v_0}(\varepsilon \cdot) \|_{1, B_1\setminus B_{1/2}} \]
%     \[ \leq \| v_0(x_0) - v_0^{0,v_0}(\varepsilon \cdot) \|_{1, B_1} \]
    
%     Ainsi,
    
%     \[ |w_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C\big( \varepsilon^{?}\|v_\omega(x/\varepsilon)\|_{1/2,\partial B_R} + \varepsilon^{?}\|v_0(x_0) - v_0^{0,v_0}(\cdot/\varepsilon)\|_{1/2,\partial B_1} \big) \]
    
%     Enfin, (44)
    
%     \[ \|\nabla (v_\varepsilon^{0,\psi} - v_0^{0,\psi} + V^{0,\psi} ) \cdot n\|_{-1/2,\partial B_R} \leq C |v_\varepsilon^{0,\psi} - v_0^{0,\psi} + V^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ \leq C |v_\varepsilon^{0,\psi} - v_0^{0,\psi} + V^{0,\psi} + W^{0,\psi} - W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ = C |v_\varepsilon^{0,\psi} - v_0^{0,\psi} + v_\omega - W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ = C |w_\varepsilon - W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ \leq C \Big(|w_\varepsilon|_{1,B_R\setminus B_{R/2}} + |W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \Big) \]
    
%     % Mais
    
%     % \[ v_\varepsilon^{0,v_0} - v_0^{0,v_0} = v_\omega + o(\varepsilon^?) \]
    
%     % ---------------------------------------------------------
    
%     % \[  = \int_{B_R} \nabla(v_\varepsilon^{0,v_0} - v_0^{0,v_0})\cdot\nabla 1\ dx + \int_{B_R} \Delta (v_\varepsilon^{0,v_0} - v_0^{0,v_0})\ dx \]
%     % \[  = \int_{B_R} \Delta (v_\varepsilon^{0,v_0} - v_0^{0,v_0})\ dx \]
%     % \[  = \int_{B_R\setminus B_\varepsilon} \Delta v_\varepsilon^{0,v_0}\ dx - \int_{B_R\setminus B_\varepsilon} \Delta v_0^{0,v_0}\ dx +  \int_{B_\varepsilon} \Delta v_\varepsilon^{0,v_0}\ dx - \int_{B_\varepsilon} \Delta v_0^{0,v_0}\ dx \]
%     % \[  = \frac{1}{\alpha}\int_{B_R\setminus B_\varepsilon} v_\varepsilon^{0,v_0}\ dx - \frac{1}{\alpha}\int_{B_R\setminus B_\varepsilon} v_0^{0,v_0}\ dx +  \int_{B_\varepsilon} \Delta v_\varepsilon^{0,v_0}\ dx - \frac{1}{\alpha} \int_{B_\varepsilon} v_0^{0,v_0}\ dx \]
    
%     % ---------------------------------------------------
    
%     % $h := v_\varepsilon^{0,v_0} - v_0^{0,v_0}$.
    
%     % \[ \left \{ \begin{array}{cc}
%     %     -\alpha\Delta h_\varepsilon + h_\varepsilon = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%     %     h_\varepsilon = - v_0^{0,v_0}, & \text{sur}\ \partial B_\varepsilon, \\
%     %     h_\varepsilon = 0, & \text{sur}\ \partial B_R.
%     % \end{array}
%     % \right .\]
    
%     % \[ \int_{\partial B_R} (T_\varepsilon-T_0) v_0\ d\sigma = \int_{\partial B_R} \partial_n h_\varepsilon\ d\sigma \]
    
%     % \[ \left \{ \begin{array}{cc}
%     %     -\alpha\Delta \tilde{h}_\varepsilon + \tilde{h}_\varepsilon = 0, & \text{dans}\ B_R, \\
%     %     \tilde{h}_\varepsilon = 0, & \text{sur}\ \partial B_R.
%     % \end{array}
%     % \right .\]
    
%     % \[ \left \{ \begin{array}{cc}
%     %     -\alpha\Delta \epsilon_\varepsilon + \epsilon_\varepsilon = 0, & \text{dans}\ B_\varepsilon, \\
%     %     \epsilon_\varepsilon = \tilde{h}_\varepsilon +  v_0^{0,v_0}, & \text{sur}\ \partial B_\varepsilon, \\
%     % \end{array}
%     % \right .\]
    
%     % J'affirme que $h_\varepsilon = \tilde{h}_\varepsilon - \epsilon_\varepsilon$. D'où
    
%     % \[ \int_{\partial B_R} (T_\varepsilon-T_0) v_0\ d\sigma = \int_{B_R} \Delta h_\varepsilon\ dx = \int_{B_R}\Delta\tilde{h}_\varepsilon\ dx - \int_{B_\varepsilon} \Delta \epsilon_\varepsilon\ dx \]
%     % \[ = \frac{1}{\alpha} \int_{B_R}\tilde{h}_\varepsilon\ dx - \frac{1}{\alpha} \int_{B_\varepsilon} \epsilon_\varepsilon\ dx \]
    
%     % Dans le papier du L2 : 
%     % \[ \frac{1}{\alpha} \int_{B_R}\tilde{h}_\varepsilon\ dx =  \]
%     % et
%     % \[ \frac{1}{\alpha} \int_{B_\varepsilon} \epsilon_\varepsilon\ dx = \]
% \end{proof}
% As we have 
% \[
% a_\varepsilon(v, w) - a_0(v, w) = \alpha\int_{\partial B_R} (T_\varepsilon-T_0) v\, w\ d\sigma.
% \]
% a straightforward consequence of the previous lemma is 
% \begin{proposition}
%     % Soit $\varphi\in H^{1/2}(\partial B_R)$. Soit $v_\omega^{0,\phi}$ la solution du problème extérieur 
    
%     % \[ \left \{ \begin{array}{cc}
%     %     -\alpha\Delta v_\omega^{0,\phi} + v_\omega^{0,\phi} = 0, & \text{dans}\ \R^2\setminus B(x_0,1), \\
%     %     v_\omega^{0,\phi} = v_0^{0,\phi}(x_0), & \text{sur}\ \partial B(x_0,1), \\
%     %     v_\omega^{0,\phi} = 0, & \text{à}\ \infty.
%     % \end{array} \right .\]
    
%     Let $\delta T : H^{1/2}(\partial B_R) \to H^{-1/2}(\partial B_R)$ such that for all $\phi$ in $H^{1/2}(\partial B_R)$,
%     \[ \delta T\phi = -\nabla v_\omega^{0,\phi} \cdot n. \]
%     Let $v,w$ be in $V_R$, we set,
%     \[ \delta a(v,w) := \alpha\int_{\partial B_R} \delta T v\, w\ d\sigma. \]
%     Then, for $\varepsilon$ small enough, we have,
%     \[ \|a_\varepsilon - a_0 - \varepsilon^{1/2}\,\delta a\|_{\mathcal{L}_2(V_R)} = O(\varepsilon^{1/2}). \]
% \end{proposition}

\color{black}

\end{comment}


\subsection{Variations of the Linear Form}

We give an explicit formulation for both $v_0^{h,0}$ and $v_\varepsilon^{h,0}$ with the following proposition: \\

% \newpage
% \begin{proposition} \label{prop:solution-unhomo} For $h$ in $L^2(B_R)$, we have,
%     \[ v_0^{h,0} (r, \theta) = \sum_{n\in\mathbb{N}} \Big( \big( A_{0,n} +  A_{0,n}^\text{p}(r) \big) I_n(\alpha^{-1/2}\,r) + B_{0,n}^\text{p}(r) K_n(\alpha^{-1/2}\,r) \Big)\,e^{in\theta}, \]
%     with
%     \begin{align*}
%         & A_{0,n}^\text{p}(r) := -\alpha^{-1}\int_0^r s\,K_n(\alpha^{-1/2}\, s) h_n(s)\ ds, \\
%         %
%         & B_{0,n}^\text{p}(r) := \alpha^{-1}\int_0^r s\,I_n(\alpha^{-1/2}\, s) h_n(s)\ ds, \\
%         %
%         & A_{0,n} := -\frac{ A_{0,n}^\text{p}(R) I_n(\alpha^{-1/2}\, R) + B_{0,n}^\text{p}(R) K_n(\alpha^{-1/2}\, R) }{I_n(\alpha^{-1/2}\, R)}.
%     \end{align*}
    
%     Moreover, 
%     \[ v_\varepsilon^{h,0}(r, \theta) = \sum_{n\in\mathbb{N}} \Big(\big( A_{\varepsilon,n} +  A_{\varepsilon,n}^\text{p}(r) \big) I_n(\alpha^{-1/2}\,r) + \big(B_{\varepsilon,n} + B_{\varepsilon,n}^\text{p}(r)\big) K_n(\alpha^{-1/2}\,r) \Big) \,e^{in\theta}, \]
%     with
%     \begin{align*}
%         & A_{\varepsilon,n}^\text{p}(r) = -\alpha^{-1}\int_\varepsilon^r s\,K_n(\alpha^{-1/2}\, s) h_n(s)\ ds, \\
%         %
%         & B_{\varepsilon,n}^\text{p}(r) = \alpha^{-1}\int_\varepsilon^r s\,I_n(\alpha^{-1/2}\, s) h_n(s)\ ds, \\
%         %
%         & A_{\varepsilon, n} = \frac{K_n(\alpha^{-1/2}\varepsilon)\big( A_{\varepsilon, n}^\text{p}(R)I_n(\alpha^{-1/2}R) + B_{\varepsilon, n}^\text{p}(R)K_n(\alpha^{-1/2}R) \big)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)}, \\
%         %
%         & B_{\varepsilon, n} = -\frac{I_n(\alpha^{-1/2}\varepsilon)\big( A_{\varepsilon, n}^\text{p}(R)I_n(\alpha^{-1/2}R) + B_{\varepsilon, n}^\text{p}(R)K_n(\alpha^{-1/2}R) \big)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)}.
%     \end{align*}
% \end{proposition}
% \begin{proof}
%     Using polar coordinates in $\R^2$, we have
%     \[ v_\varepsilon^{h,0}(r, \theta) = \sum_{n\in\mathbb{N}} c_n(r) \,e^{in\theta} \qquad \text{and} \qquad h(r, \theta) = \sum_{n\in\mathbb{N}} h_n(r) \,e^{in\theta}, \]
%     where $c_n$ satisfies, for all $n$ in $\N$,
%     \[ -\alpha\,r^2\,c_n''(r) - \alpha\,r\,c_n'(r) + (r^2+\alpha n^2) c_n(r) = r^2 h_n(r). \]
%     First, we use the variation of parameters method to get the following particular solution :
%     \[ c_n^\text{p}(r) = A_{\varepsilon,n}^\text{p}(r) I_n(\alpha^{-1/2}\,r) + B_{\varepsilon,n}^\text{p}(r) K_n(\alpha^{-1/2}\,r). \]
%     Then by the superposition principle, by using the previously computed homogeneous solution and by using the boundaries conditions, we have the result. Same for $v_0^{h,0}$.
% \end{proof}
% \newpage

\begin{proposition} \label{prop:solution-unhomo} For $h$ in $L^2(B_R)$, we have,
    \[ v_0^{h,0} (r, \theta) = \sum_{n\in\mathbb{Z}} \Big( \big( A_{0,n} +  A_{n}^\text{p}(r) \big) I_n(\alpha^{-1/2}\,r) + B_{n}^\text{p}(r) K_n(\alpha^{-1/2}\,r) \Big)\,e^{in\theta}, \]
    with,
    \begin{align*}
        & A_{n}^\text{p}(r) := -\alpha^{-1}\int_0^r s\,K_n(\alpha^{-1/2}\, s) h_n(s)\ ds, \\
        %
        & B_{n}^\text{p}(r) := \alpha^{-1}\int_0^r s\,I_n(\alpha^{-1/2}\, s) h_n(s)\ ds, \\
        %
        & A_{0,n} := -\frac{ A_{n}^\text{p}(R) I_n(\alpha^{-1/2}\, R) + B_{n}^\text{p}(R) K_n(\alpha^{-1/2}\, R) }{I_n(\alpha^{-1/2}\, R)}.
    \end{align*}
    
    Moreover, 
    \[ v_\varepsilon^{h,0}(r, \theta) = \sum_{n\in\mathbb{Z}} \Big(\big( A_{\varepsilon,n} +  A_{n}^\text{p}(r) \big) I_n(\alpha^{-1/2}\,r) + \big(B_{\varepsilon,n} + B_{n}^\text{p}(r)\big) K_n(\alpha^{-1/2}\,r) \Big) \,e^{in\theta}, \]
    with,
    \begin{align*}
        & A_{\varepsilon, n} = \frac{K_n(\alpha^{-1/2}\varepsilon)\big( A_{n}^\text{p}(R)I_n(\alpha^{-1/2}R) + B_{n}^\text{p}(R)K_n(\alpha^{-1/2}R) \big)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)}, \\
        %
        & B_{\varepsilon, n} = -\frac{I_n(\alpha^{-1/2}\varepsilon)\big( A_{n}^\text{p}(R)I_n(\alpha^{-1/2}R) + B_{n}^\text{p}(R)K_n(\alpha^{-1/2}R) \big)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)}.
    \end{align*}
\end{proposition}
\begin{proof}
    Using polar coordinates in $\R^2$, we have,
    \[ v_\varepsilon^{h,0}(r, \theta) = \sum_{n\in\Z} c_n(r) \,e^{in\theta} \qquad \text{and} \qquad h(r, \theta) = \sum_{n\in\Z} h_n(r) \,e^{in\theta}, \]
    where $c_n$ satisfies, for all $n$ in $\Z$ and $0<r\leq R$,
    \begin{equation} \label{eq:fourier-coeff-equation}
        -\alpha\,r^2\,c_n''(r) - \alpha\,r\,c_n'(r) + (r^2+\alpha n^2) c_n(r) = r^2 h_n(r).
    \end{equation}
    Firstly, we solve the homogeneous equation, and we get,
    $$ c_{0,n}^\text{h}(r) = A_{0,n} I_n(\alpha^{-1/2}\,r), $$
    and
    $$ c_{\varepsilon,n}^\text{h}(r) = A_{\varepsilon,n} I_n(\alpha^{-1/2}\,r) + B_{\varepsilon,n} K_n(\alpha^{-1/2}\,r). $$
    Secondly, we use the variation of parameters method to get the particular solution,
    \begin{equation} \label{eq:particular-solution}
        c_n^\text{p}(r) = A_{n}^\text{p}(r) I_n(\alpha^{-1/2}\,r) + B_{n}^\text{p}(r) K_n(\alpha^{-1/2}\,r).
    \end{equation}
    By replacing \eqref{eq:particular-solution} into \eqref{eq:fourier-coeff-equation}, and by supposing that, $$ (A_{n}^\text{p})'(r) I_n(\alpha^{-1/2}\,r) + (B_{n}^\text{p})'(r) K_n(\alpha^{-1/2}\,r) = 0, $$
    we get,
    $$ (A_{n}^\text{p})'(r) I_n'(\alpha^{-1/2}\,r) + (B_{n}^\text{p})'(r) K_n'(\alpha^{-1/2}\,r) = -\alpha^{-1/2} h_n(r). $$
    Solving the last two equations, we get the value of $A_{n}^\text{p}(r)$ and $B_{n}^\text{p})(r)$ as stated in the theorem. Finally, by the superposition principle and by using the boundaries conditions, we have the result.
\end{proof}

% \newpage


\begin{note} 
    Since $h$ is in $L^2(D)$, using the Parseval's equality we have that the Fourier coefficients $h_n$ are in $L^2(D)$ as well. Similarly for the Fourier coefficients $c_n$. As a result, we have that the integral in the $A_{n}^\text{p}$ is convergent.
\end{note}

\begin{note} 
    We have, $$ v_0^{h,0} (x_0) = \sum_{n\in\mathbb{Z}} A_{0,n} I_n(0)\,e^{in\theta},\ \forall \theta \in [0,2\pi[, $$
    and in particular, for $\theta=0$, we have 
    $$ v_0^{h,0} (x_0) = \sum_{n\in\mathbb{Z}} A_{0,n} I_n(0). $$
    Moreover, \cite{Abramowitz1972, Oldham2009}, $I_n(0)$ vanishes for $n\in\N^*$ and $I_0(0) = 1$. Then,
    \begin{equation} \label{eq:A00}
        A_{0,0} = v_0^{h,0}(x_0).
    \end{equation}
\end{note}

Now, we can state the variation of the solution with respect to hole's radius: \\

% \newpage
% \begin{proposition} For $h$ in $L^2(B_R)$, we set,
%     \[ \delta v^{h,0}(r) := -A_{0,0} \frac{I_0(\alpha^{-1/2}\, R)K_0(\alpha^{-1/2}r) - K_0(\alpha^{-1/2}R)I_0(\alpha^{-1/2}r)}{I_0(\alpha^{-1/2}\,R)}, \]
%     where $A_{0,0}$ is defined in Proposition \ref{prop:solution-unhomo}. Then, for $\varepsilon$ sufficiently small, we have the following asymptotic estimation,
%     \[ v_\varepsilon^{h,0}(r, \theta) - v_0^{h,0}(r, \theta) - \frac{-1}{\ln{\varepsilon}}\delta v^{h,0}(r) = o\left(\frac{-1}{\ln{\varepsilon}}\right). \]
% \end{proposition}
% \begin{proof} We have,
%      $$ v_\varepsilon^{h,0}(r, \theta) - v_0^{h,0}(r, \theta) = \delta A_{\varepsilon, 0}(r) I_0(\alpha^{-1/2}\,r) + \delta B_{\varepsilon, 0}(r) K_0(\alpha^{-1/2}\,r) + R_{\varepsilon}(r), $$
%     where,
%     $$ \delta A_{\varepsilon, n}(r) := \big( A_{\varepsilon,n} - A_{0,n} \big) +  \big( A_{\varepsilon,n}^\text{p}(r) - A_{0,n}^\text{p}(r) \big), $$
%     $$ \delta B_{\varepsilon, n}(r) := B_{\varepsilon,n} + \big( B_{\varepsilon,n}^\text{p}(r) - B_{0,n}^\text{p}(r) \big), $$
%     and,
%     $$ R_{\varepsilon}(r) := \sum_{n\in\mathbb{N}^*} \Big( \delta A_{\varepsilon, n}(r) I_n(\alpha^{-1/2}\,r) + \delta B_{\varepsilon, n}(r) K_n(\alpha^{-1/2}\,r) \Big)\,e^{in\theta}. $$
%     Now, we use estimates stated in Appendix \ref{app:calculus}, and we get,
%     $$ \delta A_{\varepsilon,  0}(r) = A_{0,0} \frac{K_0(\alpha^{-1/2}R)}{I_0(\alpha^{-1/2}\, R)} \frac{-1}{\ln{\varepsilon}} + o\left(\frac{-1}{\ln{\varepsilon}}\right), $$
%     $$ \delta B_{\varepsilon, 0}(r) = -A_{0,0}\frac{-1}{\ln{\varepsilon}} + o\left(\frac{-1}{\ln{\varepsilon}}\right). $$
%     This gives us the dominant part of the asymptotic development. It remains to show that $R_\varepsilon(r) = o\left(\frac{-1}{\ln{\varepsilon}}\right)$. It is sufficient to show that for all $n$ in $\N^*$,
%     $$ |\ln{\varepsilon}| \Big| \delta A_{\varepsilon, n}(r) I_n(\alpha^{-1/2}\,r) + \delta B_{\varepsilon, n}(r) K_n(\alpha^{-1/2}\,r) \Big|, $$
%     goes to $0$ as $\varepsilon$ goes to $0$.
%     % First, we have,
%     % $$ \delta A_{\varepsilon, n}(r) = \big( \frac{K_n(\alpha^{-1/2}\varepsilon)\big( A_{\varepsilon, n}^\text{p}(R)I_n(\alpha^{-1/2}R) + B_{\varepsilon, n}^\text{p}(R)K_n(\alpha^{-1/2}R) \big)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)} $$ $$ + \frac{ A_{0,n}^\text{p}(R) I_n(\alpha^{-1/2}\, R) + B_{0,n}^\text{p}(R) K_n(\alpha^{-1/2}\, R) }{I_n(\alpha^{-1/2}\, R)} \big) + \big( A_{\varepsilon,n}^\text{p}(r) - A_{0,n}^\text{p}(r) \big), $$
%     % $$ = \frac{K_n(\alpha^{-1/2}\varepsilon) A_{\varepsilon, n}^\text{p}(R)I_n(\alpha^{-1/2}R) + \big( A_{0,n}^\text{p}(R) + A_{\varepsilon,n}^\text{p}(r) - A_{0,n}^\text{p}(r) \big) (I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R))}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)} $$ $$ + \frac{K_n(\alpha^{-1/2}\varepsilon) B_{\varepsilon, n}^\text{p}(R)K_n(\alpha^{-1/2}R)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)} + \frac{ B_{0,n}^\text{p}(R) K_n(\alpha^{-1/2}\, R) }{I_n(\alpha^{-1/2}\, R)}  $$
%     Using that, $$ \big(A_{\varepsilon, n}^\text{p}(R) - A_{0, n}^\text{p}(R)\big) - \big(A_{\varepsilon, n}^\text{p}(r) - A_{0, n}^\text{p}(r)\big) = 0, $$
%     we rewrite,
%     \begin{multline*}
%         \delta A_{\varepsilon, n}(r) = \frac{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) A_{\varepsilon, n}^\text{p}(R)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)} \\ + \frac{I_n(\alpha^{-1/2}\, R) K_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) \big(B_{\varepsilon, n}^\text{p}(R)-B_{0, n}^\text{p}(R)\big)}{I_n(\alpha^{-1/2}\, R) \Big(I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R) \Big)} \\ + \frac{K_n(\alpha^{-1/2}\, R)^2 I_n(\alpha^{-1/2}\varepsilon) B_{0,n}^\text{p}(R)}{I_n(\alpha^{-1/2}\, R) \Big(I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R) \Big)},
%     \end{multline*}
%     and,
%     \begin{multline*}
%         \delta B_{\varepsilon, n}(r) = -\frac{I_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R) A_{\varepsilon, n}^\text{p}(R)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)} \\ - \frac{K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)\Big(B_{\varepsilon,n}^\text{p}(R) - B_{0,n}^\text{p}(R)\Big)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)} \\ - \frac{I_n(\alpha^{-1/2}\varepsilon) K_n(\alpha^{-1/2}R)B_{0,n}^\text{p}(R)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)}.
%     \end{multline*}
%     %($\delta A$ et $\delta B$ constants en $r$ ?)
%     Straightforward computations give,
%     \begin{multline*}
%         \delta A_{\varepsilon, n}(r) I_n(\alpha^{-1/2}\,r) + \delta B_{\varepsilon, n}(r) K_n(\alpha^{-1/2}\,r) = \Big(I_n(\alpha^{-1/2}\,\varepsilon)A_{\varepsilon, n}^\text{p}(R) \\ + K_n(\alpha^{-1/2}\,\varepsilon)\Big(B_{\varepsilon,n}^\text{p}(R) - B_{0,n}^\text{p}(R)\Big) + \frac{K_n(\alpha^{-1/2}\,R)}{I_n(\alpha^{-1/2}\,R)} I(\varepsilon) B_{0, n}^\text{p}(R)\Big) \phi_n(r),
%     \end{multline*}
%     where,
%     $$ \phi_n(r) := \frac{I_n(\alpha^{-1/2} r)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2} r)I_n(\alpha^{-1/2}R)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)}. $$
%     Since $I_n$ is an increasing function and $K_n$ is a decreasing function, we have, for $r\in[\varepsilon,R]$,
%     $$ \big|I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}r) - K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}r)\big| \leq \big|I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}\varepsilon) - K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}\varepsilon)\big|, $$
%     and thus,
%     $$ |\phi_n(r)| \leq 1. $$
%     We have,
%     \begin{multline*}
%         |\ln{\varepsilon}| \Big|\delta A_{\varepsilon, n}(r) I_n(\alpha^{-1/2}\,r) + \delta B_{\varepsilon, n}(r) K_n(\alpha^{-1/2}\,r) \Big| \leq \Big|I(\varepsilon)A_{\varepsilon, n}^\text{p}(R)\ln{\varepsilon}\Big| \\ + \Big|K(\varepsilon)\Big(B_{\varepsilon,n}^\text{p}(R) - B_{0,n}^\text{p}(R)\ln{\varepsilon}\Big)\Big| + \Big|\frac{K(R)}{I(R)}B_{0, n}^\text{p}(R)I(\varepsilon)\ln{\varepsilon}\Big|.
%     \end{multline*}
%     For $\varepsilon$ small enough, we have using Appendix \ref{app:calculus}, \cite{Abramowitz1972, Oldham2009} and that $A_{\varepsilon, n}^\text{p}$ is bounded uniformly in $\varepsilon$ (see previous Remark),
%     $$ \Big|I_n(\alpha^{-1/2}\,\varepsilon)A_{\varepsilon, n}^\text{p}(R) \ln{\varepsilon}\Big| =  M\Big|\Big(\frac{2^{-n}\alpha^{-n/2}}{n!} \varepsilon^n + \varepsilon^n\,r(\varepsilon) \Big)\ln{\varepsilon}\Big| \to_{\varepsilon\to 0} 0. $$
%     %
%     If $n = 1$, we have,
%     $$ \Big|K_n(\alpha^{-1/2}\,\varepsilon)\Big(B_{\varepsilon,n}^\text{p}(R) - B_{0,n}^\text{p}(R)\Big)\ln{\varepsilon}\Big| = \Big|\Big(\alpha^{1/2}\varepsilon^{-1} + \varepsilon^{-1} r_1(\varepsilon)\Big)\Big(\frac{\alpha^{-1/2}}{6} \varepsilon^{3} + \varepsilon^{3} r_2(\varepsilon)\Big)\ln{\varepsilon}\Big| \to_{\varepsilon\to 0} 0. $$
%     If $n > 1$, we have,
%     $$ \Big|K_n(\alpha^{-1/2}\,\varepsilon)\Big(B_{\varepsilon,n}^\text{p}(R) - B_{0,n}^\text{p}(R)\Big)\ln{\varepsilon}\Big| = \Big|\Big(2^{n-1} \Gamma(n) \varepsilon^{-n} + \varepsilon^{-n} r_1(\varepsilon)\Big)\Big(\frac{2^{-n}\alpha^{-n/2}}{n!(n+2)} \varepsilon^{n+2} + \varepsilon^{n+2} r_2(\varepsilon)\Big)\ln{\varepsilon} \Big| \to_{\varepsilon\to 0} 0. $$
%     To finish,
%     $$ \Big|\frac{K_n(\alpha^{-1/2}\,R)}{I_n(\alpha^{-1/2}\,R)}B_{0, n}^\text{p}(R)I_n(\alpha^{-1/2}\,\varepsilon)\ln{\varepsilon}\Big| = \Big|\frac{K_n(\alpha^{-1/2}\,R)}{I_n(\alpha^{-1/2}\,R)}B_{0, n}^\text{p}(R) \Big(\frac{2^{-n}\alpha^{-n/2}}{n!} \varepsilon^n + \varepsilon^n\,r(\varepsilon) \Big)\ln{\varepsilon}\Big| \to_{\varepsilon\to 0} 0. $$
%     We get the result.
% \end{proof}
% \newpage

\begin{proposition} For $h$ in $L^2(B_R)$, we set,
    \[ \delta v^{h,0}(r) := -A_{0,0} \frac{I_0(\alpha^{-1/2}\, R)K_0(\alpha^{-1/2}r) - K_0(\alpha^{-1/2}R)I_0(\alpha^{-1/2}r)}{I_0(\alpha^{-1/2}\,R)}, \]
    where $A_{0,0}$ is defined in Proposition \ref{prop:solution-unhomo}. Then, for $\varepsilon$ sufficiently small, we have the following asymptotic estimation,
    \[ v_\varepsilon^{h,0}(r, \theta) - v_0^{h,0}(r, \theta) - \frac{-1}{\ln{\varepsilon}}\delta v^{h,0}(r) = o\left(\frac{-1}{\ln{\varepsilon}}\right). \]
\end{proposition}
\begin{proof} We have,
     $$ v_\varepsilon^{h,0}(r, \theta) - v_0^{h,0}(r, \theta) = \big( A_{\varepsilon,0} - A_{0,0} \big) I_0(\alpha^{-1/2}\,r) + B_{\varepsilon,0} K_0(\alpha^{-1/2}\,r) + R_{\varepsilon}(r,\theta), $$
    and,
    $$ R_{\varepsilon}(r,\theta) := \sum_{n\in\mathbb{Z}^*} \Big( \big( A_{\varepsilon,n} - A_{0,n} \big) I_n(\alpha^{-1/2}\,r) + B_{\varepsilon,n} K_n(\alpha^{-1/2}\,r) \Big)\,e^{in\theta}. $$
    We have, for all $n$ in $\Z$,
    $$ A_{\varepsilon,n} - A_{0,n} = -A_{0,n} \frac{I_n(\alpha^{-1/2}\,\varepsilon)K_n(\alpha^{-1/2}\,R)}{I_n(\alpha^{-1/2}\,\varepsilon)K_n(\alpha^{-1/2}\,R) - K_n(\alpha^{-1/2}\,\varepsilon)I_n(\alpha^{-1/2}\,R)}, $$
    and,
    $$ B_{\varepsilon,n} = A_{0,n} \frac{I_n(\alpha^{-1/2}\varepsilon)  I_n(\alpha^{-1/2}\,R) }{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - K_n(\alpha^{-1/2}\varepsilon)I_n(\alpha^{-1/2}R)}. $$
    Thus, 
    $$ v_\varepsilon^{h,0}(r, \theta) - v_0^{h,0}(r, \theta) = -\delta v^{h,0}(r) \frac{ I_0(\alpha^{-1/2}\,R) I_0(\alpha^{-1/2}\,\varepsilon) }{I_0(\alpha^{-1/2}\,\varepsilon)K_0(\alpha^{-1/2}\,R) - K_0(\alpha^{-1/2}\,\varepsilon)I_0(\alpha^{-1/2}\,R)} + R_{\varepsilon}(r), $$
    and,
    $$ R_{\varepsilon}(r,\theta) := -\sum_{n\in\mathbb{Z}^*} A_{0,n} \frac{I_n(\alpha^{-1/2}\,\varepsilon)\Big( I_n(\alpha^{-1/2}\,r)K_n(\alpha^{-1/2}\,R) - K_n(\alpha^{-1/2}\,r)I_n(\alpha^{-1/2}\,R) \Big) }{I_n(\alpha^{-1/2}\,\varepsilon)K_n(\alpha^{-1/2}\,R) - K_n(\alpha^{-1/2}\,\varepsilon)I_n(\alpha^{-1/2}\,R)}\,e^{in\theta}. $$
    We use that, \cite{Abramowitz1972},
    \[ K_0(x) = -(\gamma-\ln{2} + \ln{x}) I_0(x) + x r_1(x), \]
    and get,
    $$ v_\varepsilon^{h,0}(r, \theta) - v_0^{h,0}(r, \theta) = -\delta v^{h,0}(r) \Big( M + \ln{\varepsilon} + \varepsilon r_2(\varepsilon) \Big)^{-1} + R_{\varepsilon}(r). $$
    where, \[ M := \frac{K_0(\alpha^{-1/2}R) + I_0(\alpha^{-1/2}R)\big(\gamma-\ln{2} + \ln{(\alpha^{-1/2})} \big)}{I_0(\alpha^{-1/2} R)}, \]
    is a constant independent of $\epsilon$. It remains to show that $R_\varepsilon(r,\theta) = o\left(\frac{-1}{\ln{\varepsilon}}\right)$. We have,
    $$ R_\varepsilon(r,\theta) := \frac{-1}{\ln{\varepsilon}}\Theta_\varepsilon(r,\theta), $$
    where,
    $$ \Theta_\varepsilon(r,\theta) := \sum_{n\in\mathbb{Z}^*} \ln{\varepsilon} \frac{ K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}r) - I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}r)}{I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R) - I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}\varepsilon)}I_n(\alpha^{-1/2}\varepsilon)\,A_{0,n}\,e^{in\theta}. $$
    Moreover,
    $$ \big|\Theta_\varepsilon(r,\theta)\big| \leq \sum_{n\in\mathbb{Z}^*} \big|\ln{\varepsilon}\big| \Bigg|\frac{ I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}r) - K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}r)}{ I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}\varepsilon) - I_n(\alpha^{-1/2}\varepsilon)K_n(\alpha^{-1/2}R)}\Bigg|\big|I_n(\alpha^{-1/2}\varepsilon)\big|\,\big|A_{0,n}\big|. $$
    Since $I_n$ is an increasing function and $K_n$ is a decreasing function, we have, for $r\in[\varepsilon,R]$,
    $$ \big|I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}r) - K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}r)\big| \leq \big|I_n(\alpha^{-1/2}R)K_n(\alpha^{-1/2}\varepsilon) - K_n(\alpha^{-1/2}R)I_n(\alpha^{-1/2}\varepsilon)\big|. $$
    Thus,
    $$ \big|\Theta_\varepsilon(r,\theta)\big| \leq \sum_{n\in\mathbb{Z}^*} \big|\ln{\varepsilon}\big| \big|I_n(\alpha^{-1/2}\varepsilon)\big|\,\big|A_{0,n}\big|. $$
    Finally, using that, $$ I_n(\alpha^{-1/2} \varepsilon) = \frac{1}{n!}\left(\frac{\alpha^{-1/2}}{2}\right)^n \varepsilon^n + \varepsilon^n\,r(\varepsilon), $$
    we have that $\Theta_\varepsilon$ tends to $0$ when $\varepsilon$ goes to $0$.
\end{proof}

% \newpage

Using the previous result and the property of the Wronskian \cite{Abramowitz1972}, we have the following: \\

\begin{proposition} For $h$ in $L^2(B_R)$, we define,
    \[ \delta h(h) := -A_{0,0}\frac{1}{R\,I_0(\alpha^{-1/2}\,R)}. \]
    where $A_{0,0}$ is defined in Proposition \ref{prop:solution-unhomo}. Then, for $\varepsilon$ sufficiently small, we have the following asymptotic estimation,
    \[  \left\|h_\varepsilon - h_0 - \frac{-1}{\ln{\varepsilon}}\delta h\right\|_{-1/2,\partial B_R} = o\left(\frac{-1}{\ln{\varepsilon}}\right). \]
\end{proposition}

Finally, we can derive from the previous proposition the variations of the linear form: \\

\begin{proposition} For $h$ in $L^2(B_R)$, we define,
    \[ \delta l(w) := -\alpha A_{0,0}\frac{w^\text{mean}}{I_0(\alpha^{-1/2} R)}. \]
    Then, for $\varepsilon$ sufficiently small, we have the following asymptotic estimation,
    \[ \left|l_\varepsilon(w) - l_0(w) - \frac{-2\pi}{\ln{\varepsilon}}\delta l(w)\right| = o\left(\frac{-1}{\ln{\varepsilon}}\right)\,\|w\|_{V_R},\ \forall w \in V_R. \]
\end{proposition}


\begin{comment}


\newpage
\color{red}
\subsection{Variations of the Linear Form}

%Then, we give the following lemma, \\

\begin{lemma} For $\varepsilon$ small enough, we have,
    \[ \|h_\varepsilon - h_0 - \varepsilon^{1/2}\delta h\|_{-1/2,\partial B_R} = O\big(\varepsilon^{1/2}\big). \]
    \label{prop:variation-g}
\end{lemma}
\begin{proof}
    We set for  $x\in \R^2\setminus B_\varepsilon$,
    \[ \Psi_\varepsilon^{h,0} := v_\varepsilon^{h,0} - v_0^{h,0} + \varepsilon^{1/2}\, v_\omega^{h,0}. \]
    Thus, $\Psi_\varepsilon^{h,0}$ is the solution of
    \[ \left \{ \begin{array}{cl}
        -\alpha\Delta \Psi_\varepsilon^{h,0} + \Psi_\varepsilon^{h,0} = 0, & \text{in}\ B_R\setminus B_\varepsilon, \\
        \Psi_\varepsilon^{h,0} = \varepsilon^{1/2}v_\omega^{h,0} - v_0^{h,0}, & \text{on}\ \partial B_\varepsilon, \\
        \Psi_\varepsilon^{h,0} = \varepsilon^{1/2}\, v_\omega^{h,0}, & \text{on}\ \partial B_R.
    \end{array} \right .\]
  %  To apply Proposition \ref{prop:v-epsilon-estimates}, we have to verify that $(\varepsilon^{1/2}v_\omega^{h,0} - v_0^{h,0})$ is in $H^{1/2}(\partial B_\varepsilon)$ and that $\varepsilon^{1/2}\, v_\omega^{h,0}$ is in $H^{1/2}(\partial B_R)$.
 %   \[ \|\varepsilon^{1/2}\, v_\omega^{h,0}\|_{1/2,\partial B_R} = C\,\varepsilon^{1/2}\,|v_0^{h,0}(x_0)| \leq C'\,\varepsilon^{1/2}\,\|h\|_{L^2(D)}. \]
    % D'après la Proposition A.2. et la Proposition B.6., on a
    % \begin{align*}
    %     \| \varepsilon\, v_\omega^{h,0}(\cdot/\varepsilon)\|_{1/2,\partial B_R} & \leq \varepsilon^2\,\| v_\omega^{h,0}\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon| v_\omega^{h,0}|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \\
    %     %
    %     & \leq C\Big( \varepsilon^{5/2}\|v_0^{h,0}(x_0)\|_{1/2,\partial B_1} + \varepsilon^{3/2}\|v_0^{h,0}(x_0)\|_{1/2,\partial B_1} \Big) \\
    %     %
    %     & \leq C \varepsilon^{3/2}|v_0^{h,0}(x_0)| \\
    %     %
    %     & \leq C\,\varepsilon^{3/2}\,\|v_0^{h,0}\|_{\mathcal{C}^0} \\
    %     %
    %     & \leq C\,\varepsilon^{3/2}\,\|v_0^{h,0}-g+g\|_{\mathcal{C}^0} \\
    %     %
    %     & \leq C\,\varepsilon^{3/2}\,\|g\|_{L^?(D)}?
    % \end{align*}
  %  Then,
   % \[ \|\varepsilon^{1/2}v_\omega^{h,0}(\varepsilon\ \cdot) - v_0^{h,0}(\varepsilon\ \cdot)\|_{1/2,\partial B_1} \leq  \|\varepsilon^{1/2}v_\omega^{h,0}(\varepsilon\ \cdot) - v_0^{h,0}(x_0)\|_{1/2,\partial B_1} + \|v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\ \cdot)\|_{1/2,\partial B_1}. \]
  %  \begin{align*}
   %     \|\varepsilon^{1/2}v_\omega^{h,0}(\varepsilon\ \cdot) - v_0^{h,0}(x_0)\|_{1/2,\partial B_1} & \leq \varepsilon^{1/2}\|v_\omega^{h,0}(\varepsilon\ \cdot)\|_{1/2,\partial B_1} + \|v_0^{h,0}(x_0)\|_{1/2,\partial B_1} \\
        %
   %     & \leq \varepsilon^{1/2}\|v_\omega^{h,0}(\varepsilon\ \cdot)\|_{0,B_1\setminus B_{1/2}} + \varepsilon^{1/2}|v_\omega^{h,0}(\varepsilon\ \cdot)|_{1,B_1\setminus B_{1/2}} + C\,|v_0^{h,0}(x_0)| \\
        %
   %     & \leq \varepsilon^{1/2}\|v_\omega^{h,0}\|_{0,B_\varepsilon\setminus B_{\varepsilon/2}} + |v_\omega^{h,0}|_{1,B_\varepsilon\setminus B_{\varepsilon/2}} + C\,|v_0^{h,0}(x_0)| \\
        %
    %    & \leq \varepsilon^{1/2}\|v_\omega^{h,0}\|_{0,B_R} + |v_\omega^{h,0}|_{1,B_R} + C\,|v_0^{h,0}(x_0)| \\
        %
   %     & \leq C\,|v_0^{h,0}(x_0)| \\
        %
   %     & \leq C\,\|h\|_{L^2(D)}.
  %  \end{align*}
  %  And
  %  \begin{align*}
   %     \|v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} & = \varepsilon\left\|\varepsilon^{-1} \left(v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\,\cdot)\right)\right\|_{1/2,\partial B_1} \\
        %
   %     & \leq C\,\varepsilon\,\|v_0^{h,0}\|_{\mathcal{C}^1(B_{R/2})} \\
        %
   %     & \leq C\,\varepsilon\,\|h\|_{L^2(D)}.
    % \end{align*}
    % \begin{align*}
    %     \|v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} & = \varepsilon\left\|\varepsilon^{-1} \left(v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\,\cdot)\right)\right\|_{1/2,\partial B_1} \\
    %     %
    %     & \leq C\,\varepsilon\,\|v_0^{h,0}\|_{\mathcal{C}^1(B_{R/2})} \\
    %     %
    %     & \leq C\,\varepsilon\,\|g\|_{L^2(D)}?
    % \end{align*}
  %  We can now apply Proposition \ref{prop:v-epsilon-estimates},
  %  \begin{align*}
   %     \|\Psi_\varepsilon^{h,0}\|_{1,B_R\setminus B_{R/2}} & \leq C\,\big(\|\varepsilon^{1/2}\, v_\omega^{h,0}\|_{1/2,\partial B_R} + e^{-R/(2\varepsilon\sqrt{\alpha})}\|\varepsilon^{1/2}v_\omega^{h,0}(\varepsilon\ \cdot) - v_0^{h,0}(\varepsilon\ \cdot)\|_{1/2,\partial B_1}\big) \\
        %
   %     & \leq C\,\varepsilon^{1/2}\,\|h\|_{L^2(D)}.
   % \end{align*}
  %  To conclude, Proposition \ref{prop:norm-minus-1-2} gives,
  %  
    Tedious computations similar to the proof of the previous lemma, lead to 
    \begin{align*}
        \|h_\varepsilon - h_0 - \varepsilon^{1/2}\delta h\|_{-1/2,\partial B_R} & = \|\nabla\big( v_\varepsilon^{h,0} - v_0^{h,0} + \varepsilon^{1/2}\,v_\omega^{h,0} \big)\cdot n\|_{-1/2,\partial B_R} \\
        %
        & = \|\nabla \Psi_\varepsilon^{h,0}\cdot n\|_{-1/2,\partial B_R} \\
        %
        & \leq C\,\|\Psi_\varepsilon^{h,0}\|_{1,B_R\setminus B_{R/2}} \\
        %
        & \leq C\,\varepsilon^{1/2}\,\|h\|_{L^2(D)}.
    \end{align*}
\end{proof}

This Lemma \ref{prop:variation-g} gives the asymptotic expansion for the linear form : \\

\begin{proposition}
    % Soit $g\in L^?(D)$. Soit $v_\omega^{h,0}$ la solution du problème extérieur 
    
    % \[ \left \{ \begin{array}{cc}
    %     -\alpha\Delta v_\omega^{h,0} + v_\omega^{h,0} = 0, & \text{dans}\ \R^2\setminus B(x_0,1), \\
    %     v_\omega^{h,0} = v_0^{h,0}(x_0), & \text{sur}\ \partial B(x_0,1), \\
    %     v_\omega^{h,0} = 0, & \text{à}\ \infty.
    % \end{array} \right .\]
    We set
    \[ \delta h = \nabla v_\omega^{h,0} \cdot n. \]
    let $w$ be in $V_R$, we set,
    \[ \delta l(w) := \alpha\int_{\partial B_R} \delta h \, w\ d\sigma. \]
    Then, for $\varepsilon$ small enough, we have,
    \[ \|l_\varepsilon - l_0 - \varepsilon^{1/2}\,\delta l\|_{\mathcal{L}(V_R)} = O(\varepsilon^{1/2}). \]
\end{proposition}
%\begin{proof} Let $w\in V_R$, we have, 
 %   \begin{align*}
%        l_\varepsilon(w) - l_0(w) %& = \int_{D\setminus B_R} h w\ dx + \alpha\int_{\partial B_R} h_\varepsilon w\ d\sigma %- \int_{D\setminus B_R} h w\ dx - \alpha\int_{\partial B_R} h_0 w\ d\sigma \\
%        %
%        & = \alpha\int_{\partial B_R} (h_\varepsilon-h_0)\, w\ d\sigma.
 %   \end{align*}
%    The result follows from Lemma \ref{prop:variation-g}.
    %To be able to conclude, we need to use Proposition \ref{prop:variation-g}.
%\end{proof}
% \begin{note} Pour $|y|\geq 1$,
%     \[ v_\omega^{h,0}(y) = \frac{v_0^{h,0}(x_0)}{K_0\left(\alpha^{-1/2}\right)} K_0\left(\alpha^{-1/2}|y-x_0|\right), \]
    
%     d'où
    
%     \begin{align*}
%         \delta g & = \frac{v_0^{h,0}(x_0)}{K_0\left(\alpha^{-1/2}\right)} \nabla K_0\left(\alpha^{-1/2}|y-x_0|\right) \cdot n \\
%          %
%         & = -\alpha^{-1/2}\frac{v_0^{h,0}(x_0)}{K_0\left(\alpha^{-1/2}\right)} K_1\left(\alpha^{-1/2}|y-x_0|\right),
%     \end{align*}

%     et pour $w$ dans $V_R$,
    
%     \begin{align*}
%         \delta l(w) & := \int_{\partial B_R} \delta g\, w\ d\sigma \\
%         %
%         & = -\alpha^{-1/2}\frac{v_0^{h,0}(x_0)}{K_0\left(\alpha^{-1/2}\right)} \int_{\partial B_R} K_1\left(\alpha^{-1/2}|y-x_0|\right)\, w\ d\sigma \\
%         %
%         & = -\alpha^{-1/2}\frac{v_0^{h,0}(x_0)}{K_0\left(\alpha^{-1/2}\right)} K_1\left(\alpha^{-1/2}R\right) \int_{\partial B_R} w\ d\sigma.
%     \end{align*}
% \end{note}

% \begin{proof}
%     We set for  $x\in \R^2\setminus B_\varepsilon$,
%     \[ \Psi_\varepsilon^{h,0} := v_\varepsilon^{h,0} - v_0^{h,0} + \varepsilon^{1/2}\, v_\omega^{h,0}. \]
%     Thus, $\Psi_\varepsilon^{h,0}$ is the solution of
%     \[ \left \{ \begin{array}{cl}
%         -\alpha\Delta \Psi_\varepsilon^{h,0} + \Psi_\varepsilon^{h,0} = 0, & \text{in}\ B_R\setminus B_\varepsilon, \\
%         \Psi_\varepsilon^{h,0} = \varepsilon^{1/2}v_\omega^{h,0} - v_0^{h,0}, & \text{on}\ \partial B_\varepsilon, \\
%         \Psi_\varepsilon^{h,0} = \varepsilon^{1/2}\, v_\omega^{h,0}, & \text{on}\ \partial B_R.
%     \end{array} \right .\]
%     To apply Proposition \ref{prop:v-epsilon-estimates} in Appendix \ref{app:lp}, we have to verify that $(\varepsilon^{1/2}v_\omega^{h,0} - v_0^{h,0})$ is in $H^{1/2}(\partial B_\varepsilon)$ and that $\varepsilon^{1/2}\, v_\omega^{h,0}$ is in $H^{1/2}(\partial B_R)$.
%     \[ \|\varepsilon^{1/2}\, v_\omega^{h,0}\|_{1/2,\partial B_R} = C\,\varepsilon^{1/2}\,|v_0^{h,0}(x_0)| \leq C'\,\varepsilon^{1/2}\,\|h\|_{L^2(D)}. \]
%     % D'après la Proposition A.2. et la Proposition B.6., on a
%     % \begin{align*}
%     %     \| \varepsilon\, v_\omega^{h,0}(\cdot/\varepsilon)\|_{1/2,\partial B_R} & \leq \varepsilon^2\,\| v_\omega^{h,0}\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon| v_\omega^{h,0}|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \\
%     %     %
%     %     & \leq C\Big( \varepsilon^{5/2}\|v_0^{h,0}(x_0)\|_{1/2,\partial B_1} + \varepsilon^{3/2}\|v_0^{h,0}(x_0)\|_{1/2,\partial B_1} \Big) \\
%     %     %
%     %     & \leq C \varepsilon^{3/2}|v_0^{h,0}(x_0)| \\
%     %     %
%     %     & \leq C\,\varepsilon^{3/2}\,\|v_0^{h,0}\|_{\mathcal{C}^0} \\
%     %     %
%     %     & \leq C\,\varepsilon^{3/2}\,\|v_0^{h,0}-g+g\|_{\mathcal{C}^0} \\
%     %     %
%     %     & \leq C\,\varepsilon^{3/2}\,\|g\|_{L^?(D)}?
%     % \end{align*}
%     Then,
%     \[ \|\varepsilon^{1/2}v_\omega^{h,0}(\varepsilon\ \cdot) - v_0^{h,0}(\varepsilon\ \cdot)\|_{1/2,\partial B_1} \leq  \|\varepsilon^{1/2}v_\omega^{h,0}(\varepsilon\ \cdot) - v_0^{h,0}(x_0)\|_{1/2,\partial B_1} + \|v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\ \cdot)\|_{1/2,\partial B_1}. \]
%     \begin{align*}
%         \|\varepsilon^{1/2}v_\omega^{h,0}(\varepsilon\ \cdot) - v_0^{h,0}(x_0)\|_{1/2,\partial B_1} & \leq \varepsilon^{1/2}\|v_\omega^{h,0}(\varepsilon\ \cdot)\|_{1/2,\partial B_1} + \|v_0^{h,0}(x_0)\|_{1/2,\partial B_1} \\
%         %
%         & \leq \varepsilon^{1/2}\|v_\omega^{h,0}(\varepsilon\ \cdot)\|_{0,B_1\setminus B_{1/2}} + \varepsilon^{1/2}|v_\omega^{h,0}(\varepsilon\ \cdot)|_{1,B_1\setminus B_{1/2}} + C\,|v_0^{h,0}(x_0)| \\
%         %
%         & \leq \varepsilon^{1/2}\|v_\omega^{h,0}\|_{0,B_\varepsilon\setminus B_{\varepsilon/2}} + |v_\omega^{h,0}|_{1,B_\varepsilon\setminus B_{\varepsilon/2}} + C\,|v_0^{h,0}(x_0)| \\
%         %
%         & \leq \varepsilon^{1/2}\|v_\omega^{h,0}\|_{0,B_R} + |v_\omega^{h,0}|_{1,B_R} + C\,|v_0^{h,0}(x_0)| \\
%         %
%         & \leq C\,|v_0^{h,0}(x_0)| \\
%         %
%         & \leq C\,\|h\|_{L^2(D)}.
%     \end{align*}
%     And
%     \begin{align*}
%         \|v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} & = \varepsilon\left\|\varepsilon^{-1} \left(v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\,\cdot)\right)\right\|_{1/2,\partial B_1} \\
%         %
%         & \leq C\,\varepsilon\,\|v_0^{h,0}\|_{\mathcal{C}^1(B_{R/2})} \\
%         %
%         & \leq C\,\varepsilon\,\|h\|_{L^2(D)}.
%     \end{align*}
%     % \begin{align*}
%     %     \|v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} & = \varepsilon\left\|\varepsilon^{-1} \left(v_0^{h,0}(x_0) - v_0^{h,0}(\varepsilon\,\cdot)\right)\right\|_{1/2,\partial B_1} \\
%     %     %
%     %     & \leq C\,\varepsilon\,\|v_0^{h,0}\|_{\mathcal{C}^1(B_{R/2})} \\
%     %     %
%     %     & \leq C\,\varepsilon\,\|g\|_{L^2(D)}?
%     % \end{align*}
%     We can now apply Proposition \ref{prop:v-epsilon-estimates} in Appendix \ref{app:lp},
%     \begin{align*}
%         \|\Psi_\varepsilon^{h,0}\|_{1,B_R\setminus B_{R/2}} & \leq C\,\big(\|\varepsilon^{1/2}\, v_\omega^{h,0}\|_{1/2,\partial B_R} + e^{-R/(2\varepsilon\sqrt{\alpha})}\|\varepsilon^{1/2}v_\omega^{h,0}(\varepsilon\ \cdot) - v_0^{h,0}(\varepsilon\ \cdot)\|_{1/2,\partial B_1}\big) \\
%         %
%         & \leq C\,\varepsilon^{1/2}\,\|h\|_{L^2(D)}.
%     \end{align*}
%     To conclude, Proposition \ref{prop:norm-minus-1-2} in Appendix \ref{app:lp} gives,
%     \begin{align*}
%         \|h_\varepsilon - h_0 - \varepsilon^{1/2}\delta h\|_{-1/2,\partial B_R} & = \|\nabla\big( v_\varepsilon^{h,0} - v_0^{h,0} + \varepsilon^{1/2}\,v_\omega^{h,0} \big)\cdot n\|_{-1/2,\partial B_R} \\
%         %
%         & = \|\nabla \Psi_\varepsilon^{h,0}\cdot n\|_{-1/2,\partial B_R} \\
%         %
%         & \leq C\,\|\Psi_\varepsilon^{h,0}\|_{1,B_R\setminus B_{R/2}} \\
%         %
%         & \leq C\,\varepsilon^{1/2}\,\|h\|_{L^2(D)}.
%     \end{align*}
% \end{proof}

\color{black}

\newpage \color{red}
\subsection{Variations of the Cost Function} 

Finally, we give the asymptotic development of the variations of the cost function. We start, by giving an estimate of the variations of the solution with the proposition below : \\

\begin{proposition} 
    % Soit $\varphi\in H^{1/2}(\partial B_R)$ et $g\in ?$. Soit $v_\omega^{0,\phi}$ la solution du problème extérieur 
    
    % \[ \left \{ \begin{array}{cc}
    %     -\alpha\Delta v_\omega^{h,\phi} + v_\omega^{h,\phi} = 0, & \text{dans}\ \R^2\setminus B(x_0,1), \\
    %     v_\omega^{h,\phi} = v_0^{h,\phi}(x_0), & \text{sur}\ \partial B(x_0,1), \\
    %     v_\omega^{h,\phi} = 0, & \text{à}\ \infty.
    % \end{array} \right .\]
    We set
    \[ \delta v^{h,\phi} := -v_\omega^{h,\phi}. \]
    Then, for $\varepsilon$ small enough, we have,
    \[ \|v_\varepsilon^{h,\phi} - v_0^{h,\phi} - \varepsilon^{1/2}\,\delta v^{h,\phi}\|_{0,B_R\setminus B_\varepsilon} = o(\varepsilon^{1/2}). \]
\end{proposition}
\begin{proof}
    We proceed as in the previous lemmas, and set for $x\in\R^2\setminus B_\varepsilon$,
    \[ \Psi_\varepsilon^{h,\phi} := v_\varepsilon^{h,\phi} - v_0^{h,\phi} + \varepsilon^{1/2}\,v_\omega^{h,\phi}. \]
    Thus, $\Psi_\varepsilon^{h,\phi}$ is the solution of
    \[ \left \{ \begin{array}{cl}
        -\alpha\Delta \Psi_\varepsilon^{h,\phi} + \Psi_\varepsilon^{h,\phi} = 0, & \text{in}\ B_R\setminus B_\varepsilon, \\
        \Psi_\varepsilon^{h,\phi} = \varepsilon^{1/2}v_\omega^{h,\phi} - v_0^{h,\phi}, & \text{on}\ \partial B_\varepsilon, \\
        \Psi_\varepsilon^{h,\phi} = \varepsilon^{1/2}\, v_\omega^{h,\phi}, & \text{on}\ \partial B_R.
    \end{array} \right .\]
    using Proposition \ref{prop:v-epsilon-estimates}, we get 
    %need to check that $(\varepsilon^{1/2}v_\omega^{h,\phi} - v_0^{h,\phi})$ is in $H^{1/2}(\partial B_\varepsilon)$ and that $\varepsilon^{1/2}\, v_\omega^{h,\phi}$ is in $H^{1/2}(\partial B_R)$.
   % \[ \|\varepsilon^{1/2}\, v_\omega^{h,\phi}\|_{1/2,\partial B_R} \leq C\,\varepsilon^{1/2}\,\big(\|\phi\|_{1/2,\partial B_R} + \|h\|_{L^2(D)}\big). \]
   % Then,
   % \[ \|\varepsilon^{1/2}v_\omega^{h,\phi}(\varepsilon\,\cdot) - v_0^{h,\phi}(\varepsilon\,\cdot)\|_{1/2,\partial B_1} \leq C\,\big(\|\phi\|_{1/2,\partial B_R} + \|h\|_{L^2(D)}\big). \]
    %Therefore, we can use Proposition \ref{prop:v-epsilon-estimates},
    \begin{align*}
        \|\Psi_\varepsilon^{h,\phi}\|_{0,B_R\setminus B_\varepsilon} & \leq C\,\big(\|\varepsilon^{1/2}\, v_\omega^{h,\phi}\|_{1/2,\partial B_R} + e^{-R/(2\varepsilon\sqrt{\alpha})}\|\varepsilon^{1/2}v_\omega^{h,\phi}(\varepsilon\,\cdot) - v_0^{h,\phi}(\varepsilon\,\cdot)\|_{1/2,\partial B_1}\big) \\
        %
        & \leq C\,\varepsilon^{1/2}\,\big(\|\phi\|_{1/2,\partial B_R} + \|h\|_{L^2(D)}\big).
    \end{align*}
\end{proof}
% \begin{note}
%     \[ \delta v(y) := \frac{v_0^{h,\phi}(x_0)}{K_0\left(\alpha^{-1/2}\right)} K_0\left(\alpha^{-1/2}|y-x_0|/\varepsilon\right). \]
% \end{note}

% \begin{note}
%     Si $p=2$, $g(x,t) = \frac{1}{2} t^2$ et $g_s(x,t) = t$, d'où
    
%     \begin{align*}
%         g(x,t) - g(x,s) &= \frac{1}{2}(t^2-s^2) \\
%         %
%         & = \frac{1}{2}(t+s)(t-s) \\
%         %
%         & = \frac{1}{2}s(t-s) + \frac{1}{2}t(t-s) \\
%         %
%         & = s(t-s) - \frac{1}{2}s(t-s) + \frac{1}{2}t(t-s) \\
%         %
%         & = s(t-s) + \frac{1}{2}(t-s)^2 \\
%         %
%         & = g_s(x,s)(t-s) + \underbrace{\theta(x,s,t)}_{=:1/2\leq M/2}(t-s)^2.
%     \end{align*}
% \end{note}


% \begin{note}
%     Si $p=1$, $g(x,t) = |t|$ et $g_s(x,t) = \begin{cases} -1 & \text{si}\ t<0, \\ 1 & \text{sinon} \end{cases}$, d'où
    
%     \begin{align*}
%         g(x,t) - g(x,s) &= |t|-|s| \\
%         %
%         & = g_s(x,t)t - g_s(x,s)s \\
%         %
%         & = g_s(x,t)t - g_s(x,s)s + g_s(x,s)t - g_s(x,s)t \\
%         %
%         & = g_s(x,s)(t-s) + \big(g_s(x,t)-g_s(x,s)\big)t
%     \end{align*}
% \end{note}

% \begin{note}
%     $g(x,t)=\frac{1}{p}|t|^p$ et $\partial_t\, g(x,t)=t|t|^{p-2}$ et $\partial_{tt}\, g(x,t)=|t|^{p-2} + (p-2) t^2 |t|^{p-4}$
    
%     \[ g(t) = \frac{{\left| t \right|}^{p}}{p} \]
    
%     \[ g'(t) = \frac{t {\left| t \right|}^{p - 1}}{{\left| t \right|}} \]
    
%     \[ g''(t) = {\left(p - 1\right)} {\left| t \right|}^{p - 2} \]
    
%     \[ g'''(t) = \frac{{\left(p - 1\right)} {\left(p - 2\right)} t {\left| t \right|}^{p - 3}}{{\left| t \right|}} \]
    
%     d'où Taylor
    
%     \[ g(x,t) - g(x,t) = \partial_t g(x,s) (t-s) + \frac{1}{2}\partial_{tt} g(x,s) (t-s)^2 + \frac{1}{6}\partial_{ttt} g(x,s) (t-s)^3 + \hdots \]
%     \[ = s {\left| s \right|}^{p - 2} (t-s) + \frac{1}{2}{\left(p - 1\right)} {\left| s \right|}^{p - 2} (t-s)^2 + \frac{1}{6}\frac{{\left(p - 1\right)} {\left(p - 2\right)} s {\left| s \right|}^{p - 3}}{{\left| s \right|}} (t-s)^3 + \hdots \]

%     Donc si $p=2$ : 
    
%     \[ g(x,t) - g(x,t) = s(t-s) + \frac{1}{2} (t-s)^2 \]
    
%     et si $p=1$:

%     \[ g(x,t) - g(x,t) = s {\left| s \right|}^{-1} (t-s) + 0 (t-s)^2 \]
% \end{note}

Now we can state the estimate of the variations of the cost function. \\

\begin{proposition}
    We set for $v$ in $V_R$,
    \[ \delta J(v) := \int_{B_R} g_s(x,\widetilde{v}_0)\,\delta v^{h,v}\ dx - \alpha\int_{\partial B_R} \partial_n w_0\,\delta v^{h,v}\ d\sigma. \]
    Then, for $\varepsilon$ small enough, we have,
    \[ J_\varepsilon(v) - J_0(v) - \varepsilon^{1/2} \delta J(v)  = o(\varepsilon^{1/2}). \]
\end{proposition}
\begin{proof}
    Let $v\in V_R$, we consider its extension in $D$, namely $\widetilde{v}_0$, and in $D\setminus B_\varepsilon$, namely $\widetilde{v}_\varepsilon$. We remind that $\widetilde{v}_0$ and $\widetilde{v}_\varepsilon$ are not necessarily solutions of Problems \ref{pb:problem:v-D} and \ref{pb:problem:u-D}, respectively, since $v$ do not solve necessarily \ref{pb:problem:v-epsilon-outside}.
    \begin{align*}
        I_\varepsilon & := J_\varepsilon(v) - J_0(v) - \varepsilon^{1/2} \delta J(v) \\
        %
        & = \widetilde{J}_\varepsilon(\widetilde{v}_\varepsilon) - \widetilde{J}_0(\widetilde{v}_0) - \varepsilon^{1/2} \delta J(v) \\
        %
        & = \int_{D\setminus B_\varepsilon} g(x,\widetilde{v}_\varepsilon)\ dx - \int_D g(x,\widetilde{v}_0)\ dx - \varepsilon^{1/2} \int_{B_R} g_s(x,\widetilde{v}_0)\, \delta v^{h,v}\ dx + \varepsilon^{1/2} \alpha\int_{\partial B_R} \partial_n w_0\,\delta v^{h,v}\ d\sigma.
    \end{align*}
    Since $\widetilde{v}_\varepsilon = \widetilde{v}_0$ on $D\setminus B_R$,
    \begin{align*}
        I_\varepsilon & = \int_{B_R\setminus B_\varepsilon} \big(g(x,\widetilde{v}_\varepsilon) - g(x,\widetilde{v}_0)\big)\ dx - \int_{B_\varepsilon} g(x,\widetilde{v}_0)\ dx - \varepsilon^{1/2} \int_{B_R} g_s(x,\widetilde{v}_0)\, \delta v^{h,v}\ dx + \varepsilon^{1/2} \alpha\int_{\partial B_R} \partial_n w_0\,\delta v^{h,v}\ d\sigma.
    \end{align*} 
    Using Proposition \ref{prop:g},
    \begin{align*}
        I_\varepsilon & = \int_{B_R\setminus B_\varepsilon} g_s(x,\widetilde{v}_0)(\widetilde{v}_\varepsilon - \widetilde{v}_0)\ dx + \int_{B_R\setminus B_\varepsilon} \theta(x,\widetilde{v}_0,\widetilde{v}_\varepsilon)(\widetilde{v}_\varepsilon - \widetilde{v}_0)^2\ dx - \int_{B_\varepsilon} g(x,\widetilde{v}_0)\ dx \\ & \hspace{3cm} - \varepsilon^{1/2} \int_{B_R} g_s(x,\widetilde{v}_0)\, \delta v^{h,v}\ dx + \varepsilon^{1/2} \alpha\int_{\partial B_R} \partial_n w_0\,\delta v^{h,v}\ d\sigma  \\
        %
        & = \int_{B_R\setminus B_\varepsilon} g_s(x,\widetilde{v}_0)(\widetilde{v}_\varepsilon - \widetilde{v}_0 - \varepsilon^{1/2}\delta v^{h,v})\ dx + \varepsilon^{1/2}\int_{B_R\setminus B_\varepsilon} g_s(x,\widetilde{v}_0)\,\delta v^{h,v}\ dx \\ & \hspace{3cm} + \int_{B_R\setminus B_\varepsilon} \theta(x,\widetilde{v}_0,\widetilde{v}_\varepsilon)(\widetilde{v}_\varepsilon - \widetilde{v}_0)^2\ dx - \int_{B_\varepsilon} g(x,\widetilde{v}_0)\ dx \\ & \hspace{3cm} - \varepsilon^{1/2} \int_{B_R} g_s(x,\widetilde{v}_0)\, \delta v^{h,v}\ dx + \varepsilon^{1/2} \alpha\int_{\partial B_R} \partial_n w_0\,\delta v^{h,v}\ d\sigma \\
        %
        % & = \int_{B_R\setminus B_\varepsilon} g_s(x,\widetilde{v}_0)(\widetilde{v}_\varepsilon - \widetilde{v}_0 - \varepsilon^{1/2}\delta v^{h,v})\ dx - \varepsilon^{1/2}\int_{B_R\setminus B_\varepsilon} g_s(x,\widetilde{v}_0)\,v_\omega^{h,v}\ dx \\ & \hspace{3cm} + \int_{B_R\setminus B_\varepsilon} \theta(x,\widetilde{v}_0,\widetilde{v}_\varepsilon)(\widetilde{v}_\varepsilon - \widetilde{v}_0)^2\ dx - \int_{B_\varepsilon} g(x,\widetilde{v}_0)\ dx \\ & \hspace{3cm} + \varepsilon^{1/2} \int_{B_R} g_s(x,\widetilde{v}_0)\, v_\omega^{h,v}\ dx - \varepsilon^{1/2} \alpha\int_{\partial B_R} \partial_n w_0\,v_\omega^{h,v}\ d\sigma \\
        %
        & = \int_{B_R\setminus B_\varepsilon} g_s(x,\widetilde{v}_0)(\widetilde{v}_\varepsilon - \widetilde{v}_0 - \varepsilon^{1/2}\delta v^{h,v})\ dx - \varepsilon^{1/2}\int_{B_\varepsilon} g_s(x,\widetilde{v}_0)\,\delta v^{h,v}\ dx \\ & \hspace{3cm} + \int_{B_R\setminus B_\varepsilon} \theta(x,\widetilde{v}_0,\widetilde{v}_\varepsilon)(\widetilde{v}_\varepsilon - \widetilde{v}_0)^2\ dx - \int_{B_\varepsilon} g(x,\widetilde{v}_0)\ dx + \varepsilon^{1/2} \alpha\int_{\partial B_R} \partial_n w_0\,\delta v^{h,v}\ d\sigma. \\
    \end{align*}
    Thus,
    \begin{align*}
        |I_\varepsilon| & \leq \int_{B_R\setminus B_\varepsilon}\left| g_s(x,\widetilde{v}_0)(\widetilde{v}_\varepsilon - \widetilde{v}_0 - \varepsilon^{1/2}\delta v^{h,v})\right|\ dx + \varepsilon^{1/2}\int_{B_\varepsilon} \left| g_s(x,\widetilde{v}_0)\,\delta v^{h,v}\right|\ dx \\ & \hspace{3cm} + \frac{M}{2} \int_{B_R\setminus B_\varepsilon} (\widetilde{v}_\varepsilon - \widetilde{v}_0)^2\ dx + \int_{B_\varepsilon} |g(x,\widetilde{v}_0)|\ dx + \varepsilon^{1/2} \alpha\int_{\partial B_R} \left| \partial_n w_0\,\delta v^{h,v}\right| \ d\sigma. \\
    \end{align*}
    and
    \begin{align*}
        & \bullet\hspace{0.5cm} \int_{B_R\setminus B_\varepsilon}\left| g_s(x,\widetilde{v}_0)(\widetilde{v}_\varepsilon - \widetilde{v}_0 - \varepsilon^{1/2}\delta v^{h,v})\right|\ dx \leq C\,\varepsilon^{1/2}. \\
        %
        & \bullet\hspace{0.5cm} \varepsilon^{1/2}\int_{B_\varepsilon} \left| g_s(x,\widetilde{v}_0)\,\delta v^{h,v}\right|\ dx \leq \varepsilon^{1/2} \int_{B_R} \left| g_s(x,\widetilde{v}_0)\,\delta v^{h,v}\right| \ dx \leq C\,\varepsilon^{1/2}. \\
        %
        & \bullet\hspace{0.5cm} \int_{B_R\setminus B_\varepsilon} (\widetilde{v}_\varepsilon - \widetilde{v}_0)^2\ dx = \int_{B_R\setminus B_\varepsilon} \big(\varepsilon^{1/2}\,\delta v^{h,v} + o(\varepsilon^{1/2})\big)^2\ dx = o(\varepsilon^{1/2})\int_{B_R\setminus B_\varepsilon}\ dx \leq o(\varepsilon^{1/2})\int_{B_R}\ dx \leq C\,\varepsilon^{1/2}. \\
        %
        & \bullet\hspace{0.5cm} \int_{B_\varepsilon} |g(x,\widetilde{v}_0)|\ dx \leq \left( \int_{B_\varepsilon} \big(g(x,\widetilde{v}_0)\big)^2\ dx \right)^{1/2}\left( \int_{B_\varepsilon} 1^2\ dx \right)^{1/2} \leq \left( \int_{B_R} \big(g(x,\widetilde{v}_0)\big)^2\ dx \right)^{1/2}\left( \int_{B_\varepsilon}\ dx \right)^{1/2} \leq C\,\varepsilon. \\
        %
        & \bullet\hspace{0.5cm} \varepsilon^{1/2}\int_{\partial B_R} \left| \partial_n w_0\,\delta v^{h,v} \right| \ d\sigma = C\,\varepsilon^{1/2}.
    \end{align*}
    Finally,
    \[ |I_\varepsilon| \leq C\,\varepsilon^{1/2}. \]
    % -------
    % \textbullet ~ \textbf{Si $\mathbf{p=2}$ :}
    % \begin{align*}
    %     I_\varepsilon & = \frac{1}{2}\int_{B_R\setminus B_\varepsilon} \Big((v_\varepsilon^{h,\phi})^2 - (v_0^{h,\phi})^2\Big)\ dx - \frac{1}{2}\int_{B_\varepsilon} (v_0^{h,\phi})^2\ dx - \varepsilon \int_{B_R} v_0^{h,\phi}\, \delta v\ dx \\
    %     %
    %     & = \int_{B_R\setminus B_\varepsilon} v_0^{h,\phi}(v_\varepsilon^{h,\phi} - v_0^{h,\phi})\ dx + \frac{1}{2}\int_{B_R\setminus B_\varepsilon}(v_\varepsilon^{h,\phi} - v_0^{h,\phi})^2\ dx - \frac{1}{2}\int_{B_\varepsilon} (v_0^{h,\phi})^2\ dx - \varepsilon \int_{B_R} v_0^{h,\phi}\, \delta v\ dx \\
    %     %
    %     & = \int_{B_R\setminus B_\varepsilon} v_0^{h,\phi}(v_\varepsilon^{h,\phi} - v_0^{h,\phi} - \varepsilon\,\delta v)\ dx + \frac{1}{2}\int_{B_R\setminus B_\varepsilon}(v_\varepsilon^{h,\phi} - v_0^{h,\phi})^2\ dx - \frac{1}{2}\int_{B_\varepsilon} (v_0^{h,\phi})^2\ dx - \varepsilon \int_{B_\varepsilon} v_0^{h,\phi}\, \delta v\ dx.
    % \end{align*}
    
    % D'où
    
    % \[ |I_\varepsilon| \leq \int_{B_R\setminus B_\varepsilon} |v_0^{h,\phi}|\,|v_\varepsilon^{h,\phi} - v_0^{h,\phi} - \varepsilon\,\delta v|\ dx + \frac{1}{2}\int_{B_R\setminus B_\varepsilon}(v_\varepsilon^{h,\phi} - v_0^{h,\phi})^2\ dx + \frac{1}{2}\int_{B_\varepsilon} (v_0^{h,\phi})^2\ dx + \varepsilon \int_{B_\varepsilon} |v_0^{h,\phi}|\,| \delta v|\ dx. \]

    % Mais 
    
    % \begin{align*}
    %     \int_{B_R\setminus B_\varepsilon} |v_0^{h,\phi}|\,|v_\varepsilon^{h,\phi} - v_0^{h,\phi} - \varepsilon\,\delta v|\ dx & \leq \|v_0^{h,\phi}\|_{0,B_R\setminus B_\varepsilon}\,\|v_\varepsilon^{h,\phi} - v_0^{h,\phi} - \varepsilon\,\delta v\|_{0,B_R\setminus B_\varepsilon} \\ 
    %     %
    %     & \leq \|v_0^{h,\phi}\|_{0,B_R}\,\|v_\varepsilon^{h,\phi} - v_0^{h,\phi} - \varepsilon\,\delta v\|_{0,B_R\setminus B_\varepsilon} \\ 
    %     %
    %     & \leq C\,\varepsilon^{3/2}.
    % \end{align*}
    
    % \begin{align*}
    %     \frac{1}{2}\int_{B_R\setminus B_\varepsilon}(v_\varepsilon^{h,\phi} - v_0^{h,\phi})^2\ dx & \leq C\,\varepsilon^2\ ?
    % \end{align*}
    
    % \begin{align*}
    %     \frac{1}{2}\int_{B_\varepsilon} (v_0^{h,\phi})^2\ dx & \leq \frac{1}{2}\,\|v_0^{h,\phi}\|_{\infty,B_R}^2\,\int_{B_\varepsilon} \ dx \\
    %     %
    %     & = C\,\varepsilon^2.
    % \end{align*}
    
    % \begin{align*}
    %     \varepsilon \int_{B_\varepsilon} |v_0^{h,\phi}|\,|\delta v|\ dx & \leq \varepsilon\,\|v_0^{h,\phi}\|_{0,B_\varepsilon}\,\|\delta v\|_{0,B_\varepsilon} \\
    %     %
    %     & \leq \varepsilon\,\|v_0^{h,\phi}\|_{0,B_R}\,\|\delta v\|_{0,B_\varepsilon} \\
    %     %
    %     & \leq C\,\varepsilon\,\|\delta v\|_{0,B_\varepsilon}. \\
    % \end{align*}
\end{proof}

Similar computations give, \\

\begin{proposition}
    $J_0$ is differentiable on $V_R$ and for $v,w$ in $V_R$, we have, for $\varepsilon$ small enough,
    \[ J_\varepsilon(w) - J_0(v) = \varepsilon^{1/2}\delta J(v) + D J_0(v)(w-v) + o(\varepsilon^{1/2} + \|w-v\|_{V_R}). \]
\end{proposition}
% \begin{proof}
%     By definition, $\widetilde{J}_0$ is differentiable on $H^1(D)$ and for all $\varphi$ in $H^1(D)$,
%     \[ D\widetilde{J}_0(\widetilde{v}_0)\varphi = \int_D g_s(x,\widetilde{v}_0)\,\varphi\ dx.  \]
%     Then, $J_0$ is differentiable on $V_R$ and if we note $\widetilde{\varphi}$ the extension on $H^1(D)$ of $\varphi\in V_R$ such that $-\alpha\Delta\widetilde{\varphi}+\widetilde{\varphi}=0$ in $B_R$, we have
%     \[ DJ_0(v_0)\,\varphi = D\widetilde{J}_0(\widetilde{v}_0)\,\widetilde{\varphi}. \]
%     Using the previous proposition, we get for $v,w$ in $V_R$,
%     \begin{align*}
%         J_\varepsilon(w) - J_0(v) & = J_\varepsilon(w) - J_0(w) + J_0(w) - J_0(v) \\
%         %
%         & = \varepsilon^{1/2} \delta J(w) + o(\varepsilon^{1/2}) + DJ_0(v)(w-v) + o(\|w-v\|_{V_R}) \\
%         %
%         & = \varepsilon^{1/2} \delta J(w) + \varepsilon^{1/2} \delta J(v) - \varepsilon^{1/2} \delta J(v) + DJ_0(v)(w-v) + o(\varepsilon^{1/2} + \|w-v\|_{V_R}) \\
%         %
%         & = \varepsilon^{1/2} \delta J(v) + DJ_0(v)(w-v) + \varepsilon^{1/2} \big(\delta J(w) - \delta J(v)\big) + o(\varepsilon^{1/2} + \|w-v\|_{V_R}).
%     \end{align*}
%     To conclude, it remains to show that $\varepsilon^{1/2} \big(\delta J(w) - \delta J(v)\big) = o(\varepsilon^{1/2} + \|w-v\|_{V_R})$.
%     \begin{align*}
%         \delta J(w) - \delta J(v) & = -\int_{B_R} g_s(x,\widetilde{w}_0)\,v_\omega^{h,w}\ dx + \alpha\int_{\partial B_R} \partial_n w_0\,v_\omega^{h,w}\ d\sigma + \int_{B_R} g_s(x,\widetilde{v}_0)\,v_\omega^{h,v}\ dx \\ & \hspace{3cm} - \alpha\int_{\partial B_R} \partial_n w_0\,v_\omega^{h,v}\ d\sigma \\
%         %
%         & = -\int_{B_R} g_s(x,\widetilde{w}_0)\,v_\omega^{h,w}\ dx + \int_{B_R} g_s(x,\widetilde{v}_0)\,v_\omega^{h,w}\ dx - \int_{B_R} g_s(x,\widetilde{v}_0)\,v_\omega^{h,w}\ dx \\ & \hspace{3cm} + \alpha\int_{\partial B_R} \partial_n w_0\,v_\omega^{h,w}\ d\sigma + \int_{B_R} g_s(x,\widetilde{v}_0)\,v_\omega^{h,v}\ dx - \alpha\int_{\partial B_R} \partial_n w_0\,v_\omega^{h,v}\ d\sigma \\
%         %
%         & = \int_{B_R} (g_s(x,\widetilde{v}_0)-g_s(x,\widetilde{w}_0))\,v_\omega^{h,w}\ dx + \int_{B_R} g_s(x,\widetilde{v}_0)\,(v_\omega^{h,v}-v_\omega^{h,w})\ dx \\ & \hspace{3cm} + \alpha\int_{\partial B_R} \partial_n w_0\,(v_\omega^{h,w}-v_\omega^{h,v})\ d\sigma.
%     \end{align*}
%     Then,
%     \begin{align*}
%         |\delta J(w) - \delta J(v)| & \leq \int_{B_R} |(g_s(x,\widetilde{v}_0)-g_s(x,\widetilde{w}_0))\,v_\omega^{h,w}|\ dx + \int_{B_R} |g_s(x,\widetilde{v}_0)\,(v_\omega^{h,v}-v_\omega^{h,w})|\ dx \\ & \hspace{3cm} + \alpha\int_{\partial B_R} |\partial_n w_0\,(v_\omega^{h,w}-v_\omega^{h,v})|\ d\sigma \\
%         %
%         & \leq \int_{B_R} M|\widetilde{v}_0-\widetilde{w}_0|\,|v_\omega^{h,w}|\ dx + \int_{B_R} M|\widetilde{v}_0|\,|v_\omega^{h,v}-v_\omega^{h,w}|\ dx \\ & \hspace{3cm} + \alpha\int_{\partial B_R} |\partial_n w_0\,(v_\omega^{h,w}-v_\omega^{h,v})|\ d\sigma.
%     \end{align*}
%     Finally,
%     \begin{align*}
%         & \bullet\hspace{0.5cm} \int_{B_R} M|\widetilde{v}_0-\widetilde{w}_0|\,|v_\omega^{h,w}|\ dx \leq C\,\|v_\omega^{h,w}\|_{L^2(B_R)}\,\|\widetilde{v}_0-\widetilde{w}_0\|_{L^2(B_R)} \leq C\,\|v-w\|_{V_R}. \\
%         %
%         & \bullet\hspace{0.5cm} \int_{B_R} M|\widetilde{v}_0|\,|v_\omega^{h,v}-v_\omega^{h,w}|\ dx \leq C\,\|v_\omega^{h,v}-v_\omega^{h,w}\|_{L^2(B_R)} \leq C'\,\|v-w\|_{V_R}. \\
%         %
%         & \bullet\hspace{0.5cm} \int_{\partial B_R} |\partial_n w_0\,(v_\omega^{h,w}-v_\omega^{h,v})|\ d\sigma \leq C\,\|v_\omega^{h,w}-v_\omega^{h,v}\|_{L^2(\partial B_R)} \leq C'\,\|w-v\|_{V_R}.
%     \end{align*}
%     We have the result.
% \end{proof}
% \begin{note}
%     \[ \delta v(y) := \frac{v_0^{h,\phi}(x_0)}{K_0\left(\alpha^{-1/2}\right)} K_0\left(\alpha^{-1/2}|y-x_0|/\varepsilon\right). \]
    
%     D'où,
    
%     \begin{align*}
%         \delta J &:= -\int_{B_R} |\widetilde{v}_0|^{p-2}\widetilde{v}_0\,\delta v\ dx \\
%         %
%         & = -\frac{v_0^{h,\phi}(x_0)}{K_0\left(\alpha^{-1/2}\right)} \int_{B_R} |\widetilde{v}_0|^{p-2}\widetilde{v}_0\, K_0\left(\alpha^{-1/2}|y-x_0|/\varepsilon\right)\ dx \\
%         %
%         & = -2\pi\frac{v_0^{h,\phi}(x_0)}{K_0\left(\alpha^{-1/2}\right)} \int_{B_R} |\widetilde{v}_0|^{p-2}\widetilde{v}_0\, E(|x-x_0|)\ dx.
%     \end{align*}
    
%     Théorie du potentiel : 
    
%     \[ \delta J = 2\pi\frac{v_0^{h,\phi}(x_0)}{K_0\left(\alpha^{-1/2}\right)} w(x_0). \]
% \end{note}

% \subsubsection{Variations de la fonction coût 2}

% \begin{proposition}
%     \[ J_\varepsilon(v_\varepsilon) = J_\varepsilon(v_0) + D J_\varepsilon(v_0)(v_\varepsilon-v_0) + f(\varepsilon) \delta J_1 + o(f(\varepsilon)). \]
% \end{proposition}
% \begin{proof}
%     \[ J_\varepsilon(v_\varepsilon) - J_\varepsilon(v_0) - D J_\varepsilon(v_0)(v_\varepsilon-v_0) = \tilde{J}_\varepsilon(\tilde{v}_\varepsilon) - \tilde{J}_\varepsilon(\widetilde{v}_0). \]
% \end{proof}

% \begin{proposition}
%     \[ J_\varepsilon(v_0) = J_0(v_0) + f(\varepsilon) \delta J_2 + o(f(\varepsilon)). \]
% \end{proposition}

% On a la proposition suivante, \\

% \begin{proposition}
%     \[ J_\varepsilon(v_\varepsilon) - J_\varepsilon(v_0) - DJ_\varepsilon(v_0)(v_\varepsilon - v_0) = f(\varepsilon)\delta J_1 + o\big( f(\varepsilon) \big), \]
% \end{proposition}
% \begin{proof}
%     \[ DJ_\varepsilon(v_0)(v_\varepsilon - v_0) = \int |v_0|^{p-2} v_0(v_\varepsilon - v_0)\ dx \]
    
%     D'où 
    
%     \[ J_\varepsilon(v_\varepsilon) - J_\varepsilon(v_0) - DJ_\varepsilon(v_0)(v_\varepsilon - v_0) = \frac{1}{p}\int_D |v_\varepsilon|^p\ dx - \frac{1}{p}\int_D |v_0|^p\ dx - \int |v_0|^{p-2} v_0(v_\varepsilon - v_0)\ dx \]
%     \[ = \frac{1}{p}\int_D |v_\varepsilon|^p\ dx - \frac{1}{p}\int_D |v_0|^p\ dx - \int |v_0|^{p-2} v_0\,v_\varepsilon\ dx + \int |v_0|^{p}\ dx \]
    
%     \[ = \frac{1}{p}\int_D |v_\varepsilon|^p\ dx + (1- \frac{1}{p})\int_D |v_0|^p\ dx - \int |v_0|^{p-2} v_0\,v_\varepsilon\ dx \]
    
%     \[ = \int_D \frac{1}{p}|v_\varepsilon|^{p-2}v_\varepsilon v_\varepsilon - |v_0|^{p-2} v_0\,v_\varepsilon\ dx + (1- \frac{1}{p})\int_D |v_0|^p\ dx \]
% \end{proof}

% \begin{proposition}
%     \[ J_\varepsilon(v_0) - J_0(v_0) = 0. \]
% \end{proposition}
% \begin{proof}
%     \[ J_\varepsilon(v_0) - J_0(v_0) = \tilde{J}_\varepsilon(\widetilde{v}_0) - \widetilde{J}_0(\widetilde{v}_0) = \frac{1}{p}\int_D |\widetilde{v}_0|^p\ dx - \frac{1}{p}\int_D |\widetilde{v}_0|^p\ dx = 0. \]
% \end{proof}

% \subsection{Brouillon}

% \[ E(x) = \frac{1}{2\pi}K_0(\alpha^{-1/2}|x|) \]

% \[ v_\omega = v_D(x_0) \frac{E(x-x_0)}{E(1)} = \frac{1}{K_0(\alpha^{-1/2})} v_D(x_0) K_0(\alpha^{-1/2}|x-x_0|) \]

% \begin{align*}
%     \delta a - \delta l & = -\int_{\partial B_R} \nabla v_\omega^{h,\phi} \cdot n \, w_D\ d\sigma \\
%     %
%     & = -\int_{\partial B_R} \nabla v_\omega^{h,\phi} \cdot n \, w_D\ d\sigma + \int_{B_R}\Delta w_D v_\omega|_{\partial B_R}\ dx - \int_{B_R}\Delta w_D v_\omega|_{\partial B_R}\ dx \\
%     %
%     & = -\int_{\partial B_R} \nabla v_\omega^{h,\phi} \cdot n \, w_D\ d\sigma - \int_{B_R}\nabla w_D\cdot\nabla v_\omega|_{\partial B_R}\ dx + \int_{\partial B_R}\partial_n w_D v_\omega|_{\partial B_R}\ d\sigma(x) - \int_{B_R}\Delta w_D v_\omega|_{\partial B_R}\ dx.
% \end{align*}

% Mais $\nabla v_\omega|_{\partial B_R} = 0$ et $v_\omega|_{\partial B_R} = v_\omega$ sur $\partial B_R$,

% \[ \delta a - \delta l = \int_{\partial B_R} \Big(\partial_n w_D v_\omega - \partial_n v_\omega^{h,\phi} w_D \Big)\ d\sigma - \int_{B_R}\Delta w_D v_\omega|_{\partial B_R}\ dx \]
% \[ = \int_{\partial B_R} \Big(\partial_n w_D v_\omega - \partial_n v_\omega^{h,\phi} w_D \Big)\ d\sigma - v_D(x_0) \frac{E(R)}{E(1)} \int_{B_R}\Delta w_D\ dx \]
% \[ = \int_{\partial B_R} \Big(\partial_n w_D v_\omega - \partial_n v_\omega^{h,\phi} w_D \Big)\ d\sigma - v_D(x_0) \frac{K_0(\alpha^{-1/2}R)}{K_0(\alpha^{-1/2})} \int_{B_R}\Delta w_D\ dx \]

% De plus,

% \begin{align*}
%     w_D(x_0) & = \int_{B_R} w_D(x)\delta_{x_0}(x)\ dx \\
%     %
%     & = \int_{B_R} w_D(x)\big(-\alpha\Delta E(x-x_0)+E(x-x_0)\big)\ dx \\
%     %
%     & = \int_{B_R} E(x-x_0)\big(-\alpha\Delta w_D(x)+w_D(x)\big)\ dx + \alpha\int_{\partial B_R} \Big(\partial_n w_D(x) E(x-x_0) - \partial_n E(x-x_0) w_D(x)\Big)\ d\sigma(x). \\
% \end{align*}

% D'où 

% \[ \alpha\int_{\partial B_R} \Big(\partial_n w_D(x) E(x-x_0) - \partial_n E(x-x_0) w_D(x)\Big)\ d\sigma(x) = w_D(x_0) - \int_{B_R} E(x-x_0)\big(-\alpha\Delta w_D(x)+w_D(x)\big)\ dx. \]

% On multiplie par $\frac{v_D(x_0)}{E(1)}$, et on utilise que $v_\omega(x) = v_D(x_0) \frac{E(x-x_0)}{E(1)}$,

% \[ \int_{\partial B_R} \Big(\partial_n w_D(x) v_\omega(x) - \partial_n v_\omega(x) w_D(x)\Big)\ d\sigma(x) = \frac{1}{\alpha E(1)}\,v_D(x_0)\,w_D(x_0) - \int_{B_R} v_\omega(x)\big(-\Delta w_D(x)+\alpha^{-1} w_D(x)\big)\ dx. \]

% En combinant les deux

% \[ \delta a - \delta l = \frac{1}{\alpha E(1)}\,v_D(x_0)\,w_D(x_0) - \int_{B_R} v_\omega(x)\big(-\Delta w_D(x)+\alpha^{-1} w_D(x)\big)\ dx - \int_{B_R}\Delta w_D v_\omega|_{\partial B_R}(x)\ dx \]
% \[ = \frac{1}{\alpha E(1)}\,v_D(x_0)\,w_D(x_0) + \int_{B_R} v_\omega(x)\Delta w_D(x)\ dx - \alpha^{-1}\int_{B_R} v_\omega(x)\,w_D(x)\ dx - \int_{B_R}\Delta w_D v_\omega|_{\partial B_R}(x)\ dx \]
% \[ = \frac{1}{\alpha E(1)}\,v_D(x_0)\,w_D(x_0) + \int_{B_R} \Delta w_D(x)\Big(v_\omega(x)-v_\omega|_{\partial B_R}(x)\Big)\ dx - \alpha^{-1}\int_{B_R} v_\omega(x)\,w_D(x)\ dx \]
% \[ = \frac{1}{\alpha E(1)}\,v_D(x_0)\,w_D(x_0) + \int_{B_R} \Big(\Delta w_D(x)-\alpha^{-1} w_D(x)\Big)\Big(v_\omega(x)-v_\omega|_{\partial B_R}(x)\Big)\ dx - \alpha^{-1}\int_{B_R} v_\omega|_{\partial B_R}(x)\,w_D(x)\ dx \]
% \[ = \frac{1}{\alpha E(1)}\,v_D(x_0)\,w_D(x_0) - \delta J - \alpha^{-1}\int_{B_R} v_\omega|_{\partial B_R}(x)\,w_D(x)\ dx \]

\color{black}

\end{comment}

==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/section04.tex <==
\section{Computation of the topological derivative}
\label{sec:summary-numerical}

We now gather the previous section results to derive the topological derivative. We consider the adjoint problem of Problem \ref{pb:problem:v-D}: \\
\begin{problem} Find $\widetilde{w}_0$ in $H^1(D)$ such that
	\begin{equation}
		\left \{ \begin{array}{cl}
            -\alpha\Delta \widetilde{w}_0 + \widetilde{w}_0 = -\widetilde{v}_0|\widetilde{v}_0|^{p-2}, & \text{in}\ D, \\
            \partial_n \widetilde{w}_0 = 0, & \text{on}\ \partial D. \\
        \end{array} \right .\label{eq:problem:w-D}
	\end{equation}
	\label{pb:problem:w-D}
\end{problem}
\color{black}

Then, we have the following proposition, \\

\begin{proposition}
    $w_0$, solution of Problem \ref{pb:problem:w-epsilon-outside}, is the restriction of $\widetilde{w}_0$ to $D\setminus B_R$.
    \label{prop:w0-wD}
\end{proposition}
\begin{proof}
    We set $w_R := \widetilde{w}_0|_{D\setminus B_R}$. We have to show that $w_R=w_0$ i.e. $a_0(w_R,\varphi_R) = -DJ_0(v_0)\varphi_R$, $\forall \varphi_R\in V_R$. Let $\varphi_R\in V_R$. We denote $\widetilde{\varphi}\in V_0$ the extension of $\varphi_R$ to $V_0$ such that $-\alpha\Delta\widetilde{\varphi} + \widetilde{\varphi} = 0$ in $B_R$. Thus,
    % Soit $\varphi\in H^1_0(D)$ telle que $-\alpha\Delta\varphi + \varphi = 0$ sur $B_R$. On pose $\varphi_R := \varphi|_{D\setminus B_R}$.
    \begin{align*}
        a_0(w_R,\varphi_R) & = \alpha\int_{D\setminus B_R}\nabla w_R\cdot\nabla\varphi_R\ dx + \alpha\int_{\partial B_R} T_0 w_R\, \varphi_R\ d\sigma + \int_{D\setminus B_R} w_R\,\varphi_R\ dx \\
        %
        & = \alpha\int_{D\setminus B_R}\nabla w_R\cdot\nabla\varphi_R\ dx + \alpha\int_{\partial B_R} T_0 w_R\, \varphi_R\ d\sigma + \int_{D\setminus B_R} w_R\,\varphi_R\ dx + \int_{B_R}\underbrace{(-\alpha\Delta\widetilde{\varphi} + \widetilde{\varphi})}_{=0} \widetilde{w}_0\ dx. \\
        %
        % & = \alpha\int_{D\setminus B_R}\nabla w_R\cdot\nabla\varphi_R\ dx + \alpha\int_{\partial B_R} T_0 w_R\, \varphi_R\ d\sigma + \int_{D\setminus B_R} w_R\,\varphi_R\ dx -\alpha \int_{B_R}\Delta\widetilde{\varphi} \widetilde{w}_0\ dx \\ & \hspace{3cm} + \int_{B_R}\widetilde{\varphi}\,\widetilde{w}_0\ dx \\
        %
        % & = \alpha\int_{D\setminus B_R}\nabla w_R\cdot\nabla\varphi_R\ dx + \alpha\int_{\partial B_R} T_0 \varphi_R\,w_R\ d\sigma + \int_{D\setminus B_R} w_R\,\varphi\ dx + \alpha\int_{B_R}\nabla\widetilde{\varphi}\cdot\nabla \widetilde{w}_0\ dx \\ & \hspace{3cm} - \alpha\int_{\partial B_R}\partial_n \widetilde{\varphi}\, \widetilde{w}_0\ d\sigma + \int_{B_R}\widetilde{\varphi}\,\widetilde{w}_0\ dx \\
        %
        % & = \alpha\int_{D\setminus B_R}\nabla w_R\cdot\nabla\varphi_R\ dx + \alpha\int_{\partial B_R} T_0 \varphi_R\,w_R\ d\sigma + \int_{D\setminus B_R} w_R\varphi_R\ dx + \alpha\int_{B_R}\nabla\widetilde{\varphi}\cdot\nabla \widetilde{w}_0\ dx \\ & \hspace{3cm} - \alpha\int_{\partial B_R}T_0 \varphi_R\, w_R\ d\sigma + \int_{B_R}\widetilde{\varphi}\,\widetilde{w}_0\ dx \\
        %
    \end{align*}
    And after integrating by parts,
    \begin{align*}
        a_0(w_R,\varphi_R) & = \alpha\int_{D\setminus B_R}\nabla w_R\cdot\nabla\varphi_R\ dx + \int_{D\setminus B_R} w_R\varphi_R\ dx + \alpha\int_{B_R}\nabla\widetilde{\varphi}\cdot\nabla \widetilde{w}_0\ dx + \int_{B_R}\widetilde{\varphi}\,\widetilde{w}_0\ dx \\
        %
        & = \alpha\int_{D}\nabla \widetilde{w}_0\cdot\nabla\widetilde{\varphi}\ dx + \int_{D}\widetilde{w}_0\,\widetilde{\varphi}\ dx \\
        %
        & = \widetilde{a}_0(\widetilde{w}_0,\widetilde{\varphi}) = -D\widetilde{J}_0(v_D)\widetilde{\varphi}.
    \end{align*}
    Moreover, by definition $\widetilde{J}_0(v_D) = J_0(v_R)$, % pour tout $v\in V_0$ telle que $-\alpha\Delta v + v = \alpha\Delta f$ dans $B_R$ (on pose $v_R := v|_{D\setminus B_R}$). Et
    thus, 
    \[ D\widetilde{J}_0(v_D)\widetilde{\varphi} = DJ_0(v_0)\varphi_R. \]
    % d'où,
    % Enfin, soit $\varphi_R\in V_R$. On note $\varphi\in V_0$ l'extension de $\varphi_R$ à $V_0$ telle que $-\alpha\Delta\varphi + \varphi = 0$ dans $B_R$. Alors,
    % \[ a_0(\varphi_R, w_R) = -DJ_0(v_0)\varphi_R. \]
    By uniqueness of the solution, $w_R = w_0$.
\end{proof}

Using that, if $u$ and $v$ are solutions of the linear diffusion equation on $B_R$, $$ v(x_0) = \frac{v^\text{mean}}{I_0(\alpha^{-1/2} R)} \qquad \text{and} \qquad w(x_0) = \frac{w^\text{mean}}{I_0(\alpha^{-1/2} R)}, $$
it follows the topological gradient based on the adjoint method given by: \\

\begin{proposition} \label{prop:topo-grad} For $\varepsilon$ small enough, we have,
    \[ j(K_\varepsilon) - j(K) = 2\alpha\,\widetilde{v}_0(x_0)\,\widetilde{w}_0(x_0)\frac{-2\pi}{\ln{\varepsilon}} + o\left(\frac{-1}{\ln{\varepsilon}}\right), \]
    with $\widetilde{v}_0$ solution of Problem \ref{pb:problem:v-D} and $\widetilde{w}_0$ solution of Problem \ref{pb:problem:w-D}.
\end{proposition}

% \begin{proof}
%     Unlike in previous proofs, we have that $\widetilde{v}_0$ and $\widetilde{w}_0$ are the solutions of Problem \ref{pb:problem:v-D} and Problem \ref{pb:problem:w-D} respectively and are the extensions of $v_0$, solution of Problem \ref{pb:problem:v-epsilon-outside}, and $w_0$, solution of Problem \ref{pb:problem:w-epsilon-outside}, respectively. Since the conditions for the adjoint method are fulfilled, we have,
%     \[ j(\varepsilon) = j(0) + \big(\delta a(v_0,w_0) - \delta l(w_0) + \delta J(v_0)\big)\,\varepsilon^{1/2} + o(\varepsilon^{1/2}). \]
%     Using that $v_\omega^{h, v_0} = v_\omega^{h, 0} + v_\omega^{0, v_0}$,
%     \begin{align*}
%         \delta j(x_0) & =  \delta a(v_0,w_0) - \delta l(w_0) + \delta J(v_0) \\
%         %
%         & = -\alpha\int_{\partial B_R} \partial_n v_\omega^{0, v_0}\, w_0\ d\sigma -\alpha\int_{\partial B_R} \partial_n v_\omega^{h, 0}\, w_0\ d\sigma - \int_{B_R} g_s(x,\widetilde{v}_0)\,v_\omega^{h, v_0}\ dx + \alpha\int_{\partial B_R} \partial_n w_0\,v_\omega^{h, v_0}|_{\partial B_R}\ dx \\
%         %
%         & = -\alpha\int_{\partial B_R} \partial_n v_\omega^{h, v_0}\, w_0\ d\sigma - \int_{B_R} g_s(x,\widetilde{v}_0)\,v_\omega^{h, v_0}\ dx + \alpha\int_{\partial B_R} \partial_n w_0\,v_\omega^{h, v_0}\ dx. \\
%     \end{align*}
%     With Proposition \ref{prop:gluing-solutions} and Proposition \ref{prop:w0-wD},
%     \begin{align*}
%         \delta j(x_0) & = -\alpha\int_{\partial B_R} \partial_n v_\omega^{h, v_0}\, \widetilde{w}_0\ d\sigma - \int_{B_R} g_s(x,\widetilde{v}_0)\, v_\omega^{h, v_0}\ dx + \alpha\int_{\partial B_R} \partial_n \widetilde{w}_0\,v_\omega^{h, v_0}\ dx.
%     \end{align*}
%     Since $-\alpha\Delta \widetilde{w}_0 + \widetilde{w}_0 = - g_s\big(\cdot,\widetilde{v}_0(\cdot)\big)$,
%     \begin{align*}
%         \delta j(x_0) & = -\alpha\int_{\partial B_R} \partial_n v_\omega^{h, v_0}\, \widetilde{w}_0\ d\sigma + \int_{B_R} (-\alpha\Delta \widetilde{w}_0 + \widetilde{w}_0) v_\omega^{h, v_0}\ dx + \alpha\int_{\partial B_R} \partial_n \widetilde{w}_0\,v_\omega^{h, v_0}\ dx \\
%         %
%         & = -\alpha\int_{\partial B_R} \partial_n v_\omega^{h, v_0}\, \widetilde{w}_0\ d\sigma - \alpha\int_{B_R} \Delta \widetilde{w}_0 v_\omega^{h, v_0}\ dx + \int_{B_R} \widetilde{w}_0v_\omega^{h, v_0}\ dx + \alpha\int_{\partial B_R} \partial_n \widetilde{w}_0\,v_\omega^{h, v_0}\ dx \\
%         %
%         & = -\alpha\int_{\partial B_R} \partial_n v_\omega^{h, v_0}\, \widetilde{w}_0\ d\sigma + \alpha\int_{B_R} \nabla \widetilde{w}_0 \cdot\nabla v_\omega^{h, v_0}\ dx - \alpha\int_{\partial B_R} \partial_n \widetilde{w}_0\,v_\omega^{h, v_0}\ d\sigma \\ & \hspace{2cm} + \int_{B_R} \widetilde{w}_0v_\omega^{h, v_0}\ dx + \alpha\int_{\partial B_R} \partial_n \widetilde{w}_0\,v_\omega^{h, v_0}\ dx \\
%         %
%         & = -\alpha\int_{\partial B_R} \partial_n v_\omega^{h, v_0}\, \widetilde{w}_0\ d\sigma + \alpha\int_{B_R} \nabla \widetilde{w}_0 \cdot\nabla v_\omega^{h, v_0}\ dx + \int_{B_R} \widetilde{w}_0v_\omega^{h, v_0}\ dx \\
%         %
%         & = -\alpha\int_{\partial B_R} \partial_n v_\omega^{h, v_0}\, \widetilde{w}_0\ d\sigma - \alpha\int_{B_R} \widetilde{w}_0 \Delta v_\omega^{h, v_0}\ dx + \alpha\int_{\partial B_R}\partial_n v_\omega^{h, v_0}\,\widetilde{w}_0\ d\sigma + \int_{B_R} \widetilde{w}_0v_\omega^{h, v_0}\ dx \\
%         %
%         & = - \alpha\int_{B_R} \widetilde{w}_0 \Delta v_\omega^{h, v_0}\ dx + \int_{B_R} \widetilde{w}_0v_\omega^{h, v_0}\ dx \\
%         %
%         & = \int_{B_R} (-\alpha\Delta v_\omega^{h, v_0} + v_\omega^{h, v_0})\, \widetilde{w}_0\ dx \\
%         %
%         & = \frac{1}{E(1)}v_0^{h, v_0}(x_0) \int_{B_R} \big(-\alpha\Delta E(x-x_0) + E(x-x_0)\big)\, \widetilde{w}_0\ dx \\
%         %
%         & = \frac{1}{E(1)}v_0^{h, v_0}(x_0) \int_{B_R} \delta_{x_0}\, \widetilde{w}_0\ dx \\
%         %
%         & = \frac{1}{E(1)}\,v_0^{h, v_0}(x_0)\,\widetilde{w}_0(x_0).
%     \end{align*}
%     Finally, using Proposition \ref{prop:w0-wD}, we have $v_0^{h, v_0}(x_0) = \widetilde{v}_0(x_0)$ and we get the result.
% \end{proof}

% \begin{proof}
%     Les hypothèses de la méthode de l'adjoint étant satisfaites, on a pour $v,w$ dans $V_R$
    
%     \[ j(\varepsilon) = j(0) + \big(\delta a(v,w) - \delta l(w) + \delta J(v)\big)\,\varepsilon + o(\varepsilon), \]
    
%     % ----------------------------------
    
%     avec 
    
%     \[ \delta a(v,w) = \alpha^{-1/2}\frac{v_0^{0,v}(x_0)}{K_0\left(\alpha^{-1/2}\right)} K_1\left(\alpha^{-1/2}R\right) \int_{\partial B_R} w\ d\sigma, \]
    
%     \[ \delta l(w) = -\alpha^{-1/2}\frac{v_0^{g,0}(x_0)}{K_0\left(\alpha^{-1/2}\right)} K_1\left(\alpha^{-1/2}R\right) \int_{\partial B_R} w\ d\sigma, \]
    
%     et
    
%     \[ \delta J(v) = 2\pi\frac{v_0^{g,\varphi}(x_0)}{K_0\left(\alpha^{-1/2}\right)} w(x_0). \]
    
%     D'où 
    
%     \begin{align*}
%         \delta a(v,w) - \delta l(w) + \delta J(v) & = \alpha^{-1/2}\frac{v_0^{g,v}(x_0)}{K_0\left(\alpha^{-1/2}\right)} K_1\left(\alpha^{-1/2}R\right) \int_{\partial B_R} w\ d\sigma + 2\pi\frac{v_0^{g,\varphi}(x_0)}{K_0\left(\alpha^{-1/2}\right)} w(x_0) \\
%         %
%         & = \frac{v_0^{g,v}(x_0)}{K_0\left(\alpha^{-1/2}\right)} \left(\alpha^{-1/2} K_1\left(\alpha^{-1/2}R\right) \int_{\partial B_R} w\ d\sigma + 2\pi w(x_0) \right).
%     \end{align*}
    
%     En faisant un développement de Taylor autour de $x_0$,
    
%     \begin{align*}
%         \delta a(v,w) - \delta l(w) + \delta J(v) & = \frac{v_0^{g,v}(x_0)}{K_0\left(\alpha^{-1/2}\right)} \left(\alpha^{-1/2} K_1\left(\alpha^{-1/2}R\right) 2\pi R w(x_0) + o(\varepsilon) + 2\pi w(x_0) \right) \\
%         %
%         & = \frac{v_0^{g,v}(x_0)w(x_0)}{K_0\left(\alpha^{-1/2}\right)} \left(\alpha^{-1/2} K_1\left(\alpha^{-1/2}R\right) 2\pi R + 2\pi \right) + o(\varepsilon).
%     \end{align*}

%     Pour conclure,
    
%     \begin{align*}
%         j(\varepsilon) - j(0) & = 2\pi\frac{v_0^{g,v}(x_0)w(x_0)}{K_0\left(\alpha^{-1/2}\right)} \left(\alpha^{-1/2} K_1\left(\alpha^{-1/2}R\right) R + 1 \right)\varepsilon + o(\varepsilon) \\
%         %
%         & = 2\pi\frac{\alpha^{-1/2} K_1\left(\alpha^{-1/2}R\right) R + 1}{K_0\left(\alpha^{-1/2}\right)}\,v_D(x_0)w_D(x_0)\,\varepsilon + o(\varepsilon).
%     \end{align*}
    
%     % ----------------------------------
    
%     % De plus, puisque pour $g\in L^?(D)$ et pour $\varphi\in H^{1/2}(B_?)$, $v_\omega^{g,\varphi} = v_\omega^{g,0} + v_\omega^{0,\varphi}$, on a 
    
%     % \begin{align*}
%     %     \delta a(v,w) - \delta l(w) & = \int_{\partial B_R} \big(\delta T v - \delta g\big)\, w\ d\sigma \\
%     %     %
%     %     & = -\int_{\partial B_R} \nabla\big( v_\omega^{0,\varphi} + v_\omega^{g,0} \big)\cdot n\, w\ d\sigma \\
%     %     %
%     %     & = \underbrace{-\int_{\partial B_R} \nabla v_\omega^{g,\varphi}\cdot n\, w\ d\sigma}_{\text{Green}} \\
%     %     %
%     %     & = \underbrace{-\int_{B_R} \nabla v_\omega^{g,\varphi}\cdot\nabla w\ dx}_{\text{Green}} - \int_{B_R} \Delta v_\omega^{g,\varphi} w\ dx \\
%     %     %
%     %     & = \int_{B_R} \Delta w\, v_\omega^{g,\varphi}\ dx - \int_{\partial B_R} \nabla w\cdot n\, v_\omega^{g,\varphi}\ d\sigma \underbrace{- \int_{B_R} \Delta v_\omega^{g,\varphi} w\ dx}_{\text{Green}} \\
%     %     %
%     %     & = \int_{B_R} \Delta w\, v_\omega^{g,\varphi}\ dx - \int_{\partial B_R} \nabla w\cdot n\, v_\omega^{g,\varphi}\ d\sigma - \int_{B_R} \nabla v_\omega^{g,\varphi}\cdot\nabla w\ dx  + \int_{\partial B_R} \nabla v_\omega^{g,\varphi}\cdot n\, w\ d\sigma \\
%     %     %
%     %     & = \int_{\partial B_R} \Big(\nabla v_\omega^{g,\varphi}\cdot n\, w - \nabla w\cdot n\, v_\omega^{g,\varphi}\Big)\ d\sigma + \int_{B_R} \Delta w\, v_\omega^{g,\varphi}\ dx - \int_{B_R} \nabla v_\omega^{g,\varphi}\cdot\nabla w\ dx.
%     % \end{align*}
    
%     % De plus, avec la théorie du potentiel, 
    
%     % \begin{align*}
%     %     w_D(x_0) & = -\int_{B_R} E(x-x_0)\,v_0(x)|v_0(x)|^{p-2}\ dx \\
%     %     %
%     %     & = -\int_{B_R} E(x-x_0)(-\alpha\Delta w_D(x) + w_D(x))\ dx \\
%     %     %
%     %     & = \alpha\int_{B_R} E(x-x_0)\Delta w_D(x)\ dx - \int_{B_R} E(x-x_0) w_D(x)\ dx
%     % \end{align*}
    
%     % % \begin{align*}
%     % %     w_D(x_0) & = -\int_{B_R} E(x-x_0)\,v_0(x)|v_0(x)|^{p-2}\ dx \\
%     % %     %
%     % %     & = -DJ_0(v_0)E(\cdot-x_0) \\
%     % %     %
%     % %     & = a_0(w_D,E(\cdot-x_0)) \\
%     % %     %
%     % %     & = \alpha\int_{D\setminus B_R}\nabla w_D\cdot\nabla E(x-x_0)\ dx + \int_{\partial B_R} T_0 w_D\,E(x-x_0)\ d\sigma + \int_{D\setminus B_R}w_D E(x-x_0)\ dx \\
%     % %     %
%     % %     & = \alpha\int_D\nabla w_D\cdot\nabla E(x-x_0)\ dx - \alpha\int_{B_R}\nabla w_D\cdot\nabla E(x-x_0)\ dx + \int_{\partial B_R} T_0 w_D\,E(x-x_0)\ d\sigma \\ 
%     % %     & \hspace{2cm} + \int_D w_D E(x-x_0)\ dx - \int_{B_R}w_D E(x-x_0)\ dx \\
%     % %     %
%     % %     & = \underbrace{\alpha\int_D\nabla w_D\cdot\nabla E(x-x_0)\ dx + \int_D w_D E(x-x_0)\ dx}_{=-D\tilde{J_0}(\tilde{v_D})E(\cdot-x_0)} + \int_{\partial B_R} T_0 w_D\,E(x-x_0)\ d\sigma \\ 
%     % %     & \hspace{2cm} - \alpha\int_{B_R}\nabla w_D\cdot\nabla E(x-x_0)\ dx - \int_{B_R}w_D E(x-x_0)\ dx \\
%     % %     %
%     % %     & = -D\tilde{J_0}(\tilde{v_D})E(\cdot-x_0) + \int_{\partial B_R} T_0 w_D\,E(x-x_0)\ d\sigma - \alpha\int_{B_R}\nabla w_D\cdot\nabla E(x-x_0)\ dx - \int_{B_R}w_D E(x-x_0)\ dx
%     % % \end{align*}

%     % D'où
    
%     % \begin{align*}
%     %     \delta a(v_D,w_D) - \delta l(w_D) & = \int_{\partial B_R} \Big(\nabla v_\omega^{g,\varphi}\cdot n\, w_D - \nabla w_D\cdot n\, v_\omega^{g,\varphi}\Big) \ d\sigma + \int_{B_R} \Delta w_D\, v_\omega^{g,\varphi}\ dx - \int_{B_R} \nabla v_\omega^{g,\varphi}\cdot\nabla w_D\ dx.
%     % \end{align*}
    
%     % et
    
%     % \begin{align*}
%     %     \delta J(v) & = \int_{B_R} |\tilde{v_0}|^{p-2} \tilde{v_0}\, v_\omega^{g,\varphi}\ dx
%     % \end{align*}
    
%     % ---------------------------
    
%     % \[ V(y) := \sqrt{\frac{1}{8\pi\sqrt{\alpha}}}|y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\int_{\partial B_1} p(x)\ d\sigma(x) \]
    
%     % Si on utilise les estimations avec $V$ plutôt que $v_\omega$, on a 
    
%     % \begin{align*}
%     %     \delta a(v_0,w_0) - \delta l(w_0) & = -\int_{\partial B_R} \nabla V^{g,\varphi}\cdot n\, w\ d\sigma \\
%     %     %
%     %     & = -\sqrt{\frac{1}{8\pi\sqrt{\alpha}}}\left(\int_{\partial B_R} \nabla |y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\cdot n\, w_0\ d\sigma\right)\, \underbrace{\int_{\partial B_1} p(x)\ d\sigma(x)}_{:=A(v_0(x_0))} \\
%     %     %
%     %     & = -\sqrt{\frac{1}{8\pi\sqrt{\alpha}}} A(v_0(x_0)) \int_{\partial B_R} \nabla |y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\cdot n\, w_0\ d\sigma \\
%     %     %
%     %     & = \sqrt{\frac{1}{8\pi\sqrt{\alpha}}} A(v_0(x_0))\left(\frac{R^{-3/2}}{2} + \frac{R^{1/2}}{\sqrt{\alpha}}\right)e^{-R/\sqrt{\alpha}} \int_{\partial B_R} w_0\ d\sigma.
%     % \end{align*}
% \end{proof}

We notice that with this expansion, we get the main theoretical result of the paper which might be summarized as follows: to minimize the $L^p$-error between an image and its reconstruction from linear diffusion inpainting, we have to keep in the mask the pixels $x_0$ which minimize the product $\widetilde{v}_0(x_0)\,\widetilde{w}_0(x_0)$. 
%The previous computations, does not used  directly the $L^p$-error,  since it this one does not satisfy the right hypotheses (for $p=1$). 


% Il en découle l'algorithme suivant, \\

% \begin{algorithm}[H]
% 	\KwData{$f$, $\alpha$, $c$}
%  	\KwResult{$K$}
%  	\vspace{0.2cm}
    
%     $K\leftarrow \emptyset$\;
    
%     \While{La densité de pixel dans $K$ est inférieure à $c$}{
%         calculer $v_0$\;
%         calculer $w_0$\;
%         $K\leftarrow K\cup\big\{x_0\ \big|\ \min\ v_0(x_0)\,w_0(x_0)\big\}$\;
%     }
%     \vspace{0.2cm}
% 	\caption{Méthode de l'adjoint pour la compression.}
% \end{algorithm} \vspace{0.4cm}

% ---------------------------------------------- \\

% et pour $v,w$ dans $V_R$,

% \[ \delta a(v,w) - \delta l(w) = \alpha^{-1/2}\frac{v_0^{g,v}(x_0)}{K_0\left(\alpha^{-1/2}\right)} K_1\left(\alpha^{-1/2}R\right) \int_{\partial B_R} w\ d\sigma. \]

% Taylor autour de $x_0$,

% \[ \delta a(v,w) - \delta l(w) = 2\pi\,R\,\alpha^{-1/2}\frac{K_1\left(\alpha^{-1/2}R\right)}{K_0\left(\alpha^{-1/2}\right)}  v_0^{g,v}(x_0)\,w(x_0) + O(\varepsilon). \]

==> Adjoint-Method-in-PDE-based-Image-Compression-main/tex_parts/section05.tex <==
\section{Numerical Results}
\label{sec:numerical-results}

In this section, we present numerical results when the cost functional is the $L^1$-error and the $L^2$-error, respectively, as they are the most representative for noise in practice. In fact, we take these specific values of $p$, depending on the nature of the noise considered: $p=2$ is well suited for Gaussian noise while $p=1$ is better for impulse noise such as salt and pepper noise.

Let us denote by $f$ the original image, $f_\delta$ the noisy one, $K$ the inpainting mask, and $u$ the reconstructed image. Proposition \ref{prop:topo-grad} gives a hard-threshold criterion for the selection of $K$, namely, we must keep the pixels $x\in D$ which minimize the quantity $\widetilde{v}_0(x)\,\widetilde{w}_0(x)$ (or equivalently, which maximize $-\widetilde{v}_0(x)\,\widetilde{w}_0(x)$). In fact, the adjoint state is obtained by solving a linear PDE which is, by the elliptic regularity, $H^2$ (the right-hand side is $L^2$ even when $p=1$ with the regularization adopted in the article).
The distribution of this function measures the influence of a considered single pixel and its neighborhood in the cost variations. This is referred to as soft-thresholding (in contrast to hard-thresholding with pixel-wise asymptotics) and is implemented using the \textit{Floyd-Steinberg} halftoning technique \cite{Ulichney1987}. Digital halftoning is a technique used to simulate continuous-tone images using a limited palette of colors or shades, often just black and white. The compression step states as follows:
\begin{enumerate}
	\item solve Problem \ref{pb:problem:v-D} with $h=\alpha\Delta f_\delta$, and save the result in $\widetilde{v_0}$,
	\item solve Problem \ref{pb:problem:w-D} and save the result in $\widetilde{w_0}$,
	\item apply hard/soft-thresholding to $-\widetilde{v_0} \widetilde{w_0}$ and store the selected pixels in $K$.
\end{enumerate}
We emphasize that the inpainting mask is built from $f_\delta$, which is available in $D$ during the mask selection step, while it is only available in $K$ for the reconstruction.

The reconstruction step is performed by solving the heat equation with the semi-implicit discrete scheme of time step $dt>0$ and with initial condition $u_0$. In fact, Problem \ref{pb:problem_1} is formally the first iteration of the semi-implicit discrete scheme of the heat equation, and directly solving Problem \ref{pb:problem_1} will result to a small diffusion of the data, leading to a poor reconstruction's quality. We choose the time step $dt=10$ and the initial condition $u_0=\mathbf{1}_K f_\delta$ for boundary conditions compatibility. The diffusion process is stopped as soon as the error $e_n$ between the reconstruction $u_n$ and the noisy data $f_\delta$ at the iteration $n\in\N^*$ starts to increase i.e. when $e_{n} \geq e_{n-1}$ where $e_n := \|u_n - f_\delta\|_{L^p(D)}$.

We denote by \textit{Lp-ADJ-T} the algorithm using the adjoint method by selecting the pixels using hard-thresholding, and by \textit{Lp-ADJ-H} the algorithm combining with the \textit{Floyd-Steinberg} halftoning. For comparison purposes, we consider the methods \textit{H1-T} and \textit{H1-H}, which correspond to mask selection based on the asymptotic expansion provided in \cite{Belhachmi2009}. In these methods, the authors use a hard/soft-thresholding of $|\Delta f_\delta|$ as pixel selection criterion, combined with homogeneous diffusion inpainting for the reconstruction. Note that the homogeneous diffusion equation can be viewed as a limiting case of the heat equation as $t$ approaches infinity.
In their paper, Belhachmi \textit{et al} stated that they smoothed the data prior to computing its Laplacian. However, since we aim to demonstrate the effectiveness of our methods on noisy data, we believe that pre-processing the data introduces an unfair advantage. For this reason, we do not smooth $f_\delta$ when calculating its Laplacian, although we do apply smoothing for the \textit{H1-} methods as described by the authors.

To solve the equations, we discretize the problems using the finite difference method where every degree of freedom correspond to a pixel of the image, and we manually select the parameter $\alpha$ to achieve the best reconstruction. The implementation of the algorithms is done in Python and can be found in \cite{Jacumin2024}.

\subsection{Impulse Noise}

We begin the experiments by evaluating the robustness of our methods against impulse noise. Impulse noise, such as salt-and-pepper noise, is often addressed by minimizing the $L^1$-error, as discussed in \cite{Nikolova2002, Nikolova2004}. Here, we focus on the case $p=1$, and our proposed methods are refereed by \textit{L1-ADJ-}. Figure \ref{fig:input-impulse-noise} shows the input images in the following order, from left to right: the noiseless image, the image with salt noise, the one with pepper noise, and the image with a combination of both salt and pepper noise.

\begin{figure}[H]
	\centering
	\subfloat[Without noise.]{
		\includegraphics[width=3.6cm]{images/Trui.png}
	}
	\quad
	\subfloat[With $2\%$ of salt noise.]{
		\includegraphics[width=3.6cm]{images/sp/Trui-sp-0.02-0.png}
	}
	\quad
	\subfloat[With $2\%$ of pepper noise.]{
		\includegraphics[width=3.6cm]{images/sp/Trui-sp-0-0.02.png}
	}
	\quad
	\subfloat[With $2\%$ of salt and pepper noise.]{
		\includegraphics[width=3.6cm]{images/sp/Trui-sp-0.01-0.01.png}
	}
	\caption{Input images.}
	\label{fig:input-impulse-noise}
\end{figure}

We give in Table \ref{tab:methods-comparison:l1:0.1} (and in Appendix \ref{app:sp}) the $L^1$-error for the \textit{H1-} and \textit{L1-ADJ-} methods for several amounts of salt and/or pepper noise, and hand-picked regularization parameter $\alpha$ ($\|\cdot\|_1$ denotes the $L^1$ norm). The first notable observation is that \textit{L1-ADJ-H} gives the lowest $L^1$-error with and without presence of noise. Additionally, consistent with findings from \cite{Belhachmi2009,Belhachmi2022Jun}, the soft-thresholding rule consistently results in a more effective inpainting mask for image reconstruction.

\begin{table}[H]
	\centering
	\begin{tabular}{|c|c||c|c||c|c||c||c|}
		\hline
		\multicolumn{2}{|c||}{\textbf{Noise}} & \multicolumn{2}{c||}{\textbf{L1-ADJ-T}} & \multicolumn{2}{c||}{\textbf{L1-ADJ-H}} & \textbf{H1-T} & \textbf{H1-H} \\
		\hline
		Salt & Pepper & $\alpha$ & $\|f-u\|_1$ & $\alpha$ & $\|f-u\|_1$ & $\|f-u\|_1$ & $\|f-u\|_1$ \\
		\hhline{|========|}
		0 & 0 & 0.01 & 4248.14 & 2.27 & \textbf{904.21} & 4648.99 & 961.01 \\
		0.02 & 0 & 0.41 & 3203.43 & 0.66 & \textbf{1194.91} & 6531.56 & 3875.63 \\
		0 & 0.02 & 0.36 & 2505.63 & 0.71 & \textbf{1204.80} & 5461.22 & 4019.73 \\
		0.01 & 0.01 & 0.56 & 2252.71 & 0.76 & \textbf{1321.55} & 4573.62 & 3097.18 \\
		0.04 & 0 & 0.36 & 4132.62 & 0.56 & \textbf{1453.11} & 12381.64 & 9611.86 \\
		0 & 0.04 & 2.07 & 2938.43 & 0.56 & \textbf{1454.21} & 15171.93 & 11195.98 \\
		0.02 & 0.02 & 0.46 & 2912.86 & 0.61 & \textbf{2098.27} & 6654.28 & 5901.86 \\
		0.1 & 0 & 0.26 & 8414.41 & 0.51 & \textbf{1845.45} & 28163.84 & 22580.17 \\
		0 & 0.1 & 2.42 & 4320.62 & 0.51 & \textbf{1840.34} & 34035.09 & 27595.06 \\
		0.05 & 0.05 & 0.36 & 6191.32 & 0.51 & \textbf{4623.07} & 17716.39 & 15806.10 \\
		\hline
	\end{tabular} \vspace{0.2cm}
	
	\caption{$L^1$-error between the original image $f$ and the reconstruction $u$ (built from  $f_\delta$)  with $10\%$ of total pixels saved.}
	\label{tab:methods-comparison:l1:0.1}
\end{table}

Figure \ref{fig:sp:0.01-0.01:l1:0.1} (and Appendix \ref{app:sp}) shows the resulting masks and reconstructions corresponding to the data in the tables. We note that most of the corrupted pixels are not selected in $K$ for the \textit{L1-ADJ-} methods, while they are in the case of \textit{H1-} ones. It is explained as follows: the asymptotic provided for the \textit{H1-} methods leads to a pixel selection criterion which is proportional to $|\Delta f_\delta|^2$. In the presence of impulse noise, the Laplacian is high at the edges, with even greater intensities at noisy pixels. Thus, noisy pixels are selected as a priority on pixels close to edges. On the other hand, the \textit{L1-ADJ-} methods keep pixel in the inpainting mask that are located near the edges and around noisy pixels. In fact, for well-chosen $\alpha$, if the Laplacian is too large at an isolated pixel, we are in presence of the noise and if it is too small, we are in homogeneous parts, and in both case, the \textit{L1-ADJ-} methods do not select the pixel.

\begin{figure}[H]
	\centering
	\subfloat[Mask L1-ADJ-T.]{
		\includegraphics[width=3.6cm]{images/sp/mask-L1-T-sp-0.01-0.01.png}
	}
	\quad
	\subfloat[Reconstruction with L1-ADJ-T.]{
		\includegraphics[width=3.6cm]{images/sp/decoded-L1-T-sp-0.01-0.01.png}
	}
	\quad
	\subfloat[Mask L1-ADJ-H.]{
		\includegraphics[width=3.6cm]{images/sp/mask-L1-H-sp-0.01-0.01.png}
	}
	\quad
	\subfloat[Reconstruction with L1-ADJ-H.]{
		\includegraphics[width=3.6cm]{images/sp/decoded-L1-H-sp-0.01-0.01.png}
	}
	\quad
	\subfloat[Mask H1-T.]{
		\includegraphics[width=3.6cm]{images/sp/mask-H1-T-sp-0.01-0.01.png}
	}
	\quad
	\subfloat[Reconstruction with H1-T.]{
		\includegraphics[width=3.6cm]{images/sp/decoded-H1-T-sp-0.01-0.01.png}
	}
	\quad
	\subfloat[Mask H1-H.]{
		\includegraphics[width=3.6cm]{images/sp/mask-H1-H-sp-0.01-0.01.png}
	}
	\quad
	\subfloat[Reconstruction with H1-H.]{
		\includegraphics[width=3.6cm]{images/sp/decoded-H1-H-sp-0.01-0.01.png}
	}
	\caption{Masks and reconstructions from image with $2\%$ of salt and pepper noise and with $10\%$ of total pixels saved.}
	\label{fig:sp:0.01-0.01:l1:0.1}
\end{figure}

To provide further clarification on this last statement, we present the following case study: a binary image with two corrupted pixels (see Figure \ref{fig:alpha-influence} (a)). On Figure \ref{fig:alpha-influence} (a), (b), we plot the value of the criterion evaluated at several positions (noise, edge and homogeneous) with respect to the value of the regularization parameter $\alpha$. Formally, the criterion reads, for a well-chosen $\gamma>0$, depending on $\alpha$,
$$ \alpha \big(K_\gamma \star \Delta f_\delta\big)\big(K_\gamma\star\text{sign}(\Delta f_\delta)\big), $$
where $\star$ denote the convolution product and $K_\gamma$ is the heat kernel, fundamental solution of the linear diffusion equation. When $\alpha$ is small, the criterion is close to $\alpha\,\text{sign}(\Delta f_\delta) \Delta f_\delta = \alpha |\Delta f_\delta|$ which behaves similarly to the \textit{H1-} method, and, in particular, the noisy pixel is kept. For large $\alpha$, the criterion in the homogeneous part is dominant, and the edges of the image are lost. There is a window for the value of $\alpha$ in which the edge pixels are sectioned. We give in Figure \ref{fig:sp:under-over-regularization} illustrations for under/over-regularization.

\begin{figure}[H]
	\centering
	\subfloat[Study case.]{
		\includegraphics[height=3.1cm]{images/sp/crit-value-test.png}
	}
	\subfloat[Zoom on small $\alpha$.]{
		\includegraphics[height=3.9cm]{images/sp/alpha-influence-zoom.png}
	}
	\qquad
	\subfloat[Behavior for large $\alpha$.]{
		\includegraphics[height=3.9cm]{images/sp/alpha-influence.png}
	}
	
	\caption{Influence of $\alpha$ on the criterion evaluated at a noisy pixel, an edge pixel and a pixel in the homogeneous part.}
	\label{fig:alpha-influence}
\end{figure}


\begin{figure}[H]
	\centering
	\subfloat[Mask $\alpha=0.01$.]{
		\includegraphics[width=3.6cm]{images/sp/mask-l1-under-regularized.png}
	}
	\quad
	\subfloat[Reconstruction.]{
		\includegraphics[width=3.6cm]{images/sp/u-l1-under-regularized.png}
	}
	\quad
	\subfloat[Mask $\alpha=100$.]{
		\includegraphics[width=3.6cm]{images/sp/mask-l1-over-regularized.png}
	}
	\quad
	\subfloat[Reconstruction.]{
		\includegraphics[width=3.6cm]{images/sp/u-l1-over-regularized.png}
	}
	\caption{Example of under-regularization on the left and of over-regularization on the right. For both case, \textit{L1-ADJ-H} is used on the salt and pepper corrupted input (Figure \ref{fig:input-impulse-noise} (d)).}
	\label{fig:sp:under-over-regularization}
\end{figure}

\subsection{Gaussian Noise}

Now, we consider images with Gaussian noise and we take $p=2$. Figure \ref{fig:input-wn} presents the input images without noise on the left, followed by the noisy images.

\begin{figure}[H]
	\centering
	\subfloat[Without noise.]{
		\includegraphics[width=3.6cm]{images/Trui.png}
	}
	\quad
	\subfloat[$\sigma=0.03$.]{
		\includegraphics[width=3.6cm]{images/wn/Trui-wn-0.03.png}
	}
	\quad
	\subfloat[$\sigma=0.05$.]{
		\includegraphics[width=3.6cm]{images/wn/Trui-wn-0.05.png}
	}
	\quad
	\subfloat[$\sigma=0.1$.]{
		\includegraphics[width=3.6cm]{images/wn/Trui-wn-0.1.png}
	}
	\caption{Input images $f_\delta$ with gaussian noise of deviation $\sigma$.}
	\label{fig:input-wn}
\end{figure}

Table \ref{tab:methods-comparison:l2:0.1} (and Appendix \ref{app:wn}) gives the $L^2$-error for the \textit{L2-ADJ-} methods and the \textit{H1-T} methods with respect to the deviation $\sigma>0$ of Gaussian noise and the value of $\alpha$ (we write $\|\cdot\|_2$ the $L^2$ norm). For a reasonable level of noise, the \textit{L2-ADJ-H} gives the lowest $L^2$-error. Moreover, and as for the \textit{L1-ADJ-} methods, using digital halftoning enhance the reconstruction by giving a better distribution of the pixel in the mask.

\begin{table}[H]
	\centering
	\begin{tabular}{|c||c|c||c|c||c||c|}
		\hline
		\textbf{Noise} & \multicolumn{2}{c||}{\textbf{L2-ADJ-T}} & \multicolumn{2}{c||}{\textbf{L2-ADJ-H}} & \textbf{H1-T} & \textbf{H1-H} \\
		\hline
		$\sigma$ & $\alpha$ & $\|f-u\|_2$ & $\alpha$ & $\|f-u\|_2$ & $\|f-u\|_2$ & $\|f-u\|_2$ \\
		\hhline{|=======|}
		0    & 0.01 & 23.08 & 0.01 & 9.70 & 25.57 & \textbf{4.99} \\
		0.03 & 0.71 &  9.38 & 0.96 & \textbf{7.91} & 9.23 & 8.57 \\
		0.05 & 0.86 & 13.25 & 0.76 & \textbf{12.39} & 13.78 & 12.55 \\
		0.1  & 0.71 & 26.95 & 0.66 & 24.47 & 27.15 & \textbf{22.95} \\
		0.2  & 0.01 & 56.08 & 2.27 & 46.46 & 61.94 & \textbf{42.62} \\
		\hline
	\end{tabular} \vspace{0.2cm}
	
	\caption{$L^2$-error between the original image $f$ and the reconstruction $u$ (built from $f_\delta$)  with $10\%$ of total pixels saved.}
	\label{tab:methods-comparison:l2:0.1}
\end{table}

In Figure \ref{fig:w:0.05:l2:0.1} (and in Appendix \ref{app:wn}), we present the resulting masks and reconstruction for various noise level. In the presence of Gaussian noise, the Laplacian amplifies the noise, and we cannot distinguish the edges from the noise if the noise level is sufficiently large. This explains why the \textit{H1-} methods result in poor reconstructions. Conversely, the edges of the image are clearly discernible in the \textit{L2-ADJ-} masks, and the reconstructed image appears to contain less noise compared to the input.

\begin{figure}[H]
	\centering
	\subfloat[Mask L2-ADJ-T.]{
		\includegraphics[width=3.6cm]{images/wn/mask-L2-T-wn-0.05.png}
	}
	\quad
	\subfloat[Reconstruction with L2-ADJ-T.]{
		\includegraphics[width=3.6cm]{images/wn/decoded-L2-T-wn-0.05.png}
	}
	\quad
	\subfloat[Mask L2-ADJ-H.]{
		\includegraphics[width=3.6cm]{images/wn/mask-L2-H-wn-0.05.png}
	}
	\quad
	\subfloat[Reconstruction with L2-ADJ-H.]{
		\includegraphics[width=3.6cm]{images/wn/decoded-L2-H-wn-0.05.png}
	}
	\quad
	\subfloat[Mask H1-T.]{
		\includegraphics[width=3.6cm]{images/wn/mask-H1-T-wn-0.05.png}
	}
	\quad
	\subfloat[Reconstruction with H1-T.]{
		\includegraphics[width=3.6cm]{images/wn/decoded-H1-T-wn-0.05.png}
	}
	\quad
	\subfloat[Mask H1-H.]{
		\includegraphics[width=3.6cm]{images/wn/mask-H1-H-wn-0.05.png}
	}
	\quad
	\subfloat[Reconstruction with H1-H.]{
		\includegraphics[width=3.6cm]{images/wn/decoded-H1-H-wn-0.05.png}
	}
	\caption{Masks and reconstructions from image with gaussian noise of deviation $\sigma=0.1$ and with $10\%$ of total pixels saved.}
	\label{fig:w:0.05:l2:0.1}
\end{figure}

For small $\alpha$, the criterion $-\widetilde{v}_0\,\widetilde{w}_0$ is formally close to $\alpha|\Delta f|^2$ which is similar to the result found in \cite{Belhachmi2022Jun}, but the fact that the adjoint state $\widetilde{w}_0$ and primal variable $\widetilde{v}_0$ are computed by solving linear PDEs improves distribution of the topological derivative. When $\alpha$ is large, we lose the information given by the edges, as showed in Figure \ref{fig:w:under-over-regularization}.

\begin{figure}[H]
	\centering
	\subfloat[Mask $\alpha=0.01$.]{
		\includegraphics[width=3.6cm]{images/wn/mask-l2-under-regularized.png}
	}
	\quad
	\subfloat[Reconstruction.]{
		\includegraphics[width=3.6cm]{images/wn/u-l2-under-regularized.png}
	}
	\quad
	\subfloat[Mask $\alpha=100$.]{
		\includegraphics[width=3.6cm]{images/wn/mask-l2-over-regularized.png}
	}
	\quad
	\subfloat[Reconstruction.]{
		\includegraphics[width=3.6cm]{images/wn/u-l2-over-regularized.png}
	}
	\caption{Example of under-regularization on the left and of over-regularization on the right. For both case, \textit{L2-ADJ-H} is used on the salt and pepper corrupted input (Figure \ref{fig:input-wn} (c)).}
	\label{fig:w:under-over-regularization}
\end{figure}

==> tex_parts/draft.tex <==
% \section{draft}

% \[ E(z) := \frac{1}{2\pi} K_0\left(\frac{z}{\sqrt{\alpha}}\right). \]

% Lorsque $z$ est grand,

% \[ K_n(z) = \sqrt{\frac{\pi}{2}}z^{-1/2}e^{-z} + O\big(z^{-3/2}e^{-z}\big). \]

% Taylor quand $|y|\to +\infty$,

% \[ E\big(|y-x|\big) = E\big(|y|\big) + o(1) = E\big(|y|\big) - \nabla_y E\big(|y|\big)\cdot x + o(1). \]

% et

% \[ \nabla_y E\big(|y|\big) = \frac{1}{2\pi} \nabla_y K_0\left(\frac{|y|}{\sqrt{\alpha}}\right) = -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y \]

% d'où 

% \[ E\big(|y-x|\big) = E(|y|) + \nabla E(|y|) \cdot x + o(\|x\|^2) \]
% \[ = \frac{1}{2\pi} K_0\left(\frac{|y|}{\sqrt{\alpha}}\right) + \frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y\cdot x + O\left(K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y\cdot x\right). \]

% \[ \tilde{V}(y) := E(|y|) =\frac{1}{2\pi} K_0\left(\frac{|y|}{\sqrt{\alpha}}\right) \]
% \[ \tilde{W}(y) := O\left( K_0\left(\frac{|y|}{\sqrt{\alpha}}\right) \right) \]
% \[ \nabla \tilde{V}(y) := -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y \]

% \[ \nabla E\big(|y-x|\big) = \nabla\tilde{V}(y) + \nabla \tilde{W}(y) \]
% \[ \Leftrightarrow -\frac{1}{2\pi} K_1\left(\frac{|y-x|}{\sqrt{\alpha}}\right) |y-x|^{-1} y = -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y + \nabla \tilde{W}(y) \]
% \[ \Leftrightarrow -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y + O\left(K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y\right) = -\frac{1}{2\pi} K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y + \nabla \tilde{W}(y) \]
% \[ \Leftrightarrow  \nabla \tilde{W}(y) = O\left(K_1\left(\frac{|y|}{\sqrt{\alpha}}\right) |y|^{-1} y\right) \]



% % \[ V(y) := \sqrt{\frac{\sqrt{\alpha}}{8\pi}}|y|^{-1/2}e^{-|y|/\sqrt{\alpha}} \int p\ d\sigma \]
% % \[ W(y) := O\big(|y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\big) \]
% % \[ \nabla V(y) := \sqrt{\frac{\sqrt{\alpha}}{8\pi}}|y|^{-3/2}e^{-|y|/\sqrt{\alpha}} y \int p\ d\sigma \]
% % \[ \nabla W(y) := O\big(|y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\big) y \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow V(y) := \sqrt{\frac{1}{8\pi\sqrt{\alpha}}}|y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\int_{\partial B_1} p(x)\ d\sigma(x) \]
% \[ \Longrightarrow W(y) := O\big(|y|^{-3/2}e^{-|y|/\sqrt{\alpha}}\big) \]

% ---------------------------------------------------------------------------------

% SageMath : 

% \[ -\frac{e^{\left(-\frac{u\left(z\right)}{\sqrt{\alpha}}\right)} \frac{\partial}{\partial z}u\left(z\right)}{\sqrt{\alpha} \sqrt{u\left(z\right)}} - \frac{e^{\left(-\frac{u\left(z\right)}{\sqrt{\alpha}}\right)} \frac{\partial}{\partial z}u\left(z\right)}{2 \, u\left(z\right)^{\frac{3}{2}}} \]

% et 

% \[ u(z) = |z|, \]
% \[ \partial_z u(z) = \nabla u(z) = |z|^{-1} z, \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow \nabla V(y) = - \sqrt{\frac{1}{8\pi\sqrt{\alpha}}} e^{\left(-\frac{|y|}{\sqrt{\alpha}}\right)} |y|^{-1} \left( \frac{1}{\sqrt{\alpha} \sqrt{|y|}} + \frac{1}{2 \, |y|^{\frac{3}{2}}} \right) y \int_{\partial B_1} p(x)\ d\sigma(x) \]

% ---------------------------------------------------------------------------------

% \[ \nabla_y v_\omega(y) = -\frac{1}{2\pi}\int_{\partial B_1} |y-x|^{-1} K_1(|y-x|)\, p(x)\ d\sigma(x)\ y \]
% \[ = -\sqrt{\frac{1}{8\pi\sqrt{\alpha}}}|y|^{-1}\int_{\partial B_1}  |y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\, p(x)\ d\sigma(x)\ y + O\big(|y|^{-5/2}e^{-|y|/\sqrt{\alpha}}\big)y \]
% \[ = -\sqrt{\frac{1}{8\pi\sqrt{\alpha}}}\int_{\partial B_1}  |y|^{-3/2}e^{-|y|/\sqrt{\alpha}}\, p(x)\ d\sigma(x)\ y + O\big(|y|^{-5/2}e^{-|y|/\sqrt{\alpha}}\big)y. \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow \nabla W(y) = O\big(|y|^{-7/2}e^{-|y|/\sqrt{\alpha}}\big)y \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow |V(y)| \leq C_1\, |y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\, \|\varphi\|, \]
% \[ \Longrightarrow |W(y)| \leq C_2\, |y|^{-3/2}e^{-|y|/\sqrt{\alpha}}\, \|\varphi\|, \]
% \[ \Longrightarrow |\nabla V(y)| \leq C_3\,|y|^{-1/2}\left( 1 + |y|^{-1} \right) e^{-|y|/\sqrt{\alpha}} \, \|\varphi\| \leq C_3\,|y|^{-1/2}e^{-|y|/\sqrt{\alpha}} \, \|\varphi\|, \]
% \[ \Longrightarrow |\nabla W(y)| \leq C_4\, |y|^{-5/2}e^{-|y|/\sqrt{\alpha}}\, \|\varphi\|. \]

% ---------------------------------------------------------------------------------

% \[ \Longrightarrow |V(y)| \leq C_1\, |y|^{-1/2}\, \|\varphi\|_{1/2,\partial B_1}, \]
% \[ \Longrightarrow |W(y)| \leq C_2\, |y|^{-3/2}\, \|\varphi\|_{1/2,\partial B_1}, \]
% \[ \Longrightarrow |\nabla V(y)| \leq C_3\,|y|^{-1/2} \, \|\varphi\|_{1/2,\partial B_1}, \]
% \[ \Longrightarrow |\nabla W(y)| \leq C_4\, |y|^{-5/2}\, \|\varphi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|V\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |V|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_3\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |W|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_4\, \, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|V\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_5\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |V|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_6\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_7\, \varepsilon^{1/2} \,\|\psi\|_{1/2,\partial B_1}, \]
% \[ |W|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_8\, \varepsilon^{3/2}\, \|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|V\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\,\|\psi\|_{1/2,\partial B_1}, \]
% \[ \|V\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_3\, \varepsilon^{-1/2} \,\|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_4\, \varepsilon^{1/2} \,\|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |v_\omega|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_3\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_4\,\varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |v_\omega|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_5\, \varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_6\,\varepsilon^{-1/2}\, \|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \begin{proposition} Soit $\psi\in H^{1/2}(\partial B_1)$.

%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta v_\varepsilon + v_\varepsilon = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         v_\varepsilon = \psi(\,\cdot\,/\varepsilon), & \text{sur}\ \partial B_\varepsilon, \\
%         v_\varepsilon = 0, & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\varepsilon\|_{0,B_R\setminus B_\varepsilon} \leq C_1\,\varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}, \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_\varepsilon} \leq C_2\,\varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}, \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C_3\,\varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}. \]
% \end{proposition}

% \begin{proposition}
%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta v_\varepsilon + v_\varepsilon = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         v_\varepsilon = \psi, & \text{sur}\ \partial B_\varepsilon, \\
%         v_\varepsilon = \varphi, & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\varepsilon\|_{0,B_R\setminus B_\varepsilon} \leq C_1\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}\big), \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_\varepsilon} \leq C_2\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}\big), \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C_3\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}\big). \]
% \end{proposition}

% ---------------------------------------------------------------------------------

% \[ \int_{\partial B_R} (T_\varepsilon-T_0) v_0\ d\sigma = \int_{\partial B_R} \partial_n (v_\varepsilon^{0,v_0} - v_0^{0,v_0})\ d\sigma \]

%     On pose pour $x\in \R^2\setminus B_\varepsilon$,
    
%     \[ w_\varepsilon^{0,v_0}(x) := v_\varepsilon^{0,v_0}(x) - v_0^{0,v_0}(x) + v_\omega(x/\varepsilon). \]
    
%     Ainsi, 
    
%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta w_\varepsilon^{0,v_0} + w_\varepsilon^{0,v_0} = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         w_\varepsilon^{0,v_0} = v_0(x_0) - v_0^{0,v_0}, & \text{sur}\ \partial B_\varepsilon, \\
%         w_\varepsilon^{0,v_0} = v_\omega(\cdot/\varepsilon), & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\omega(\cdot/\varepsilon)\|_{1/2,\partial B_R} \leq \|v_\omega(\cdot/\varepsilon)\|_{1,B_{R/2}\setminus B_R} \]
%     \[ \leq \|v_\omega(\cdot/\varepsilon)\|_{0,B_{R/2}\setminus B_R} + |v_\omega(\cdot/\varepsilon)|_{1,B_{R/2}\setminus B_R} \]
%     \[ \leq \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|v_\omega|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \]
%     \[ \leq \|V\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \|W\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|V|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} + \varepsilon|W|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \]
%     \[ \leq \big(C_5\,R^{1/2}\varepsilon^{-1/2} + C_6\,R^{-1/2}\varepsilon^{1/2} + C_7\,R^{-1/2}\varepsilon^{3/2} + C_8\,R^{1/2}\varepsilon^{1/2}\big)\|\psi\|_{1/2,\partial B_1} \]
%     \[ \leq C\,\varepsilon^{-1/2}\|\psi\|_{1/2,\partial B_1}. \]
    
%     Aussi, (Annexe)

%     \[ \| v_0(x_0) - v_0^{0,v_0}(\varepsilon \cdot) \|_{1/2,\partial B_1} \leq \| v_0(x_0) - v_0^{0,v_0}(\varepsilon \cdot) \|_{1, B_1\setminus B_{1/2}} \]
%     \[ \leq \| v_0(x_0) - v_0^{0,v_0}(\varepsilon \cdot) \|_{1, B_1} \]
    
%     Ainsi,
    
%     \[ |w_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C\big( \varepsilon^{?}\|v_\omega(x/\varepsilon)\|_{1/2,\partial B_R} + \varepsilon^{?}\|v_0(x_0) - v_0^{0,v_0}(\cdot/\varepsilon)\|_{1/2,\partial B_1} \big) \]
    
%     Enfin, (44)
    
%     \[ \|\nabla (v_\varepsilon^{0,\psi} - v_0^{0,\psi} + V^{0,\psi} ) \cdot n\|_{-1/2,\partial B_R} \leq C |v_\varepsilon^{0,\psi} - v_0^{0,\psi} + V^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ \leq C |v_\varepsilon^{0,\psi} - v_0^{0,\psi} + V^{0,\psi} + W^{0,\psi} - W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ = C |v_\varepsilon^{0,\psi} - v_0^{0,\psi} + v_\omega - W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ = C |w_\varepsilon - W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \]
%     \[ \leq C \Big(|w_\varepsilon|_{1,B_R\setminus B_{R/2}} + |W^{0,\psi} |_{1,B_R\setminus B_{R/2}} \Big) \]
    
% \newpage \section{Draft 2}

% \[ \Longrightarrow |V(y)| \leq C_1\, |y|^{-1/2}e^{-|y|/\sqrt{\alpha}}\, \|\varphi\|, \]
% \[ \Longrightarrow |W(y)| \leq C_2\, |y|^{-3/2}\, \|\varphi\|, \]
% \[ \Longrightarrow |\nabla V(y)| \leq C_3\,|y|^{-1/2}e^{-|y|/\sqrt{\alpha}} \, \|\varphi\|, \]
% \[ \Longrightarrow |\nabla W(y)| \leq C_4\, |y|^{-5/2}\, \|\varphi\|. \]

% ---------------------------------------------------------------------------------

% \[ \|V\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |V|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_3\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |W|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_4\, \, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|V\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_5\, e^{-R/(\varepsilon\sqrt{\alpha})}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |V|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_6\, e^{-R/(\varepsilon\sqrt{\alpha})}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_7\, \varepsilon^{1/2} \,\|\psi\|_{1/2,\partial B_1}, \]
% \[ |W|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_8\, \varepsilon^{3/2}\, \|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|V\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\,\|\psi\|_{1/2,\partial B_1}, \]
% \[ \|V\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_3\, e^{-R/(\varepsilon\sqrt{\alpha})} \,\|\psi\|_{1/2,\partial B_1}, \]
% \[ \|W\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_4\, \varepsilon^{1/2} \,\|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \[ \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_1} \leq C_1\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |v_\omega|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_2\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{1,B_{R/\varepsilon}\setminus B_1} \leq C_3\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{0,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_4\,\varepsilon^{1/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ |v_\omega|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_5\, \varepsilon^{3/2}\, \|\psi\|_{1/2,\partial B_1}, \]
% \[ \|v_\omega\|_{1,B_{R/\varepsilon}\setminus B_{R/(2\varepsilon)}} \leq C_6\,\varepsilon^{1/2}\, \|\psi\|_{1/2,\partial B_1}. \]

% ---------------------------------------------------------------------------------

% \begin{proposition} Soit $\psi\in H^{1/2}(\partial B_1)$.

%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta v_\varepsilon + v_\varepsilon = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         v_\varepsilon = \psi(\,\cdot\,/\varepsilon), & \text{sur}\ \partial B_\varepsilon, \\
%         v_\varepsilon = 0, & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\varepsilon\|_{0,B_R\setminus B_\varepsilon} \leq C_1\,\varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}, \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_\varepsilon} \leq C_2\,\varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}, \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C_3\,\varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}. \]
% \end{proposition}

% \begin{proposition} Soient $\psi\in H^{1/2}(\partial B_1)$ et $\varphi\in H^{1/2}(\partial B_R)$.
%     \[ \left \{ \begin{array}{cc}
%         -\alpha\Delta v_\varepsilon + v_\varepsilon = 0, & \text{dans}\ B_R\setminus B_\varepsilon, \\
%         v_\varepsilon = \psi(\,\cdot\,/\varepsilon), & \text{sur}\ \partial B_\varepsilon, \\
%         v_\varepsilon = \varphi, & \text{sur}\ \partial B_R.
%     \end{array} \right .\]
    
%     \[ \|v_\varepsilon\|_{0,B_R\setminus B_\varepsilon} \leq C_1\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}\big), \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_\varepsilon} \leq C_2\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}\big), \]
%     \[ |v_\varepsilon|_{1,B_R\setminus B_{R/2}} \leq C_3\,\big(\|\varphi\|_{1/2,\partial B_R} + \varepsilon^{3/2}\|\psi\|_{1/2,\partial B_1}\big). \]
% \end{proposition}


\section{Draft}


